Generating proof systems for three-valued propositional logics

In general, providing an axiomatization for an arbitrary logic is a task that may require some ingenuity. In the case of logics defined by a finite logical matrix (three-valued logics being a particularly simple example), the generation of suitable finite axiomatizations can be completely automatized, essentially by expressing the matrix tables via inference rules. In this chapter we illustrate how two formalisms, the 3-labelled calculi of Baaz, Ferm\"uller and Zach and the multiple-conclusion (or Set-Set) Hilbert-style calculi of Shoesmith and Smiley, may be uniformly employed to axiomatize logics defined by a three-valued logical matrix. The generating procedure common to both formalisms can be described as follows: first (i) convert the matrix semantics into rule form (we refer to this step as the generating subprocedure) and then (ii) simplify the set of rules thus obtained, essentially relying on the defining properties of any Tarskian consequence relation (we refer to this step as the streamlining subprocedure). We illustrate through some examples that, if a minimal expressiveness assumption is met (namely, if the matrix defining the logic is monadic), then it is straightforward to define effective translations guaranteeing the equivalence between the 3-labelled and the Set-Set approach.

==> 3LabelledL3.tex <==
\subsection{(Streamlined) 3-labelled calculus $(s)\ell.\textrm{\L}_3$}

Below we reproduce the logical rules of $\ell.\textrm{\L}3$ for 3-valued \L{}ukasiewicz logic. 
 
\begin{remark}
\label{notation:3LabelledRules}
Notice that the rules and the names of rules are in a one-to-one correspondence with matrix entries: the rule name `\,$\conn^{ij}_{k}$\,' identifies the matrix entries for binary connectives $\conn$ (resp.~unary connectives if $j$ is empty), where the vector $ij$ refers to the list of input values in the matrix (aka components of auxiliary formulas in the premise of a rule), and $k$ refers to the corresponding output value in the matrix (aka the component of the principal formula in the conclusion of the rule). Moreover, we color the output value in rules' names to emphasize all rules sharing the same output per each connective (this categorization will be relevant once we move to streamlined 3-valued calculi).
\end{remark}

\vspace{0.5cm}

\begin{math}
\hspace{1cm}
\AXC{$X, A \mid Y \mid Z$}
\RL{\fns $\aneg^\bv_\tvb$}
\UIC{$X \mid Y \mid Z, \aneg A$}
\DP
 \qquad
\AXC{$X \mid Y, A \mid Z$}
\RL{\fns $\aneg^\uv_\uvg$}
\UIC{$X \mid Y, \aneg A \mid Z$}
\DP
 \qquad
\AXC{$X \mid Y \mid Z, A$}
\RL{\fns $\aneg^\tv_\bvr$}
\UIC{$X, \aneg A \mid Y \mid Z$}
\DP
\end{math}

\vspace{0.8cm}

\begin{math}
\hspace{-2cm}
\AXC{$X, A \mid Y \mid Z$}
\AXC{$X, B \mid Y \mid Z$}
\RL{\fns $\aand^{\bv\bv}_\bvr$}
\BIC{$X, A \aand B \mid Y \mid Z$}
\DP
\ \ \  
\AXC{$X, A \mid Y \mid Z$}
\AXC{$X \mid Y, B \mid Z$}
\RL{\fns $\aand^{\bv\uv}_\bvr$}
\BIC{$X, A \aand B \mid Y \mid Z$}
\DP
\ \ \ 
\AXC{$X, A \mid Y \mid Z$}
\AXC{$X \mid Y \mid Z, B$}
\RL{\fns $\aand^{\bv\tv}_\bvr$}
\BIC{$X, A \aand B \mid Y \mid Z$}
\DP
\end{math}

\vspace{0.25cm}

\begin{math}
\hspace{-2cm}
\AXC{$X \mid Y, A \mid Z$}
\AXC{$X, B \mid Y \mid Z$}
\RL{\fns $\aand^{\uv\bv}_\bvr$}
\BIC{$X, A \aand B \mid Y \mid Z$}
\DP
\ \ \  
\AXC{$X \mid Y, A \mid Z$}
\AXC{$X \mid Y, B \mid Z$}
\RL{\fns $\aand^{\uv\uv}_\uvg$}
\BIC{$X \mid Y, A \aand B \mid Z$}
\DP
\ \ \ 
\AXC{$X \mid Y, A \mid Z$}
\AXC{$X \mid Y \mid Z, B$}
\RL{\fns $\aand^{\uv\tv}_\uvg$}
\BIC{$X \mid Y, A \aand B \mid Z$}
\DP
\end{math}

\vspace{0.25cm}

\begin{math}
\hspace{-2cm}
\AXC{$X \mid Y \mid Z, A$}
\AXC{$X, B \mid Y \mid Z$}
\RL{\fns $\aand^{\tv\bv}_\bvr$}
\BIC{$X, A \aand B \mid Y \mid Z$}
\DP
\ \ \ 
\AXC{$X \mid Y \mid Z, A$}
\AXC{$X \mid Y, B \mid Z$}
\RL{\fns $\aand^{\tv\uv}_\uvg$}
\BIC{$X \mid Y, A \aand B \mid Z$}
\DP
\ \ \ 
\AXC{$X \mid Y \mid Z, A$}
\AXC{$X \mid Y \mid Z, B$}
\RL{\fns $\aand^{\tv\tv}_\tvb$}
\BIC{$X \mid Y \mid Z, A \aand B$}
\DP
\end{math}

\vspace{0.8cm}

\begin{math}
\hspace{-2cm}
\AXC{$X, A \mid Y \mid Z$}
\AXC{$X, B \mid Y \mid Z$}
\RL{\fns $\aor^{\bv\bv}_\bvr$}
\BIC{$X, A \aor B \mid Y \mid Z$}
\DP
\ \ \  
\AXC{$X, A \mid Y \mid Z$}
\AXC{$X \mid Y, B \mid Z$}
\RL{\fns $\aor^{\bv\uv}_\bvr$}
\BIC{$X \mid Y, A \aor B \mid Z$}
\DP
\ \ \ 
\AXC{$X, A \mid Y \mid Z$}
\AXC{$X \mid Y \mid Z, B$}
\RL{\fns $\aor^{\bv\tv}_\bvr$}
\BIC{$X \mid Y \mid Z, A \aor B$}
\DP
\end{math}

\vspace{0.25cm}

\begin{math}
\hspace{-2cm}
\AXC{$X \mid Y, A \mid Z$}
\AXC{$X, B \mid Y \mid Z$}
\RL{\fns $\aor^{\uv\bv}_\bvr$}
\BIC{$X \mid Y, A \aor B \mid Z$}
\DP
\ \ \  
\AXC{$X \mid Y, A \mid Z$}
\AXC{$X \mid Y, B \mid Z$}
\RL{\fns $\aor^{\uv\uv}_\uvg$}
\BIC{$X \mid Y, A \aor B \mid Z$}
\DP
\ \ \ 
\AXC{$X \mid Y, A \mid Z$}
\AXC{$X \mid Y \mid Z, B$}
\RL{\fns $\aor^{\uv\tv}_\uvg$}
\BIC{$X \mid Y \mid Z, A \aor B$}
\DP
\end{math}

\vspace{0.25cm}

\begin{math}
\hspace{-2cm}
\AXC{$X \mid Y \mid Z, A$}
\AXC{$X, B \mid Y \mid Z$}
\RL{\fns $\aor^{\tv\bv}_\bvr$}
\BIC{$X \mid Y \mid Z, A \aor B$}
\DP
\ \ \ 
\AXC{$X \mid Y \mid Z, A$}
\AXC{$X \mid Y, B \mid Z$}
\RL{\fns $\aor^{\tv\uv}_\uvg$}
\BIC{$X \mid Y \mid Z, A \aor B$}
\DP
\ \ \ 
\AXC{$X \mid Y \mid Z, A$}
\AXC{$X \mid Y \mid Z, B$}
\RL{\fns $\aor^{\tv\tv}_\tvb$}
\BIC{$X \mid Y \mid Z, A \aor B$}
\DP
\end{math}

\vspace{0.8cm}

\begin{math}
\hspace{-2cm}
\AXC{$X, A \mid Y \mid Z$}
\AXC{$X, B \mid Y \mid Z$}
\RL{\fns $\ararr^{\bv\bv}_\bvr$}
\BIC{$X \mid Y \mid Z, A \ararr B$}
\DP
\ \ \  
\AXC{$X, A \mid Y \mid Z$}
\AXC{$X \mid Y, B \mid Z$}
\RL{\fns $\ararr^{\bv\uv}_\bvr$}
\BIC{$X \mid Y \mid Z, A \ararr B$}
\DP
\ \ \ 
\AXC{$X, A \mid Y \mid Z$}
\AXC{$X \mid Y \mid Z, B$}
\RL{\fns $\ararr^{\bv\tv}_\bvr$}
\BIC{$X \mid Y \mid Z, A \ararr B$}
\DP
\end{math}

\vspace{0.25cm}

\begin{math}
\hspace{-2cm}
\AXC{$X \mid Y, A \mid Z$}
\AXC{$X, B \mid Y \mid Z$}
\RL{\fns $\ararr^{\uv\bv}_\bvr$}
\BIC{$X \mid Y, A \ararr B \mid Z$}
\DP
\ \ \  
\AXC{$X \mid Y, A \mid Z$}
\AXC{$X \mid Y, B \mid Z$}
\RL{\fns $\ararr^{\uv\uv}_\uvg$}
\BIC{$X \mid Y \mid Z, A \ararr B$}
\DP
\ \ \ 
\AXC{$X \mid Y, A \mid Z$}
\AXC{$X \mid Y \mid Z, B$}
\RL{\fns $\ararr^{\uv\tv}_\uvg$}
\BIC{$X \mid Y \mid Z, A \ararr B$}
\DP
\end{math}

\vspace{0.25cm}

\begin{math}
\hspace{-2cm}
\AXC{$X \mid Y \mid Z, A$}
\AXC{$X, B \mid Y \mid Z$}
\RL{\fns $\ararr^{\tv\bv}_\bvr$}
\BIC{$X, A \ararr B \mid Y \mid Z$}
\DP
\ \ \ 
\AXC{$X \mid Y \mid Z, A$}
\AXC{$X \mid Y, B \mid Z$}
\RL{\fns $\ararr^{\tv\uv}_\uvg$}
\BIC{$X, A \ararr B \mid Y \mid Z$}
\DP
\ \ \ 
\AXC{$X \mid Y \mid Z, A$}
\AXC{$X \mid Y \mid Z, B$}
\RL{\fns $\ararr^{\tv\tv}_\tvb$}
\BIC{$X \mid Y \mid Z, A \ararr B$}
\DP
\end{math}

\vspace{0.5cm}



Below we list the logical rules of the streamlined 3-labelled calculus $s\ell.\mbox{\L}3$ for 3-valued \L{}ucasiewicz logic automatically generated by the system Multilog \cite{MultlogLuk21} (we simply adjusted the notation). 

\vspace{0.5cm}

\begin{math}
\hspace{1cm}
\AXC{$X \mid Y \mid Z, A$}
\RL{\fns $\aneg_\bvr$}
\UIC{$X, \aneg A \mid Y \mid Z$}
\DP
 \qquad
\AXC{$X \mid Y, A \mid Z$}
\RL{\fns $\aneg_\uvg$}
\UIC{$X \mid Y, \aneg A \mid Z$}
\DP
 \qquad
\AXC{$X, A \mid Y \mid Z$}
\RL{\fns $\aneg_\tvb$}
\UIC{$X \mid Y \mid Z, \aneg A$}
\DP
\end{math}

\vspace{0.8cm}

\begin{math}
\hspace{-3cm}
\AXC{$X, A, B \mid Y \mid Z$}
\RL{\fns $\aand_\bvr$}
\UIC{$X, A \aand B \mid Y \mid Z$}
\DP
 \ \ \ 
\AXC{$X \mid Y, A \mid Z, A \ \ \ X \mid Y, A, B \mid Z \ \ \ 
X \mid Y, B \mid Z, B$}
\RL{\fns $\aand_\uvg$}
\UIC{$X \mid Y, A \aand B \mid Z$}
\DP
 \ \ \ 
\AXC{$X \mid Y \mid Z, A$}
\AXC{$X \mid Y \mid Z, B$}
\RL{\fns $\aand_\tvb$}
\BIC{$X \mid Y \mid Z, A \aand B$}
\DP
\end{math}

\vspace{0.8cm}

\begin{math}
\hspace{-3cm}
\AXC{$X, A \mid Y \mid Z$}
\AXC{$X, B \mid Y \mid Z$}
\RL{\fns $\aor_\bvr$}
\BIC{$X, A \aor B \mid Y \mid Z$}
\DP
 \ \ \ 
\AXC{$X, A \mid Y, A \mid Z \ \ \ X \mid Y, A, B \mid Z \ \ \ 
X, B \mid Y, B \mid Z$}
\RL{\fns $\aor_\uvg$}
\UIC{$X \mid Y, A \aor B \mid Z$}
\DP
 \ \ \ 
\AXC{$X \mid Y \mid Z, A, B$}
\RL{\fns $\aor_\tvb$}
\UIC{$X \mid Y \mid Z, A \aor B$}
\DP
\end{math}

 \vspace{0.8cm}

\begin{math}
\hspace{-3cm}
\AXC{$X \mid Y \mid Z, A$}
\AXC{$X, B \mid Y \mid Z$}
\RL{\fns $\ararr_\bvr$}
\BIC{$X, A \ararr B \mid Y \mid Z$}
\DP
 \ \  
\AXC{$X, B \mid Y \mid Z, A$}
\AXC{$X \mid Y, A, B \mid Z$}
\RL{\fns $\ararr_\uvg$}
\BIC{$X \mid Y, A \ararr B \mid Z$}
\DP
 \ \ 
\AXC{$X, A \mid Y, A \mid Z, B$}
\AXC{$X, A \mid Y, B \mid Z, B$}
\RL{\fns $\ararr_\tvb$}
\BIC{$X \mid Y \mid Z, A \ararr B$}
\DP
\end{math}

\vspace{0.5cm}

\begin{proposition}
Notice that, per each connective $\conn$, the set of three-labelled rules introducing $\conn$ in the $i$-component is equivalent to the streamlined three-labelled rule $\conn_i$.
\end{proposition}

\begin{proof}
Here we only consider the case of conjunction. The rule $\aand_{\bvr}$ says that `$A \aand B$ is $\bv$ iff $A$ is $\bv$ or $B$ is $\bv$': so, this covers all the 3-labelled rules with $\bvr$ in the subscript, i.e.~the previous iff-clause is (classically) equivalent to the disjunction of the if-then-clauses capturing $\aand^{\bv\bv}_\bvr$, $\aand^{\bv\uv}_\bvr$, $\aand^{\bv\tv}_\bvr$, and $\aand^{\uv\bv}_\bvr$ respectively. 

The rule $\aand_\uvg$ says that `$A \aand B$ is $\uv$ iff $A$ is $\uv$ or $\tv$ (first premise) and $B$ is $\uv$ or $\tv$ (third premise) and $A$ or $B$ is $\uv$ (second premise)', namely at least one between $A$ and $B$ is $\uv$ and both of them are not $\bv$: so, this covers all the 3-labelled rules with $\uvg$ in the subscript, i.e.~the previous iff-clause is (classically) equivalent to the disjunction of the if-then-clauses capturing $\aand^{\uv\uv}_\uvg$, $\aand^{\uv\tv}_\uvg$, and $\aand^{\tv\uv}_\uvg$ respectively. 

The rule $\aand_\tvb$ says that `$A \aand B$ is $\tv$ iff $A$ is $\tv$ and $B$ is $\tv$': so, this covers all the 3-labelled rules with $\tvb$ in the subscript, i.e.~the previous iff-clause is (classically) equivalent to the if-then-clause capturing $\aand^{\tv\tv}_\tvb$ (notice that, after all, the clause capturing $\aand^{\tv\tv}_\tvb$ has to be an iff-clause too, and, indeed, it corresponds to a single entry in the matrix).
\end{proof}

Below we provide an $s\ell.\textrm{\L}3$-derivation of $(\aneg B \ararr \aneg A) \ararr (A \ararr B)$ automatically generated by the system Multiseq \cite{Multseq} (where the actual sets of formulas are listed immediately after the proof tree):

\vspace{0.5cm}

\begin{math}
\hspace{-1.5cm}
{\small
\infer[\ararr_\tv]{1}%
{\infer[\ararr_\tv]{2}%
{\infer[\ararr_\bv]{3}%
{\infer[\aneg_\tv]{4}%
{\infer[\ararr_\uv]{5}%
{\infer[\aneg_\uv]{6}%
{\infer[\aneg_\uv]{7}%
{\deduce{8}%
{}
}
}
&
\infer[\aneg_\bv]{9}%
{\deduce{10}%
{}
}
}
}
&
\infer[\aneg_\bv]{11}%
{\deduce{12}%
{}
}
}
&
\infer[\ararr_\bv]{13}%
{\infer[\aneg_\tv]{14}%
{\deduce{15}%
{}
}
&
\infer[\aneg_\bv]{16}%
{\infer[\ararr_\uv]{17}%
{\infer[\aneg_\uv]{18}%
{\deduce{19}%
{}
}
&
\infer[\aneg_\bv]{20}%
{\infer[\aneg_\tv]{21}%
{\deduce{22}%
{}
}
}
}
}
}
}
&
\infer[\ararr_\uv]{23}%
{\infer[\ararr_\tv]{24}%
{\infer[\ararr_\bv]{25}%
{\infer[\aneg_\tv]{26}%
{\deduce{8}%
{}
}
&
\infer[\aneg_\bv]{27}%
{\deduce{28}%
{}
}
}
&
\infer[\ararr_\bv]{25}%
{\infer[\aneg_\tv]{26}%
{\deduce{8}%
{}
}
&
\infer[\aneg_\bv]{27}%
{\deduce{28}%
{}
}
}
}
&
\infer[\ararr_\tv]{29}%
{\deduce{30}%
{}
&
\deduce{31}%
{}
}
}
}
 }
\end{math}

\vspace{0.5cm}

The list of formulas {\color{red}3-labelled formulas?3-sequents?} occurring in the previous derivation is the following:

\begin{center}
\begin{tabular}{rl}
\begin{tabular}{@{}rl}
1{:} & $\emptyset \mid \emptyset \mid ((\neg B\ararr \neg A)\ararr (A\ararr B))$ \\
2{:} & $(\neg B\ararr \neg A) \mid (\neg B\ararr \neg A) \mid (A\ararr B)$ \\
3{:} & $A, (\neg B\ararr \neg A) \mid A, (\neg B\ararr \neg A) \mid B$ \\
4{:} & $A \mid A, (\neg B\ararr \neg A) \mid B, \neg B$ \\
5{:} & $A, B \mid A, (\neg B\ararr \neg A) \mid B$ \\
6{:} & $A, B \mid A, \neg A, \neg B \mid B$ \\
7{:} & $A, B \mid A, \neg B \mid B$ \\
8{:} & $A, B \mid A, B \mid B$ \\
9{:} & $A, B, \neg A \mid A \mid B, \neg B$ \\
10{:} & $A, B \mid A \mid A, B, \neg B$ \\
11{:} & $A, \neg A \mid A, (\neg B\ararr \neg A) \mid B$ \\
12{:} & $A \mid A, (\neg B\ararr \neg A) \mid A, B$ \\
13{:} & $A, (\neg B\ararr \neg A) \mid B, (\neg B\ararr \neg A) \mid B$ \\
14{:} & $A \mid B, (\neg B\ararr \neg A) \mid B, \neg B$ \\
15{:} & $A, B \mid B, (\neg B\ararr \neg A) \mid B$ \\
16{:} & $A, \neg A \mid B, (\neg B\ararr \neg A) \mid B$ \\
\end{tabular}
 & 
\begin{tabular}{rl@{}}
17{:} & $A \mid B, (\neg B\ararr \neg A) \mid A, B$ \\
18{:} & $A \mid B, \neg A, \neg B \mid A, B$ \\
19{:} & $A \mid A, B, \neg B \mid A, B$ \\
20{:} & $A, \neg A \mid B \mid A, B, \neg B$ \\
21{:} & $A \mid B \mid A, B, \neg B$ \\
22{:} & $A, B \mid B \mid A, B$ \\
23{:} & $(\neg B\ararr \neg A) \mid (A\ararr B) \mid (A\ararr B)$ \\
24{:} & $(\neg B\ararr \neg A) \mid A, B \mid (A\ararr B)$ \\
25{:} & $A, (\neg B\ararr \neg A) \mid A, B \mid B$ \\
26{:} & $A \mid A, B \mid B, \neg B$ \\
27{:} & $A, \neg A \mid A, B \mid B$ \\
28{:} & $A \mid A, B \mid A, B$ \\
29{:} & $B, (\neg B\ararr \neg A) \mid \emptyset \mid A, (A\ararr B)$ \\
30{:} & $A, B, (\neg B\ararr \neg A) \mid A \mid A, B$ \\
31{:} & $A, B, (\neg B\ararr \neg A) \mid B \mid A, B$ \\
 & \\
\end{tabular}
 \\
\end{tabular}
\end{center}



==> FromSMCLToSLL.tex <==
\section{From $smc.L$ to $s\ell.L$}
\label{FromSMCLToSLL}

In this section we provide a more general version of Theorem \ref{thm:Derivability-MultipleToLabelledCalculi}.

Recall that the statement $\varphi_1 \mid \ldots \mid \varphi_k$ is an abbreviation for $v_1\colon \varphi_1, \ldots, v_k\colon \varphi_k$ where $\ell = \{v_1, \ldots, v_n\}$ is the set of labels and $\varphi_i$ with $1 \leq i \leq k$ are (possibly different) wffs (see section \ref{sec:3LabelledCalculi}). 

The writing $\{v_1, \ldots, v_n\}\colon \varphi$ is an abbreviation for $v_1\colon \varphi, \ldots, v_k\colon \varphi$. 

Let $\{V_1\}$ and $\{V_2\}$ be two sets of labels, $S$ a sequent, and let the writing $S\,[\{V_i\}\colon \varphi]$ stay for `$\{V_i\}\colon \varphi$ occurs in the sequent $S$'. 

Cut rules (sometimes called multi-cuts or mix rules, see \cite{Gentzen}) can be now defined in a compact way as follows \cite{Baaz}:

\begin{center}
\AXC{$S\, [\{V_1\}\colon \varphi]$}
\AXC{$S\, [\{V_2\}\colon \varphi]$}
\RL{\fns Cut$_{\{V_1\},\{V_2\}}$}
\BIC{$S\, [\{V_1 \cap V_2\}\colon \varphi]$}
\DP
\end{center}

Notice that whenever $V_1 \cap V_2 = \emptyset\colon \varphi$, we simply do not write it in the conclusion. The case where $V_1$ and $V_2$ are disjoint singletons are a particular case (see the specific definitions of the rules Cut$_{\bv,\uv}$, Cut$_{\uv,\tv}$, Cut$_{\bv,\tv}$ in section \ref{sec:3LabelledCalculi}).    

\begin{theorem}
\label{thm:Derivability-MultipleToLabelledCalculi-General}
Let us consider any logic L presentable via a single finite-valued matrix with $\{N\} = \{n_1, \ldots, n_k\}$ and $\{D\} = \{d_1, \ldots, d_l\}$ the sets of non-designated and designated elements, respectively. The translation $\lf\cdot\rf$ from $smc.\textrm{L}$-rules to $s\ell.\textrm{L}$-rules  

\vspace{0.5cm}

\begin{math}
\hspace{-0.9cm}
\begin{tabular}{c@{}c@{}c}
$\left\lf
\AXC{$\varphi_1$}
\AXC{$\cdots$}
\AXC{$\varphi_n$}
\RL{$\mathsf{r}^\conn$}
\TIC{$\psi_1, \ldots, \psi_m$}
\DP
\right\rf$
 & \ $:=$ \ &
\AXC{$\{N\}\colon \emptyset \mid \{D\}\colon \varphi_1$}
\AXC{$\cdots$}
\AXC{$\{N\}\colon \emptyset \mid \{D\}\colon \varphi_n$}
\RL{$\lf\mathsf{r}^\conn\rf$}
\TIC{$\{N\}\colon \emptyset \mid  \{D\}\colon \psi_1, \ldots, \{D\}\colon \psi_m$}
\DP
 \\
\end{tabular}
\end{math}

\vspace{0.5cm}

is derivable in $s\ell.\textrm{L}$ extended with open assumptions, i.e.~zeroary rules $\neq \textrm{Id}_\varphi$.
\end{theorem}

\begin{proof}
The calculus $sm.\textrm{L}$ is sound w.r.t.~the finite matrix presentation of L, and the $sm.\textrm{L}$-rules preserve designated values, so: 

\begin{center}
\begin{tabular}{cl}
    & $\mathsf{r}^\conn \in sm.\textrm{L}$ is sound \\
\rule[-3mm]{0mm}{0.8cm} iff & $(\SAND_{i=1}^n \varphi_i^L \in \{D\}) \Srarr (\SOR_{j=1}^m \psi_j^L \in \{D\})$ \\
\rule[-3mm]{0mm}{0.8cm} iff & $\Sneg (\SAND_{i=1}^n \varphi_i^L \in \{D\}) \Sor (\SOR_{j=1}^m \psi_j^L \in \{D\})$ \\
\rule[-3mm]{0mm}{0.8cm} iff & $(\SOR_{i=1}^n \Sneg (\varphi_i^L \in \{D\})) \Sor (\SOR_{j=1}^m \psi_j^L \in \{D\})$ \\
\rule[-3mm]{0mm}{0.8cm} iff & $(\SOR_{i=1}^n \varphi_i^L \in \{N\}) \Sor (\SOR_{j=1}^m \psi_j^L \in \{D\})$ \\
\end{tabular}
\end{center}

On the other hand, the calculus $s\ell.\textrm{L}$ is complete w.r.t.~the finite matrix presentation of L, so:

\begin{center}
\begin{tabular}{c}
$(\SOR_{i=1}^n \varphi_i^L \in \{N\}) \Sor (\SOR_{j=1}^m \psi_j^L \in \{D\})$ is valid in L \\
\rule[-3mm]{0mm}{0.8cm} iff \\ 
the associated sequent $S({\mathsf{r}^\conn}) := \SOR_{i=1}^n \{N\}\colon \varphi_i \mid \SOR_{j=1}^m \{D\}\colon \psi_j$ is derivable in $s\ell.\textrm{L}$. \\
\end{tabular}
\end{center}

First, we generate a cut-free $s\ell.\textrm{L}$-derivation $\pi$ of the associated sequent $S(\mathsf{r}^\conn)$ (for instance, via backward-looking proof search given that $s\ell.\textrm{L}$ has syntactic cut elimination \cite{xxx}). Then, assuming each premise of $\lf\mathsf{r}^\conn\rf$ as many times as non-designated elements (as open assumptions) we perform $k$ subsequent applications of Cut$_{\{D\},\{n_i\}}$ on cut formulas $\varphi_1$ as follows:

\vspace{0.5cm}

\begin{math}
\hspace{-3cm}
\AXC{\fns Asm}
\UIC{$\{N\}\colon \emptyset \mid \{D\}\colon \varphi_1$}
%%
\AXC{$ \ $}
%
\AXC{\fns Asm}
\UIC{$\{N\}\colon \emptyset \mid \{D\}\colon \varphi_1$}
\AXC{$\pi$}
\noLine
\UIC{$n_1\colon \varphi_1, \{N\setminus \{n_1\}\}\colon \varphi_1, \SOR_{i=2}^{n} \{N\}\colon \varphi_i \mid \SOR_{j=1}^m \{D\}\colon \psi_j$}
\RL{\fns Cut$_{\{D\},n_1}$}
\BIC{$n_2\colon \varphi_1, \{N\setminus \{n_1, n_2\}\}\colon \varphi_1, \SOR_{i=2}^{n} \{N\}\colon \varphi_i \mid \SOR_{j=1}^m \{D\}\colon \psi_j$}
%
\noLine
\UIC{$\iddots$}
%%
\noLine
\BIC{$n_k\colon \varphi_1 \SOR_{i=2}^{n} \{N\}\colon \varphi_i \mid \SOR_{j=1}^m \{D\}\colon \psi_j$}
\RL{\fns Cut$_{\{D\},n_k}$}
\BIC{$\e \mid n_1\colon \varphi_2, \{N\setminus \{n_1\}\}\colon \varphi_2 \SOR_{i=3}^{n} \{N\}\colon \varphi_i \mid \SOR_{j=1}^m \psi_j$}
\DP
\end{math}

\vspace{0.5cm}

We then repeat the same procedure for every $\varphi_i$ with $2 \leq i \leq n$ and we obtain the end-sequent $\{N\}\colon \emptyset \mid \SOR_{j=1}^m \psi_j$.

So, for each rule $\textrm{r}^\conn$ in $sm.\textrm{L}$, the translation $\lf\textrm{r}^\conn\rf$ is derivable in $s\ell.\textrm{L}$.
\end{proof}

==> FromSML3ToSL3.tex <==
\section{From $smc.\textrm{\L{}3}$-proofs to $s\ell.\textrm{\L{}3}$-proofs}
\label{FromSMCL3ToSLL3}

Now we consider our running example \L{}3 and we show that:
\begin{proposition}
\label{prop:TranslationL3}
The translations of $smc.\textrm{\L{}}3$-rules (see theorem \ref{thm:Derivability-MultipleToLabelledCalculi}) are derivable in $s\ell.\textrm{\L{}}3$.
\end{proposition}

\begin{proof}
Let us consider the $smc.\textrm{\L{}}3$ rules for $\aneg$:

\vspace{0,5cm}

\begin{math}
\hspace{3cm}
\AXC{$\varphi$} 
\RL{\fns $\mathsf{I}_9^\aneg$}
\UIC{$\neg\neg\varphi$}        
\DP
 \ \ \
\AXC{$\neg\varphi$}
\AXC{$\varphi$}
\RL{\fns $\mathsf{E}_1^\aneg$}
\BIC{$\phantom{\varphi}$}
\DP
 \ \ \ 
\AXC{$\neg\neg\varphi$}
\RL{\fns $\mathsf{E}_{22}^\aneg$}
\UIC{$\varphi$}        
\DP
\end{math}

\vspace{0.5cm}

We need to show that assuming the translation of the premise(s) of rules for $\aneg$ we can derive the translation of the conclusion(s). Below we simply derive the associated sequent $S({\mathsf{r}^\aneg})$ without performing the cuts afterwards.

\vspace{0.5cm}

{\small
\begin{math}
\hspace{1.1cm}
\AXC{\fns Id$_{\varphi}$}
%\RL{\fns Id$_\varphi$}
\UIC{$\varphi \mid \varphi \mid \varphi$}
\RL{\fns $\aneg_\bvr$}
\UIC{$\aneg \varphi \mid \varphi \mid \e$}
\RL{\fns $\aneg_\tvb$}
\UIC{$\underbrace{\varphi \mid \varphi \mid \aneg \aneg \varphi}_{\mathsf{I}9}$}
\DP
 \ \ \ \ 
\AXC{\fns Id$_{\varphi}+W_{\uv}$}
%\RL{\fns Id$_{\varphi}+W_{\uv}$}
%\UIC{$\varphi \mid \varphi \mid \varphi$}
%\RL{\fns $W_{\uv}$}
\UIC{$\varphi \mid \varphi, \varphi \mid \varphi$}
\RL{\fns $\aneg_\bvr$}
\UIC{$\varphi, \aneg \varphi \mid \varphi, \varphi \mid \e$}
\RL{\fns $\aneg_\uvg$}
\UIC{$\underbrace{\varphi, \aneg \varphi \mid \varphi, \aneg \varphi \mid \e}_{\mathsf{E}1}$}
\DP
 \ \ \ \
\AXC{\fns Id$_{\varphi}$}
%\RL{\fns Id$_{\varphi}$}
\UIC{$\varphi \mid \varphi \mid \varphi$}
\RL{\fns $\aneg_{\tvb}$}
\UIC{$\varphi \mid \varphi \mid \aneg \varphi, \varphi$}
\RL{\fns $\aneg_{\bvr}$}
\UIC{$\aneg \aneg \varphi \mid \varphi \mid \varphi$}
%\RL{\fns $\aneg_{\uvg}$}
%\UIC{$\aneg \aneg \varphi \mid \aneg \varphi \mid \varphi$}
\RL{\fns $\aneg_{\uvg}\times 2$}
\UIC{$\underbrace{\aneg \aneg \varphi \mid \aneg \aneg \varphi \mid \varphi}_{\mathsf{E}22}$}
\DP
\end{math}
 }

\vspace{0,5cm}

Let us consider the $smc.\textrm{\L{}}3$ rules for $\aand$:

\vspace{0,5cm}

\begin{math}
\hspace{-3.8cm}
\AXC{$\varphi$}
\AXC{$\psi$} 
\RL{\fns $\mathsf{I}_5^\aand$}
\BIC{$\varphi \land \psi$}
\DP
\ \ \ 
\AXC{$\neg\varphi$} 
\RL{\fns $\mathsf{I}_7^\aand$}
\UIC{$\neg(\varphi \land \psi)$}
\DP
 \ \ \
\AXC{$\neg\psi$}
\RL{\fns $\mathsf{I}_8^\aand$}
\UIC{$\neg(\varphi \land \psi)$}
\DP
 \ \ \ 
\AXC{$\neg(\varphi \land \psi)$}
\AXC{$\psi$}
\RL{\fns $\mathsf{E}_{12}^\aand$}
\BIC{$\neg\varphi$}
\DP
 \ \ \ 
\AXC{$\neg(\varphi \land \psi)$}
\RL{\fns $\mathsf{E}_{14}^\aand$}
\UIC{$\neg\varphi, \neg\psi$}
\DP
 \ \ \ 
\AXC{$\neg(\varphi \land \psi)$}
\AXC{$\varphi$}
\RL{\fns $\mathsf{E}_{16}^\aand$}
\BIC{$\neg\psi$}
\DP
 \ \ \ 
\AXC{$\varphi \land \psi$}  
\RL{\fns $\mathsf{E}_{20}^\aand$}
\UIC{$\varphi$}        
\DP
 \ \ \
\AXC{$\varphi \land \psi$}  
\RL{\fns $\mathsf{E}_{25}^\aand$}
\UIC{$\psi$}        
\DP
\end{math} 

\vspace{0.5cm}

We need to show that assuming the translation of the premise(s) of rules for $\aand$ we can derive the translation of the conclusion(s). Below we simply derive the associated sequent $S({\mathsf{r}^\aand})$ without performing the cuts afterwards.

\vspace{0.5cm}

{\footnotesize
\begin{math}
\hspace{1.5cm}
\AXC{$ \ $}
\RL{\fns Id$_\varphi$}
\UIC{$\varphi \mid \varphi \mid \varphi$}
\AXC{$ \ $}
\RL{\fns Id$_\psi$}
\UIC{$\psi \mid \psi \mid \psi$} 
\RL{\fns $\aand_\tvb$}
\BIC{$\underbrace{\varphi, \psi \mid \varphi, \psi \mid \varphi \aand \psi}_{\mathsf{r}5}$}
\DP
 \ \ \ \ \ 
\AXC{\fns Id$_\varphi+W_\bv$}
%\RL{Id$_\varphi$}
%\UIC{$\varphi \mid \varphi \mid \varphi$}
%\RL{\fns $W_\bv$}
\UIC{$\varphi, \psi \mid \varphi \mid \varphi$}
\RL{\fns $\aand_\bvr$}
\UIC{$\varphi \aand \psi \mid \varphi \mid \varphi$}
\RL{\fns $\aneg_\bvr$}
\UIC{$\aneg \varphi, \varphi \aand \psi \mid \varphi \mid \e$}
\RL{\fns $\aneg_\uvg$}
\UIC{$\aneg \varphi, \varphi \aand \psi \mid \aneg \varphi \mid \e$}
\RL{\fns $\aneg_\tvb$}
\UIC{$\underbrace{\aneg \varphi \mid \aneg \varphi \mid \aneg (\varphi \aand \psi)}_{\mathsf{r}7 \ (\mathsf{r}8)}$}
\DP
\end{math}

\vspace{0.5cm}

\begin{math}
\hspace{-0.5cm}
\AXC{\fns Id$_\varphi+W_\bv+W_\tv$}
%\RL{\fns Id$_\varphi+W_\bv+W_\tv$}
%\UIC{$\varphi \mid \varphi \mid \varphi$}
%\RL{\fns $W_\bv$}
%\UIC{$\varphi, \psi \mid \varphi \mid \varphi$}
%\RL{\fns $W_\tv$}
\UIC{$\varphi, \psi \mid \varphi \mid \varphi, \varphi$}
%
\AXC{\fns Id$_\varphi+W_\bv+W_{\uv}$}
%\RL{\fns Id$_\varphi$}
%\UIC{$\varphi \mid \varphi \mid \varphi$}
%\RL{\fns $W_\bv$}
%\UIC{$\varphi, \psi \mid \varphi \mid \varphi$}
%\RL{\fns $W_{\uv}$}
\UIC{$\varphi, \psi \mid \varphi, \psi \mid \varphi$}
%
\AXC{\fns Id$_\psi+W_\bv+W_\tv$}
%\RL{\fns Id$_\psi$}
%\UIC{$\psi \mid \psi \mid \psi$}
%\RL{\fns $W_\bv$}
%\UIC{$\varphi, \psi \mid \psi \mid \psi$}
%\RL{\fns $W_\tv$}
\UIC{$\varphi, \psi \mid \psi \mid \varphi, \psi$}
%
\RL{\fns $\aand_\uvg$}
\TIC{$\varphi, \psi \mid \varphi \aand \psi, \psi \mid \varphi$}
%%
\AXC{\fns Id$_\psi+W_\bv+W_{\uv}$}
%\RL{\fns Id$_\psi$}
%\UIC{$\psi \mid \psi \mid \psi$}
%\RL{\fns $W_{\bv}$}
%\UIC{$\varphi, \psi \mid \psi \mid \psi$}
%\RL{\fns $W_{\uv}$}
\UIC{$\varphi, \psi \mid \varphi \aand \psi, \psi \mid \psi$}
%%
\RL{\fns $\aand_\tvb$}
\BIC{$\varphi, \psi \mid \varphi \aand \psi, \psi \mid \varphi \aand \psi$}
\RL{\fns $\aneg_\bvr$}
\UIC{$\aneg (\varphi \aand \psi), \varphi, \psi \mid \varphi \aand \psi, \psi \mid \e$}
\RL{\fns $\aneg_\uvg$}
\UIC{$\aneg (\varphi \aand \psi), \varphi, \psi \mid \aneg (\varphi \aand \psi), \psi \mid \e$}
\RL{\fns $\aneg_\tvb$}
\UIC{$\underbrace{\aneg (\varphi \aand \psi), \psi \mid \aneg (\varphi \aand \psi), \psi \mid \aneg \varphi}_{\mathsf{r}12 \ (\mathsf{r}16)}$}
\DP
\end{math}

\vspace{0.5cm}

\begin{math}
\hspace{-1.6cm}
\AXC{\fns Id$_{\varphi}+W_\bv$}
\UIC{$\varphi, \psi \mid \varphi \mid \varphi$}
\AXC{\fns Id$_{\varphi}+W_\bv+W_{\uv}$}
\UIC{$\varphi, \psi \mid \varphi, \psi \mid \varphi$}
\AXC{\fns Id$_{\psi}+W_\bv$}
\UIC{$\varphi, \psi \mid \psi \mid \psi$}
\RL{\fns $\aand_{\uvg}$}
\TIC{$\varphi, \psi \mid \varphi \aand \psi \mid \varphi$}
%
\AXC{\fns Id$_{\varphi}+W_\bv$}
\UIC{$\varphi, \psi \mid \varphi \mid \varphi$}
\AXC{\fns Id$_{\psi}+W_\bv+W_{\uv}$}
\UIC{$\varphi, \psi \mid \varphi, \psi \mid \psi$}
\AXC{\fns Id$_{\psi}+W_\bv$}
\UIC{$\varphi, \psi \mid \psi \mid \psi$}
\RL{\fns $\aand_{\uvg}$}
\TIC{$\varphi, \psi \mid \varphi \aand \psi \mid \psi$}
%
\RL{\fns $\aand_{\tvb}$}
\BIC{$\varphi, \psi \mid \varphi \aand \psi \mid \varphi \aand \psi$}
\RL{\fns $\aneg_{\bvr}$}
\UIC{$\aneg (\varphi \aand \psi), \varphi, \psi \mid \varphi \aand \psi \mid \e$}
\RL{\fns $\aneg_{\uvg}$}
\UIC{$\aneg (\varphi \aand \psi), \varphi, \psi \mid \aneg (\varphi \aand \psi) \mid \e$}
%\RL{\fns $\aneg_{\tvb}$}
%\UIC{$\aneg (\varphi \aand \psi), \psi \mid \aneg (\varphi \aand \psi) \mid \aneg \varphi$}
\RL{\fns $\aneg_{\tvb} \times 2$}
\UIC{$\underbrace{\aneg (\varphi \aand \psi) \mid \aneg (\varphi \aand \psi) \mid \aneg \varphi, \aneg \psi}_{\mathsf{r}14}$}
\DP
\end{math}

\vspace{0.5cm}

\begin{math}
\hspace{1.8cm}
\AXC{\fns Id$_{\varphi}+W_\bv$}
\UIC{$\varphi, \psi \mid \varphi \mid \varphi$}
\AXC{\fns Id$_{\varphi}+W_\bv+W_{\uv}$}
\UIC{$\varphi, \psi \mid \varphi, \psi \mid \varphi$}
\AXC{\fns Id$_{\psi}+W_\bv$}
\UIC{$\varphi, \psi \mid \psi \mid \psi$}
\RL{\fns $\aand_{\uvg}$}
\TIC{$\varphi, \psi \mid \varphi \aand \psi \mid \varphi$}
\RL{\fns $\aand_{\bvr}$}
\UIC{$\underbrace{\varphi \aand \psi \mid \varphi \aand \psi \mid \varphi}_{\mathsf{r}20 \ (\mathsf{r}25)}$}
\DP
\end{math}

\vspace{0.5cm}

 }
 
Let us consider the $smc.\textrm{\L{}}3$ rules for $\aor$:

\vspace{0.5cm}

\begin{math}
\hspace{-0.3cm}
\AXC{$\neg\varphi$}
\AXC{$\neg\psi$}
\RL{\fns $\mathsf{I}_{10}^\aor$}
\BIC{$\neg(\varphi \lor \psi)$}        
\DP
 \ \ 
\AXC{$\neg(\varphi \lor \psi)$}
\RL{\fns $\mathsf{E}_{13}^\aor$}
\UIC{$\neg\varphi$}
\DP
 \ \  
\AXC{$\neg(\varphi \lor \psi)$}
\RL{\fns $\mathsf{E}_{17}^\aor$}
\UIC{$\neg\psi$}
\DP 
 \ \  
\AXC{$\varphi$} 
\RL{\fns $\mathsf{I}_{18}^\aor$}
\UIC{$\varphi \lor \psi$}        
\DP
 \ \  
\AXC{$\psi$} 
\RL{\fns $\mathsf{I}_{19}^\aor$}
\UIC{$\varphi \lor \psi$}        
\DP
 \ \  
\AXC{$\varphi \aor \psi$}
\RL{\fns $\mathsf{E}_{23}^\aor$}
\UIC{$\varphi, \psi$}
\DP
\end{math}

\vspace{0.5cm}

We need to show that assuming the translation of the premise(s) of rules for $\aor$ we can derive the translation of the conclusion(s). Below we simply derive the associated sequent $S({\mathsf{r}^\aor})$ without performing the cuts afterwards.

\vspace{0.5cm}

{\footnotesize

\begin{math}
\hspace{2.2cm}
\AXC{\fns Id$_{\varphi}+W_{\uv}+W_\tv$}
\UIC{$\varphi \mid \varphi, \psi \mid \varphi, \psi$}
\AXC{\fns Id$_{\psi}+W_{\uv}+W_\tv$}
\UIC{$\psi \mid \varphi, \psi \mid \varphi, \psi$}
\RL{\fns $\aor_\bvr$}
\BIC{$\varphi \aor \psi \mid \varphi, \psi \mid \varphi, \psi$}
%\RL{\fns $\aneg_\bvr$}
%\UIC{$\varphi \aor \psi, \neg \varphi \mid \varphi, \psi \mid \psi$}
\RL{\fns $\aneg_\bvr \times 2$}
\UIC{$\varphi \aor \psi, \aneg \varphi, \aneg \psi \mid \varphi, \psi \mid \e$}
%\RL{\fns $\aneg_{\uvg}$}
%\UIC{$\varphi \aor \psi, \aneg \varphi, \aneg \psi \mid \aneg \varphi, \psi \mid \e$}
\RL{\fns $\aneg_{\uvg} \times 2$}
\UIC{$\varphi \aor \psi, \aneg \varphi, \aneg \psi \mid \aneg \varphi, \aneg \psi \mid \e$}
\RL{\fns $\aneg_{\tvb}$}
\UIC{$\underbrace{\aneg \varphi, \aneg \psi \mid \aneg \varphi, \aneg \psi \mid \aneg (\varphi \aor \psi)}_{\mathsf{r}10}$}
\DP
\end{math}

\vspace{0.5cm}

\begin{math}
\AXC{\fns Id$_{\varphi}+W_{\bv}+W_\tv$}
\UIC{$\varphi, \varphi \mid \varphi \mid \varphi, \psi$}
\AXC{\fns Id$_{\varphi}+W_{\uv}+W_\tv$}
\UIC{$\varphi \mid \varphi, \psi \mid \varphi, \psi$}
\AXC{\fns Id$_{\psi}+W_\bv+W_\tv$}
\UIC{$\varphi, \psi \mid \psi \mid \varphi, \psi$}
\RL{\fns $\aor_\bvr$}
\TIC{$\varphi \mid \varphi \aor \psi \mid \varphi, \psi$}
\RL{\fns $\aor_\tvb$}
\UIC{$\varphi \mid \varphi \aor \psi \mid \varphi \aor \psi$}
\RL{\fns $\aneg_\bvr$}
\UIC{$\aneg (\varphi \aor \psi), \varphi \mid \varphi \aor \psi \mid \e$}
\RL{\fns $\aneg_{\uvg}$}
\UIC{$\aneg (\varphi \aor \psi), \varphi \mid \aneg (\varphi \aor \psi) \mid \e$}
\RL{\fns $\aneg_{\tvb}$}
\UIC{$\underbrace{\aneg (\varphi \aor \psi) \mid \aneg (\varphi \aor \psi) \mid \aneg \varphi}_{\mathsf{r}13\  (\mathsf{r}17)}$}
\DP
\ \ \ \ \ 
\AXC{\fns Id$_\varphi+W_\tv$}
\UIC{$\varphi \mid \varphi \mid \varphi, \psi$}
\RL{\fns $\aor_\tvb$}
\UIC{$\underbrace{\varphi \mid \varphi \mid \varphi \aor \psi}_{\textrm{r18 (r19)}}$}
\DP
\end{math}

\vspace{0.5cm}

\begin{math}
\hspace{-3cm}
\AXC{\fns Id$_{\varphi}+W_{\bv}+W_\tv$}
\UIC{$\varphi, \varphi \mid \varphi \mid \varphi, \psi$}
\AXC{\fns Id$_{\varphi}+W_{\uv}+W_\tv$}
\UIC{$\varphi \mid \varphi, \psi \mid \varphi, \psi$}
\AXC{\fns Id$_{\psi}+W_\bv+W_\tv$}
\UIC{$\varphi, \psi \mid \psi \mid \varphi, \psi$}
\RL{\fns $\aor_{\uvg}$}
\TIC{$\varphi \mid \varphi \aor \psi \mid \varphi, \psi$}
%
\AXC{\fns Id$_{\psi}+W_{\bv}+W_\tv$}
\UIC{$\psi, \psi \mid \psi \mid \varphi, \psi$}
\AXC{\fns Id$_{\psi}+W_{\uv}+W_\tv$}
\UIC{$\psi \mid \varphi, \psi \mid \varphi, \psi$}
\AXC{\fns Id$_{\varphi}+W_\bv+W_\tv$}
\UIC{$\varphi, \psi \mid \varphi \mid \varphi, \psi$}
\RL{\fns $\aor_{\uvg}$}
\TIC{$\psi \mid \varphi \aor \psi \mid \varphi, \psi$}
%
\RL{\fns $\aor_{\bvr}$}
\BIC{$\underbrace{\varphi \aor \psi \mid \varphi \aor \psi \mid \varphi, \psi}_{\mathsf{r}23}$}
\DP
\end{math}
 }
 
\vspace{0.5cm}

Let us consider the $smc.\textrm{\L{}}3$ rules for $\ararr$:

\vspace{0.5cm}

\begin{math}
\hspace{-4.3cm}
\AXC{$\aneg \varphi$}
\RL{\fns $\mathsf{I}_2^\ararr$}
\UIC{$\varphi \to \psi$} 
\DP
 \ \ \
\AXC{$\psi$}
\RL{\fns $\mathsf{I}_3^\ararr$}
\UIC{$\varphi \to \psi$} 
\DP
 \ \ \
\AXC{$\phantom{\varphi}$} 
\RL{\fns $\mathsf{I}_4^\ararr$}
\UIC{$\varphi \to \psi, \aneg \psi, \varphi$}      
\DP
 \ \ \
\AXC{$\neg\psi$}
\AXC{$\varphi$}
\RL{\fns $\mathsf{I}_6^\ararr$}
\BIC{$\neg(\varphi \to \psi)$}
\DP
 \ \ \
\AXC{$\varphi \ararr \psi$}
\AXC{$\aneg \psi$}
\RL{\fns $\mathsf{E}_{11}^\ararr$}
\BIC{$\neg\varphi$}
\DP
 \ \ \
\AXC{$\neg(\varphi \to \psi)$}      
\RL{\fns $\mathsf{E}_{15}^\ararr$}
\UIC{$\neg\psi$}
\DP
 \ \ \
\AXC{$\neg(\varphi \to \psi)$}
\RL{\fns $\mathsf{E}_{21}^\ararr$}
\UIC{$\varphi$}
\DP
 \ \ \
\AXC{$\varphi$}
\AXC{$\varphi \to \psi$} 
\RL{\fns $\mathsf{E}_{24}^\ararr$}
\BIC{$\psi$}
\DP
\end{math}

\vspace{0.5cm}

We need to show that assuming the translation of the premise(s) of rules for $\ararr$ we can derive the translation of the conclusion(s). Below we simply derive the associated sequent $S({\mathsf{r}^\ararr})$ without performing the cuts afterwards.

\vspace{0.5cm}

{\footnotesize

\begin{math}
\hspace{-3cm}
\AXC{\fns Id$_\varphi+W_{\uv}+W_\tv$}
\UIC{$\varphi \mid \varphi, \varphi \mid \varphi, \psi$}
\AXC{\fns Id$_\varphi+W_{\uv}+W_\tv$}
\UIC{$\varphi \mid \varphi, \psi \mid \varphi, \psi$}
\RL{\fns $\ararr_\tvb$}
\BIC{$\e \mid \varphi \mid \varphi, \varphi \ararr \psi$}
\RL{\fns $\aneg_\bvr$}
\UIC{$\aneg \varphi \mid \varphi \mid \varphi \ararr \psi$}
\RL{\fns $\aneg_{\uvg}$}
\UIC{$\underbrace{\aneg \varphi \mid \aneg \varphi \mid \varphi \ararr \psi}_{\mathsf{r}2}$}
\DP
\ \ \ 
\AXC{\fns Id$_\psi+W_{\bv}+W_{\uv}$}
\UIC{$\varphi, \psi \mid \varphi, \psi \mid \psi$}
\AXC{\fns Id$_\psi+W_{\bv}+W_{\uv}$}
\UIC{$\varphi, \psi \mid \psi, \psi \mid \psi$}
\RL{\fns $\ararr_\tvb$}
\BIC{$\underbrace{\psi \mid \psi \mid \varphi \ararr \psi}_{\mathsf{r}3}$}
\DP
\ \ \ 
\AXC{\fns Id$_\varphi+W_{\bv}+W_\tv$}
\UIC{$\varphi, \psi \mid \varphi \mid \varphi, \psi$}
\AXC{\fns Id$_\psi+W_{\bv}+W_\tv$}
\UIC{$\varphi, \psi \mid \psi \mid \varphi, \psi$}
\RL{\fns $\ararr_\tvb$}
\BIC{$\psi \mid \e \mid \varphi \ararr \psi, \varphi$}
\RL{\fns $\aneg_\bvr$}
\UIC{$\underbrace{\e \mid \e \mid \varphi \ararr \psi, \aneg \psi, \varphi}_{\mathsf{r}4}$}
\DP
\end{math}

\vspace{0.5cm}

\begin{math}
\hspace{-3.3cm}
\AXC{\fns Id$_\varphi+W_{\bv}+W_\tv$}
\UIC{$\varphi \mid \psi, \varphi \mid \psi, \varphi$}
\AXC{\fns Id$_\psi+W_{\bv}+W_{\uv}$}
\UIC{$\psi, \varphi \mid \psi, \varphi \mid \psi$}
\RL{\fns $\ararr_\bvr$}
\BIC{$\varphi \ararr \psi, \varphi \mid \psi, \varphi \mid \e$}
\RL{\fns $\aneg_\bvr$}
\UIC{$\varphi \ararr \psi, \aneg \psi, \varphi \mid \psi, \varphi \mid \e$}
\RL{\fns $\aneg_{\uvg}$}
\UIC{$\varphi \ararr \psi, \aneg \psi, \varphi \mid \aneg \psi, \varphi \mid \e$}
\RL{\fns $\aneg_\tvb$}
\UIC{$\underbrace{\aneg \psi, \varphi \mid \aneg \psi, \varphi \mid \aneg (\varphi \ararr \psi)}_{\mathsf{r}6}$}
\DP
\ \ \ 
\AXC{\fns Id$_\psi + W_\bv + W_{\uv} + W_\tv$}
\UIC{$\varphi, \psi \mid \psi \mid \varphi, \varphi, \psi$}
\AXC{\fns Id$_\psi + W_\bv$}
\UIC{$\psi, \varphi, \psi \mid \psi \mid \psi$}
\RL{\fns $\ararr_\bvr$}
\BIC{$\varphi, \varphi \ararr \psi, \psi \mid \psi \mid \varphi, \psi$}
%
\AXC{\fns Id$_\varphi + W_{\uv} + W_\tv$}
\UIC{$\varphi \mid \varphi, \psi, \psi \mid \varphi, \psi$}
\AXC{\fns Id$_\psi + W_\bv + W_{\uv}$}
\UIC{$\varphi, \psi \mid \varphi, \psi, \psi \mid \psi$}
\RL{\fns $\ararr_\bvr$}
\BIC{$\varphi, \varphi \ararr \psi \mid \varphi, \psi, \psi \mid \psi$}
%
\RL{\fns $\ararr_{\uvg}$}
\BIC{$\varphi, \varphi \ararr \psi \mid \varphi \ararr \psi, \psi \mid \psi$}
\RL{\fns $\aneg_{\bvr}$}
\UIC{$\varphi, \varphi \ararr \psi, \aneg \psi \mid \varphi \ararr \psi, \psi \mid \e$}
\RL{\fns $\aneg_{\uvg}$}
\UIC{$\varphi, \varphi \ararr \psi, \aneg \psi \mid \varphi \ararr \psi, \aneg \psi \mid \e$}
\RL{\fns $\aneg_{\tvb}$}
\UIC{$\underbrace{\varphi \ararr \psi, \aneg \psi \mid \varphi \ararr \psi, \aneg \psi \mid \aneg \varphi}_{\mathsf{r}11}$}
\DP
\end{math}

\vspace{0.5cm}

\begin{math}
\AXC{\fns Id$_\varphi + W_\bv + W_\tv$}
\UIC{$\varphi, \psi, \psi \mid \varphi \mid \varphi, \psi$}
\AXC{\fns Id$_\psi + W_\bv + W_{\uv}$}
\UIC{$\varphi, \psi \mid \varphi, \varphi, \psi \mid \psi$}
\RL{\fns $\ararr_{\uvg}$}
\BIC{$\varphi, \psi \mid \varphi, \varphi \ararr \psi \mid \psi$}
%
\AXC{\fns Id$_\psi + W_\bv + W_\tv$}
\UIC{$\varphi, \psi \mid \varphi, \psi, \psi \mid \psi$}
\AXC{\fns Id$_\psi + W_\bv + W_{\uv}$}
\UIC{$\varphi, \psi \mid \varphi, \psi, \psi \mid \psi$}
\RL{\fns $\ararr_{\uvg}$}
\BIC{$\varphi, \psi \mid \psi, \varphi \ararr \psi \mid \psi$}
%%
\RL{\fns $\ararr_{\tvb}$}
\BIC{$\psi \mid \varphi \ararr \psi \mid \varphi \ararr \psi$}
\RL{\fns $\aneg_{\bvr}$}
\UIC{$\psi, \aneg (\varphi \ararr \psi) \mid \varphi \ararr \psi \mid \e$}
\RL{\fns $\aneg_{\uvg}$}
\UIC{$\psi, \aneg (\varphi \ararr \psi) \mid \aneg (\varphi \ararr \psi) \mid \e$}
\RL{\fns $\aneg_{\tvb}$}
\UIC{$\underbrace{\aneg (\varphi \ararr \psi) \mid \aneg (\varphi \ararr \psi) \mid \aneg \psi}_{\mathsf{r}15}$}
\DP
\end{math}

\begin{math}
\AXC{\fns Id$_\varphi + W_\bv + W_\tv$}
\UIC{$\varphi, \psi \mid \varphi \mid \varphi, \varphi, \psi$}
\AXC{\fns Id$_\varphi + W_{\uv} + W_\tv$}
\UIC{$\varphi \mid \varphi, \varphi, \psi \mid \varphi, \psi$}
\RL{\fns $\ararr_{\uvg}$}
\BIC{$\varphi \mid \varphi, \varphi \ararr \psi \mid \varphi, \psi$}
%
\AXC{\fns Id$_\psi + W_\bv + W_\tv$}
\UIC{$\varphi, \psi \mid \psi \mid \varphi, \varphi, \psi$}
\AXC{\fns Id$_\varphi + W_{\uv} + W_\tv$}
\UIC{$\varphi \mid \varphi, \psi, \psi \mid \varphi, \psi$}
\RL{\fns $\ararr_{\uvg}$}
\BIC{$\varphi \mid \psi, \varphi \ararr \psi \mid \varphi, \psi$}
%%
\RL{\fns $\ararr_{\tvb}$}
\BIC{$\e \mid \varphi \ararr \psi \mid \varphi, \varphi \ararr \psi$}
\RL{\fns $\aneg_{\bvr}$}
\UIC{$\aneg (\varphi \ararr \psi) \mid \varphi \ararr \psi \mid \varphi$}
\RL{\fns $\aneg_{\uvg}$}
\UIC{$\underbrace{\aneg (\varphi \ararr \psi) \mid \aneg (\varphi \ararr \psi) \mid \varphi}_{\mathsf{r}21}$}
\DP
\end{math}

\vspace{0.5cm}

\begin{math}
\AXC{\fns Id$_\varphi + W_\bv + W_\tv$}
\UIC{$\varphi, \psi \mid \varphi \mid \varphi, \psi$}
\AXC{\fns Id$_\varphi + W_\bv + W_\tv$}
\UIC{$\varphi, \psi, \psi \mid \varphi \mid \varphi, \psi$}
\RL{\fns $\ararr_\bvr$}
\BIC{$\varphi, \varphi \ararr \psi, \psi \mid \varphi \mid \varphi, \psi$}
%
\AXC{\fns Id$_\varphi + W_{\uv} + W_\tv$}
\UIC{$\varphi \mid \varphi, \varphi, \psi \mid \varphi, \psi$}
\AXC{\fns Id$_\psi + W_\bv + W_{\uv}$}
\UIC{$\varphi, \psi \mid \varphi, \varphi, \psi \mid \psi$}
\RL{\fns $\ararr_\bvr$}
\BIC{$\varphi, \varphi \ararr \psi \mid \varphi, \varphi, \psi \mid \psi$}
%
\RL{\fns $\ararr_{\uvg}$}
\BIC{$\underbrace{\varphi, \varphi \ararr \psi \mid \varphi, \varphi \ararr \psi \mid \psi}_{\mathsf{r}24}$}
\DP
\end{math}

\vspace{0.5cm}
 }

\end{proof}
 
Therefore, we conclude that:

\begin{corollary}
There exists an effective translation from $smc.\textrm{\L{}}3$-proofs to $s\ell.\textrm{\L{}}3$-proofs.
\end{corollary}
%
\begin{proof}
Immediate from proposition \ref{prop:TranslationL3} and the fact that $s\ell.\textrm{\L{}}3$ has syntactic cut elimination \ref{}. 
\end{proof}



==> QuasiCanonicalSequentCalculi.tex <==
\section{Quasi canonical sequent calculi}
\label{QuasiCanonicalSequentCalculi}

By exploring an adequate negation $\neg$
and the ways in which truth-values may be
characterized, Avron describes some
characterizing sets of sequents, one for each truth-value, to act as
premises and other sets to act as conclusions
(in different rules). Below we describe such sets
in a more compact way, where the sets $\Pi^D_x$
are sets for premises and the sets $\Theta^D_x$
are for conclusions (when $D\subseteq\mathcal{V}$ is the set of designated values and $x \in \mathcal{V}$):

\begin{table}[H]
    \centering
    \begin{tabular}{c|c|c}
        \toprule
         $x$ & $\Pi_x^{\{\tv\}}(p)$ & $\Pi_x^{\{\tv,\uv\}}(p)$\\
         \midrule
         $\bv$ & $\sequent \neg p$ & $p \sequent$\\
         $\uv$& $p \sequent; \neg p \sequent$& $\sequent p; \sequent \neg p$\\
         $\tv$ & $\sequent p$& $\neg p \sequent$\\
         \bottomrule
    \end{tabular}\qquad
    \begin{tabular}{c|c|c}
        \toprule
         $x$ & $\Theta_x^{\{\tv\}}(p)$ & $\Theta_x^{\{\tv,\uv\}}(p)$\\
         \midrule
         $\bv$ & $\sequent \neg p; p \sequent$ & $\sequent \neg p; p \sequent$\\
         $\uv$& $p \sequent; \neg p \sequent$& $\sequent p; \sequent \neg p$\\
         $\tv$ & $\sequent p; \neg p \sequent$& $\sequent p; \neg p \sequent$\\
         \bottomrule
    \end{tabular}
    \caption{Sequents for premises and conclusions.}
\end{table}

We may check (?) that
\begin{equation}
\label{eq:premavron}
v \models \Pi^D_x(\varphi) \; \text{if{f}} \; v(\varphi)=x
\end{equation}
%\begin{equation}
%\label{eq:concavron}
%v \not\models s \text{ for all } s \in \Theta^D_x(\varphi) \text{ iff } v(\varphi) \neq x
%\end{equation}
\begin{equation}
\label{eq:concavron}
\forall y \neq x, \exists S \subseteq \Theta^D_x(\varphi) \text{ such that } v \not\models S \text{ and } v \models \bar S \text{ iff } v(\varphi) = y
\end{equation}

Given a logical matrix $\Mt=\tuple{\{\bv,\uv,\tv\},\cdot_\Mt,D}$ (with $D \in \{\{\tv\},\{\tv,\uv\}\}$) and
an $n$-ary connective $\conn$ in the signature of $\Mt$,
Avron offers the following couple of rules for each tuple $(x_1,\ldots,x_n) \in \mathcal{V}^n$:

\[
\frac{
\bigcup_i \Pi_{x_i}^D(p_i)
}{
s_1
}
\quad
\frac{
\bigcup_i \Pi_{x_i}^D(p_i)
}{
s_2
},
\]
where $\Theta_{\Tilde\conn(x_1,\ldots,x_n)}^D=\{s_1,s_2\}$
and $p_1,\ldots,p_n$ are distinct propositional variables.
The collection of all such rules plus the structural rules
gives an axiomatization for $\Mt$.

Below we provide a couple of Set-Set rules
that are equivalent to the pair of rules above:

\[
\frac{
\bigcup_i \Omega_{x_i}^D(p_i),
\Omega_{y_1}^D(\conn(\varphi_1,\ldots,\varphi_n))
}{
\bigcup_i \mho_{x_i}^D(p_i),
\mho_{y_1}^D(\conn(\varphi_1,\ldots,\varphi_n))
}\quad
\frac{
\bigcup_i \Omega_{x_i}^D(p_i),
\Omega_{y_2}^D(\conn(\varphi_1,\ldots,\varphi_n))
}{
\bigcup_i \mho_{x_i}^D(p_i),
\mho_{y_2}^D(\conn(\varphi_1,\ldots,\varphi_n))
},
\]
where $\mathcal{V}\setminus{}\{x\} = \{y_1,y_2\}$.

In order to see the equivalence, let us work contrapositively.

\sloppy Suppose that $v[\bigcup_i \Omega_{x_i}^D(p_i) \cup
\Omega_{y_1}^D(\conn(\varphi_1,\ldots,\varphi_n))] \subseteq D$ while $v[\bigcup_i \mho_{x_i}^D(p_i) \cup
\mho_{y_1}^D(\conn(\varphi_1,\ldots,\varphi_n))] \subseteq \bar D$. Then $v(p_i) = x_i$ and $v(\conn(\varphi_1,\ldots,\varphi_n))) = y_1 \neq x$.
Then, by properties  $\ref{eq:premavron}$ and $\ref{eq:concavron}$,
some of the rules given by Avron fails under $v$.
The case of $y_2$ is analogous.

Suppose now that $v \models \bigcup_i \Pi_{x_i}^D(p_i)$;
then, $v(p_i) = x_i$ for each $1 \leq i \leq n$,
and hence $v[\bigcup_i \Omega_{x_i}^D(p_i)] \subseteq D$ and 
$v[\bigcup_i \mho_{x_i}^D(p_i)] \subseteq \bar D$.
By checking each of the following cases
\begin{itemize}
    \item $v \not\models s_1$, $v \not\models s_2$
    \item $v \models s_1$, $v \not\models s_2$
    \item $v \not\models s_1$, $v \models s_2$
\end{itemize}
we have that in exactly two of them
(the remainder is absurd),
we have $v(\conn(\varphi_1,\ldots,\varphi_n)) = y \neq x$,
and so
$v[\Omega_{y}^D(\conn(\varphi_1,\ldots,\varphi_n))] \subseteq D$ and 
$v[\mho_{y}^D(\conn(\varphi_1,\ldots,\varphi_n))] \subseteq \bar D$,
that is, one of the proposed Set-Set rules does not hold,
as desired.

\begin{example}
If we have $\tv \supset \bv = \bv$ and $\neg$ interpreted
as Kleene's negation, the rules according to
Avron are

\begin{center}
\begin{tabular}{cc}
\def\fCenter{\mbox{$\ \Rightarrow \ $}}
\AXC{$\Gamma \fCenter p$}
\AXC{$\Gamma' \fCenter \neg q$}
\BIC{$\Gamma, \Gamma' \fCenter \neg (p \ararr q)$}
\DP
 & 
\def\fCenter{\mbox{$\ \Rightarrow \ $}}
\AXC{$\Gamma \fCenter p$}
\AXC{$\Gamma' \fCenter \neg q$}
\BIC{$\Gamma, \Gamma', p \ararr q \fCenter $}
\DP
 \\
\end{tabular}
\end{center}
%
%\[
%\frac{\sequent p \quad \sequent \neg q}{\sequent \neg(p \supset q)} \quad
%\frac{\sequent p \quad \sequent \neg q}{p \supset q \sequent}
%\]
which are equivalent to the pair of Set-Set rules
\[
\frac{p, \neg q, p \supset q}{\neg p, q, \neg(p \supset q)}
\quad
\frac{p, \neg q, p \supset q, \neg(p \supset q)}{\neg p, q}
\]

\end{example}

%\input{set-set-calculi/l3}
%\input{set-set-calculi/sk}
%\input{set-set-calculi/lp}
%\input{set-set-calculi/bk}
%\input{set-set-calculi/pwk}
%\input{set-set-calculi/s3}
%\input{set-set-calculi/g3}
%\input{set-set-calculi/j3}
%\input{set-set-calculi/M7}


%\subsubsection{\L ukasiewicz}
%
%$D = \{\tv\}$
%
%\begin{table}[H]
%    \centering
%    \begin{tabular}{c|ccc}
%        \toprule
%         \lukConj & \bv & \uv & \tv\\
%        \midrule
%         \bv & \bv & \bv & \bv\\
%         \uv & \bv & \uv & \uv \\
%         \tv & \bv & \uv & \tv\\
%        \bottomrule
%    \end{tabular}
%    \quad
%    \begin{tabular}{c|ccc}
%        \toprule
%         \lukDisj & \bv & \uv & \tv\\
%        \midrule
%         \bv & \bv & \uv & \tv\\
%         \uv & \uv & \uv & \tv \\
%         \tv & \tv & \tv & \tv\\
%        \bottomrule
%    \end{tabular}
%    \quad 
%    \begin{tabular}{c|ccc}
%        \toprule
%         \lukImp & \bv & \uv & \tv\\
%        \midrule
%         \bv & \tv & \tv & \tv\\
%         \uv & \uv & \tv & \tv\\
%         \tv & \bv & \uv & \tv\\
%        \bottomrule
%    \end{tabular}
%    \quad 
%    \begin{tabular}{c|c}
%        \toprule
%         & \lukNeg \\
%         \midrule
%         \bv & \tv\\
%         \uv & \uv\\
%         \tv & \bv\\
%         \bottomrule
%    \end{tabular}
%\end{table}
%
%\subsubsection{Strong Kleene}
%
%$D = \{\tv\}$
%
%\begin{table}[H]
%    \centering
%    \begin{tabular}{c|ccc}
%        \toprule
%         \KleeConj & \bv & \uv & \tv\\
%        \midrule
%         \bv & \bv & \bv & \bv\\
%         \uv & \bv & \uv & \uv \\
%         \tv & \bv & \uv & \tv\\
%        \bottomrule
%    \end{tabular}
%    \quad
%    \begin{tabular}{c|ccc}
%        \toprule
%         \KleeDisj & \bv & \uv & \tv\\
%        \midrule
%         \bv & \bv & \uv & \tv\\
%         \uv & \uv & \uv & \tv \\
%         \tv & \tv & \tv & \tv\\
%        \bottomrule
%    \end{tabular}
%    \quad 
%    \begin{tabular}{c|ccc}
%        \toprule
%         \KleeImp & \bv & \uv & \tv\\
%        \midrule
%         \bv & \tv & \tv & \tv\\
%         \uv & \uv & \uv & \tv\\
%         \tv & \bv & \uv & \tv\\
%        \bottomrule
%    \end{tabular}
%    \quad 
%    \begin{tabular}{c|c}
%        \toprule
%         & \KleeNeg \\
%         \midrule
%         \bv & \tv\\
%         \uv & \uv\\
%         \tv & \bv\\
%         \bottomrule
%    \end{tabular}
%\end{table}
%
%\subsubsection{Priest}
%
%Same as Strong Kleene,
%but with $D=\{\tv,\uv\}$.
%
%\subsubsection{Bochvar-Kleene}
%
%$D = \{\tv\}$?
%
%\begin{table}[H]
%    \centering
%    \begin{tabular}{c|ccc}
%        \toprule
%         \BKleeConj & \bv & \uv & \tv\\
%        \midrule
%         \bv & \bv & \uv & \bv\\
%         \uv & \uv & \uv & \uv \\
%         \tv & \bv & \uv & \tv\\
%        \bottomrule
%    \end{tabular}
%    \quad
%    \begin{tabular}{c|ccc}
%        \toprule
%         \BKleeDisj & \bv & \uv & \tv\\
%        \midrule
%         \bv & \bv & \uv & \tv\\
%         \uv & \uv & \uv & \uv \\
%         \tv & \tv & \uv & \tv\\
%        \bottomrule
%    \end{tabular}
%    \quad 
%    \begin{tabular}{c|ccc}
%        \toprule
%         \BKleeImp & \bv & \uv & \tv\\
%        \midrule
%         \bv & \tv & \uv & \tv\\
%         \uv & \uv & \uv & \uv\\
%         \tv & \bv & \uv & \tv\\
%        \bottomrule
%    \end{tabular}
%    \quad 
%    \begin{tabular}{c|c}
%        \toprule
%         & \BKleeNeg \\
%         \midrule
%         \bv & \tv\\
%         \uv & \uv\\
%         \tv & \bv\\
%         \bottomrule
%    \end{tabular}
%\end{table}
%
%\subsubsection{Sobociński}
%
%$D=\{\tv,\uv\}$
%
%\begin{table}[H]
%    \centering
%    \begin{tabular}{c|ccc}
%        \toprule
%         \SobocConj & \bv & \uv & \tv\\
%        \midrule
%         \bv & \bv & \bv & \bv\\
%         \uv & \bv & \uv & \tv \\
%         \tv & \bv & \tv & \tv\\
%        \bottomrule
%    \end{tabular}
%    \quad
%    \begin{tabular}{c|ccc}
%        \toprule
%         \SobocDisj & \bv & \uv & \tv\\
%        \midrule
%         \bv & \bv & \bv & \tv\\
%         \uv & \bv & \uv & \tv \\
%         \tv & \tv & \tv & \tv\\
%        \bottomrule
%    \end{tabular}
%    \quad 
%    \begin{tabular}{c|ccc}
%        \toprule
%         \SobocImp & \bv & \uv & \tv\\
%        \midrule
%         \bv & \tv & \uv & \tv\\
%         \uv & \bv & \tv & \tv\\
%         \tv & \bv & \uv & \tv\\
%        \bottomrule
%    \end{tabular}
%    \quad 
%    \begin{tabular}{c|c}
%        \toprule
%         & \SobocNeg \\
%         \midrule
%         \bv & \tv\\
%         \uv & \uv\\
%         \tv & \bv\\
%         \bottomrule
%    \end{tabular}
%\end{table}
%
%\subsubsection{D'Ottaviano's J3}
%
%Conjunction, disjunction
%and negation as in
%Strong Kleene, with $D=\{\tv,\uv\}$,
%plus the following:
%
%\begin{table}[H]
%    \centering
%    \begin{tabular}{c|ccc}
%        \toprule
%         \JThreeImp & \bv & \uv & \tv\\
%        \midrule
%         \bv & \tv & \uv & \tv\\
%         \uv & \bv & \tv & \tv\\
%         \tv & \bv & \uv & \tv\\
%        \bottomrule
%    \end{tabular}
%    \quad
%    \begin{tabular}{c|c}
%        \toprule
%         & \lukPoss \\
%         \midrule
%         \bv & \tv\\
%         \uv & \tv\\
%         \tv & \bv\\
%         \bottomrule
%    \end{tabular}    
%\end{table}
%
%\subsubsection{G\"odel}
%
%From Strong Kleene,
%by changing negation and
%implication to the following ones:
%
%\begin{table}[H]
%    \centering
%    \begin{tabular}{c|ccc}
%        \toprule
%         \HImp & \bv & \uv & \tv\\
%        \midrule
%         \bv & \tv & \tv & \tv\\
%         \uv & \bv & \tv & \tv\\
%         \tv & \bv & \uv & \tv\\
%        \bottomrule
%    \end{tabular}
%    \quad 
%    \begin{tabular}{c|c}
%        \toprule
%         & \HNeg \\
%         \midrule
%         \bv & \tv\\
%         \uv & \bv\\
%         \tv & \bv\\
%         \bottomrule
%    \end{tabular}
%\end{table}
%
%\subsubsection{Weak Kleene}

==> SomeNonMonadicCases.tex <==
\section{Some non-monadic cases}
\label{SomeNonMonadicCases}

\subsection{Disjunctive fragment of Bochvar-Kleene's logic}

Let $\SetSetCR_{BK}^{\lor}$ be the \SetSet{} logic induced by
the three-valued logical matrix $\MatA_{BK}^\lor$ whose signature contains only $\lor$, interpreted as $\BKleeDisj$ in this case --- the truth-table of which we 
repeat below for convenience --- and whose set
of designated values is $\{\tv\}$. The reader can easily verify
that this matrix is not monadic by using the fact that the sets $\{\bv\}$ and 
$\{\uv\}$ are both closed under $\BKleeDisj$. Although our previous
recipe does not apply in this scenario, we are still able
to provide an analytic axiomatization for this matrix.

\begin{table}[H]
    \centering
    \begin{tabular}{c|ccc}
        \toprule
         \BKleeDisj & \bv & \uv & \tv\\
        \midrule
         \bv & \bv & \uv & \tv\\
         \uv & \uv & \uv & \uv \\
         \tv & \tv & \uv & \tv\\
        \bottomrule
    \end{tabular}
\end{table}

\begin{definition}
Let $\CalcA^\lor_{BK}$ be the multiple-conclusion calculus 
whose rule schemas are the following:
%(cut:r11,(cut:r13,r15)) (sub):=[ (p1 or p2) or q1,q1 | p1 or q1 ]
%(cut:r9,(cut:r3,r15)) (sub):=[ (p1 or p2) or q1,q1 | p2 or q1 ]
\begin{gather*}
    \MCRule{\PropA \lor \PropB}{\PropA,\PropB}\RuleA^{\lor,1}_{BK}
    \quad
    \MCRule{\PropA,\PropB}{\PropA \lor \PropB}\RuleA^{\lor,2}_{BK}\\
    \MCRule{\PropA_1\lor\PropB_1, \PropA_2}{\PropA_1\lor\PropA_2}\RuleA^{\lor,3}_{BK}
    \quad
    \MCRule{\PropA_2\lor\PropB_1, \PropA_1}{\PropA_1\lor\PropA_2}\RuleA^{\lor,4}_{BK}
    \quad
    \MCRule{\PropA_1\lor\PropA_2,\PropB_1}{\PropA_2\lor\PropB_1}\RuleA^{\lor,5}_{BK}\\
    \MCRule{\PropA_1\lor\PropB_1,\PropA_2\lor\PropB_1}{(\PropA_1\lor\PropA_2)\lor\PropB_1,\PropA_1}\RuleA^{\lor,6}_{BK}
    \quad
    \MCRule{(\PropA_1\lor\PropA_2)\lor\PropB_1,\PropB_1}{\PropA_1\lor\PropB_1}\RuleA^{\lor,7}_{BK}
    \quad
    \MCRule{(\PropA_1\lor\PropA_2)\lor\PropB_1,\PropB_1}{\PropA_2\lor\PropB_1}\RuleA^{\lor,8}_{BK}
\end{gather*}
\end{definition}

\begin{theorem}
$\CalcA^\lor_{BK}$ is sound for $\MatA_{BK}^\lor$.
\end{theorem}
\begin{proof}
This is routine.
\end{proof}

\begin{lemma}
Some derivable rules:
\[
    \MCRule{\PropA_1\lor\PropA_2,\PropB_1}{\PropA_1\lor\PropB_1}\RuleA^{\lor,9}_{BK}\\
    \quad
    \MCRule{\PropA_1\lor\PropA_2}{\PropA_2\lor\PropA_1}\RuleA^{\lor,10}_{BK}\\
\]
\end{lemma}

\begin{theorem}
$\CalcA^\lor_{BK}$ is complete for $\MatA_{BK}^\lor$
and $\{\PropA \lor \PropB\}$-analytic.
\end{theorem}
\begin{proof}
Let $\AnalyticSetA \SymbDef \{\PropA \lor \PropB\}$.
Suppose that $\FmSetA \NAnaSetSetCR{\CalcA^\lor_{BK}}{\AnalyticSetA} \FmSetB$,
then, by cut for sets, there is $\SetCut \subseteq \LangSetA$
such that
$\SetCut \NAnaSetSetCR{\CalcA^\lor_{BK}}{\AnalyticSetA} \FmSetComp\SetCut$,
with $\FmSetA \subseteq \SetCut$ and $\FmSetB \subseteq \FmSetComp\SetCut$.
Let $\GenSubs{\AnalyticSetA} \SymbDef \Subf{\FmSetA \cup \FmSetB} \cup \{\FmA \lor \FmB \mid \FmA,\FmB \in \Subf{\FmSetA \cup \FmSetB}\}$.
Then $\TPart \NAnaSetSetCR{\CalcA^\lor_{BK}}{\AnalyticSetA} \FPart$
for some partition $(\TPart, \FPart)$ of $\GenSubs{\AnalyticSetA}$,
with $\FmSetA \subseteq \TPart$ and $\FmSetB \subseteq \FPart$.
We consider two cases, defining
for each of them a mapping 
$v : \Subf{\FmSetA\cup\FmSetB}\to\ThreeValuesSet$
and proving that $v(\FmA\lor\FmB) = v(\FmA) \BKleeDisj v(\FmB)$:
\begin{itemize}
    \item for all $\FmA,\FmB$, (a): if $\FmA \in \TPart \cap \Subf{\FmSetA\cup\FmSetB}$
    and $\FmB \in \FPart \cap \Subf{\FmSetA\cup\FmSetB}$,
    then $\FmA\lor\FmB \in \TPart$: let $v : \Subf{\FmSetA\cup\FmSetB}\to\ThreeValuesSet$ such that
    \[
        v(\FmA) \SymbDef
        \begin{cases}
            \tv & \text{ if } \FmA \in \TPart\\
            \bv & \text{ if } \FmA \in \FPart\\
        \end{cases}
    \]
    \begin{itemize}
        \item if $v(\FmA\lor\FmB)=\tv$,
        then, by $(\RuleA^{\lor,1}_{BK})$, either
        $v(\FmA)=\tv$ or $v(\FmB)=\tv$, and we are done,
        as the range of $v$ is $\{\tv,\bv\}$;
        \item if $v(\FmA)=\tv$, in case $v(\FmB)=\tv$, use $(\RuleA^{\lor,2}_{BK})$, and in case
        $v(\FmB)=\bv$, use the assumption (a).
        The argument is analogous for $v(\FmB)=\tv$, with
        the help of $(\RuleA^{\lor,10}_{BK})$;
        \item if $v(\FmA\lor\FmB)=\bv$, 
        use the contrapositive of (a),
        which gives us that either $\FmA \in \FPart$ 
        or $\FmB \in \TPart$. In the first case, assume
        that $\FmB \in \TPart$, then, by (a),
        $\FmB \lor \FmA \in \TPart$, but 
        by $(\RuleA^{\lor,10}_{BK})$ we would have 
        $\FmB\lor\FmA \in \FPart$, thus we have an absurd and $\FmB \in \FPart$.
        In the second case, if $\FmB \in \TPart$,
        by $(\RuleA^{\lor,2}_{BK})$, we would have
        $\FmA \in \FPart$, and the latter
        reasoning applies again;
        %use the contrapositive
        %of the assumption and $(\RuleA^{\lor,10}_{BK})$
        \item if $v(\FmA)=\bv$ and $v(\FmB)=\bv$, by
        $(\RuleA^{\lor,1}_{BK})$ we have $\FmA\lor\FmB \in \FPart$.
    \end{itemize}
%    In case $v(\FmA\lor\FmB) = \tv$, by rule (1), we must
%    have at least one of $\FmA$ and $\FmB$ in $\TPart$,
%    meaning that $v(\FmA\lor\FmB) = v(\FmA) \BKleeDisj v(\FmB)$.
%    In case $v(\FmA\lor\FmB) = \bv$, we have
%    $\FmA\lor\FmB \in \FPart$, and thus either
%    $\FmA \not\in \TPart \cap \Subf{\FmSetA\cup\FmSetB}$
%    or $\FmB \not\in \FPart \cap \Subf{\FmSetA\cup\FmSetB}$.
    \item for some $\FmB_{\tv} \in \TPart \cap \Subf{\FmSetA\cup\FmSetB}$
    and $\FmB_{\uv} \in \FPart \cap \Subf{\FmSetA\cup\FmSetB}$,
    we have $\FmB_{\tv}\lor\FmB_{\uv} \in \FPart$:  
     let $v : \Subf{\FmSetA\cup\FmSetB}\to\ThreeValuesSet$ such that
     \[
        v(\FmA) \SymbDef
        \begin{cases}
            \tv & \text{ if } \FmA \in \TPart\\
            \uv & \text{ if } \FmA, \FmA\lor\FmB_\tv \in \FPart\\
            \bv & \text{ if } \FmA\in\FPart, \FmA\lor\FmB_\tv \in \TPart\\
        \end{cases}
    \]    
    \begin{itemize}
        \item if $v(\FmA \lor \FmB) = \uv$,
        then $\FmA\lor\FmB, (\FmA\lor\FmB)\lor\FmB_\tv \in \FPart$.
        By (1), either $\FmA \in \FPart$
        or $\FmB \in \FPart$. In the first
        case, by (6), we have
        $\FmA\lor\FmB_\tv \in \FPart$
        or $\FmB\lor\FmB_\tv \in \FPart$.
        The former entails that
        $v(\FmA)=\uv$, while the latter, by
        (5), gives that $\FmB\lor\FmB \in \FPart$,
        which, by rule (1), gives $\FmB\in\FPart$,
        and thus $v(\FmB)=\uv$.
        In the second case, with $\FmB\in\FPart$,
        by rule (3), $\FmA\lor\FmB_\tv \in \FPart$.
        As $\FmB_\tv \in \TPart$,
        by rule (2) we have $\FmA \in \FPart$,
        and then $v(\FmA)=\uv$, as desired;
        \item if $v(\FmA) = \uv$, then
        $\FmA, \FmA\lor\FmB_\tv \in \FPart$, and, by rule (9), we have $\FmA\lor\FmB\in\FPart$; hence, by rule (7), we obtain $(\FmA\lor\FmB)\lor\FmB_\tv\in\FPart$, thus $v(\FmA\lor\FmB)=\uv$. The case $v(\FmB)=\uv$ is analogous, using
        rules (5) and (8) instead;
        \item if $v(\FmA\lor\FmB)=\bv$, 
        then $\FmA\lor\FmB\in\FPart$ and $(\FmA\lor\FmB)\lor\FmB_\tv \in \TPart$.
        By (7) and (8), $\FmA\lor\FmB_\tv \in \TPart$ and $\FmB\lor\FmB_\tv \in \TPart$
        respectively.
        By (3) and (4), then, we have
        $v(\FmB)=\bv$ and $v(\FmA)=\bv$,
        as desired;
        %use 7, 8, 3 and 4
        \item if $v(\FmA) = \bv$ and $v(\FmB)=\bv$, then $\FmA,\FmB\in\FPart$ and
        $\FmA\lor\FmB_\tv,\FmB\lor\FmB_\tv \in \TPart$. By (1), we have $\FmA\lor\FmB\in\FPart$,
        and, by (6), we get $(\FmA\lor\FmB)\lor\FmB_\tv \in \TPart$,
        entailing that $v(\FmA\lor\FmB)=\bv$;
        \item if $v(\FmA\lor\FmB)=\tv$,
        by (9) and (5), we have $\FmA\lor\FmB_\tv \in \FPart$ and $\FmB\lor\FmB_\tv \in \FPart$, thus $v(\FmA) \neq \uv$
        and $v(\FmB)\neq\uv$.
        Then, by (1), we have $\FmA\in \TPart$
        or $\FmB\in\TPart$, and hence,
        in either case, $v(\FmA\lor\FmB)=v(\FmA)\BKleeDisj v(\FmB)$;
        \item if $v(\FmA) = \tv$ and $v(\FmB) \neq \uv$, we have $\FmA \in \TPart$ and either $\FmB \in \TPart$
        or $\FmB\lor\FmB_\tv \in \FPart$.
        In the first case, by (2), we get
        $\FmA\lor\FmB \in \TPart$,
        and, in the second, by (4), 
        we have also $\FmA\lor\FmB \in \TPart$,
        and we are done.
        The case $v(\FmB) = \tv$ and $v(\FmA) \neq \uv$ is analogous.
    \end{itemize}
\end{itemize}
\end{proof}

\subsection{Implicative fragment of \L ukaziewicz's logic}

\[
    \begin{tabular}{c|ccc}
        \toprule
         \lukImp & \bv & \uv & \tv\\
        \midrule
         \bv & \tv & \tv & \tv\\
         \uv & \uv & \tv & \tv\\
         \tv & \bv & \uv & \tv\\
        \bottomrule
    \end{tabular}
\]

\begin{definition}
Let $\CalcA^\to_{\LThreeName}$ be the multiple-conclusion calculus 
whose rule schemas are the following:
\begin{gather*}
    \MCRule{\PropB}{\PropA\to\PropB}(\RuleA_{\LThreeName}^{1,\to})
    \quad
    \MCRule{\PropA_1\to\PropA_2, \PropA_1}{\PropA_2}(\RuleA_{\LThreeName}^{2,\to})\quad
    \MCRule{(\PropA_1 \to \PropA_2) \to \PropB_0}{\PropA_2 \to \PropB_0}(\RuleA_{\LThreeName}^{3,\to})\quad
    \MCRule{\PropA_2 \to \PropB_0, \PropA_1}{(\PropA_1\to\PropA_2)\to\PropB_0}(\RuleA_{\LThreeName}^{4,\to})
    \\
    \MCRule{\PropA_1 \to \PropA_2, \PropA_2 \to \PropB_0}{\PropA_1 \to \PropB_0}(\RuleA_{\LThreeName}^{5,\to})\quad
    \MCRule{(\PropA_1 \to \PropA_2) \to \PropB_0, \PropA_2 \to \PropB_0}{\PropA_1 \to \PropB_0, \PropA_1}(\RuleA_{\LThreeName}^{6,\to})\\
    \MCRule{\PropA_1 \to \PropB_0}{\PropA_1\to\PropA_2,\PropB_{\half} \to \PropB_0, \PropB_\half}(\RuleA_{\LThreeName}^{7,\to})\quad
    \MCRule{}{\PropA_1 \to \PropA_2, \PropA_2 \to \PropB_0, \PropA_1}(\RuleA_{\LThreeName}^{8,\to})\\
\end{gather*}
\end{definition}

\begin{theorem}
$\CalcA^\to_{\LThreeName}$ is sound for $\MatA_{\LThreeName}^\to$.
\end{theorem}
\begin{proof}
This is routine.
\end{proof}
\begin{theorem}
\label{the:lukimpcomp}
$\CalcA^\to_{\LThreeName}$ is complete for $\MatA_{\LThreeName}^\to$
and $\{\PropA \to \PropB\}$-analytic.
\end{theorem}
\begin{proof}
Let $\AnalyticSetA \SymbDef \{\PropA \to \PropB\}$.
Suppose that $\FmSetA \NAnaSetSetCR{\CalcA^\to_{\LThreeName}}{\AnalyticSetA} \FmSetB$,
then, by cut for sets, there is $\SetCut \subseteq \LangSetA$
such that
$\SetCut \NAnaSetSetCR{\CalcA^\to_{\LThreeName}}{\AnalyticSetA} \FmSetComp\SetCut$,
with $\FmSetA \subseteq \SetCut$ and $\FmSetB \subseteq \FmSetComp\SetCut$.
Let $\GenSubs{\AnalyticSetA} \SymbDef \Subf{\FmSetA \cup \FmSetB} \cup \{\FmA \to \FmB \mid \FmA,\FmB \in \Subf{\FmSetA \cup \FmSetB}\}$.
Then $\TPart \NAnaSetSetCR{\CalcA^\to_{\LThreeName}}{\AnalyticSetA} \FPart$
for some partition $(\TPart, \FPart)$ of $\GenSubs{\AnalyticSetA}$,
with $\FmSetA \subseteq \TPart$ and $\FmSetB \subseteq \FPart$.
We consider two cases, defining
for each of them a mapping 
$v : \Subf{\FmSetA\cup\FmSetB}\to\ThreeValuesSet$
and proving that $v(\FmA\to\FmB) = v(\FmA) \lukImp v(\FmB)$:
\begin{itemize}
    \item for every (a): $\FmA,\FmB \in \FPart \cap \Subf{\FmSetA\cup\FmSetB}$, we have
    $\FmA \to \FmB \in \TPart$:
    let $v : \Subf{\FmSetA\cup\FmSetB}\to\ThreeValuesSet$ such that
    \[
        v(\FmA) \SymbDef
        \begin{cases}
            \tv & \text{ if } \FmA \in \TPart\\
            \bv & \text{ if } \FmA \in \FPart\\
        \end{cases}
    \]
    \begin{itemize}
        \item if $v(\FmA) = \tv$ and $v(\FmB)=\bv$: 
        by rule $(\RuleA_{\LThreeName}^{2,\to})$, we
        must have $\FmA \to \FmB \in \FPart$, that is,
        $v(\FmA\to\FmB)=\bv$;
        \item if $v(\FmA\to\FmB)=\bv$:
        by $(\RuleA_{\LThreeName}^{1,\to})$, we have
        $\FmB \in \FPart$ and, by (a), we must have
        $\FmA \in \TPart$;
        \item if $v(\FmA) = \bv$: by (8), we have
        that (b): $\FmA\to\FmB \in \TPart$ or 
        (c): $\FmB\to\FmA \in \TPart$.
        Case (b), we are done. Case (c), by $(\RuleA_{\LThreeName}^{2,\to})$,
        we have $\FmB \in \FPart$,
        and then, by (a), we have $\FmA\to\FmB \in \TPart
        $;
        \item if $v(\FmB) = \tv$: by rule $(\RuleA_{\LThreeName}^{1,\to})$, we
        must have $\FmA \to \FmB \in \TPart$;
        \item if $v(\FmA\to\FmB) = \tv$:
        by $(\RuleA_{\LThreeName}^{2,\to})$, we must have
        either $\FmA \in \FPart$ or $\FmB \in \TPart$.
    \end{itemize}
    \item there are $\FmA_{\uv}, \FmB_{\bv} \in \FPart\cap\Subf{\FmSetA\cup\FmSetB}$ with
    $\FmA_{\uv} \to \FmB_{\bv} \in \FPart$: let $v : \Subf{\FmSetA\cup\FmSetB}\to\ThreeValuesSet$ such that
    \[
        v(\FmA) \SymbDef
        \begin{cases}
            \tv & \text{ if } \FmA \in \TPart\\
            \uv & \text{ if } \FmA, \FmA\to\FmB_\bv \in \FPart\\
            \bv & \text{ if } \FmA \in \FPart, \FmA\to\FmB_\bv \in \TPart\\
        \end{cases}
    \]
    \begin{itemize}
        \item if $v(\FmA) = \tv$ and $v(\FmB)=\bv$: 
        we have $\FmB \in \FPart, \FmB \to \FmB_\bv \in \TPart$,
        then, by (4), we have
        $(\FmA \to \FmB)\to\FmB_\bv \in \TPart$,
        and, by (1), $\FmA \to \FmB \in \FPart$,
        thus $v(\FmA\to\FmB) = \bv$;
        \item if $v(\FmA\to\FmB)=\bv$: by (3),
        we have $\FmB \to \FmB_\bv \in \TPart$
        and by (2), we have $\FmB \in \FPart$, thus
        $v(\FmB)=\bv$; by (6), we have either
        $\FmA \in \TPart$ or $\FmA \to \FmB_\bv \in \TPart$.
        In the first case, we are done; the second
        case leads to an absurd, by (7),
        since $\FmA_{\uv} \to \FmB_{\bv}, \FmB_{\bv} \in \FPart$;
        \item if $v(\FmA) = \bv$: by rule (8),
        we have either $\FmA\to\FmB \in \TPart$
        or $\FmB\to\FmB_{\uv} \in \TPart$.
        In the first case, we are done.
        In the second, we must have $\FmA\to\FmB \in \TPart$
        by rule (7);
        \item if $v(\FmB) = \tv$: by rule (1), we have
        $\FmA\to\FmB \in \TPart$;
        \item if $v(\FmA\to\FmB) = \tv$: then $\FmA\to\FmB \in \TPart$. By (2), we have either (b): $\FmA \in \FPart$
        or (c): $\FmB \in \TPart$. In case (b), by (5), we have either
        (d): $\FmA\to\FmB_{\bv} \in \TPart$ or
        (e): $\FmB\to\FmB_{\bv} \in \FPart$.
        Case (d), we have $v(\FmA) = \bv$, as desired.
        Case (e), if $\FmB \in \TPart$, we are done,
        and if $\FmB \in \FPart$, we will have $v(\FmB)=\uv$,
        and we are also done.
        Case (c), that is, $\FmB \in \TPart$, $v(\FmB)=\tv$ and we are done;
        \item if $v(\FmA\to\FmB) = \uv$: then
        $\FmA\to\FmB,(\FmA\to\FmB)\to\FmB_\bv \in \FPart$.
        Then, by (4), either (b): $\FmA \in \FPart$ or
        (c): $\FmB\to\FmB_\bv \in \FPart$.
        Case (b), by (8), we have $\FmB\to\FmB_\bv \in \TPart$,
        and, by (2), we have $\FmB\in\FPart$, meaning
        that $v(\FmB)=\bv$. Moreover, by (7), we have $\FmA\to\FmB_\bv\in\FPart$, hence $v(\FmA)=\uv$,
        as desired.
        Case (c), by (8) we have $\FmA \in \TPart$, i.e. $v(\FmA)=\tv$.
        Also, by (1) and the fact that $\FmA\to\FmB \in \FPart$, we
        have $\FmB \in \FPart$, and then $v(\FmB)=\uv$, as desired;
        \item if $v(\FmA) = \uv$ and $v(\FmB)=\bv$:     then
        $\FmA,\FmA\to\FmB_\bv \in \FPart$
        and $\FmB \in \FPart$ and $\FmB\to\FmB_\bv \in \TPart$.
        By (5), we have $\FmA\to\FmB \in \FPart$, and, 
        by (6), we have $(\FmA\to\FmB)\to\FmB_\bv \in \FPart$,
        we have $v(\FmA\to\FmB)=\uv$.
        \item if $v(\FmA) = \tv$ and $v(\FmB)=\uv$:
        then $\FmA \in \TPart$, $\FmB \in \FPart$
        and $\FmB\to\FmB_\bv \in \TPart$. By (4),
        we have $(\FmA\to\FmB)\to\FmB_\bv \in \FPart$,
        and, by (1), we have $\FmA\to\FmB \in \FPart$,
        thus $v(\FmA\to\FmB)=\uv$.
    \end{itemize}
\end{itemize}
\end{proof}

\subsection{Implicative fragment of G\"odel's logic}

\[
    \begin{tabular}{c|ccc}
        \toprule
             \HImp & \bv & \uv & \tv\\
        \midrule
         \bv & \tv & \tv & \tv\\
         \uv & \bv & \tv & \tv\\
         \tv & \bv & \uv & \tv\\
        \bottomrule
    \end{tabular}
\]

\begin{definition}
Let $\CalcA^\to_{\GThreeName}$ be the multiple-conclusion calculus 
whose rule schemas are the same as those of $\CalcA^\to_{\LThreeName}$,
except that we replace $(\RuleA_{\LThreeName}^{6,\to})$
by the following:
\begin{gather*}
\MCRule{\PropA_2 \to \PropB_0}{(\PropA_1\to\PropA_2)\to\PropB_0, \PropA_1\to\PropB_0}(\RuleA_{\GThreeName}^{6,\to})
\end{gather*}
\end{definition}

\begin{theorem}
$\CalcA^\to_{\GThreeName}$ is sound for $\MatA_{\GThreeName}^\to$.
\end{theorem}
\begin{proof}
This is routine.
\end{proof}
\begin{theorem}
$\CalcA^\to_{\GThreeName}$ is complete for $\MatA_{\GThreeName}^\to$
and $\{\PropA \to \PropB\}$-analytic.
\end{theorem}
\begin{proof}
The proof is very similar to the one of Theorem~\ref{the:lukimpcomp},
di{f}fering only in some sub-cases of the of of second item:
\begin{itemize}
    \item if $v(\FmA\to\FmB)=\bv$: then 
    $\FmA\to\FmB \in \FPart$
    and $(\FmA\to\FmB)\to\FmB_\bv \in \TPart$.
    By (3),
        we have $\FmB \to \FmB_\bv \in \TPart$
        and by (2), we have $\FmB \in \FPart$, thus
        $v(\FmB)=\bv$; also, by (7), we have
        $\FmA\to\FmB_\bv \in \FPart$.
        Then, if $\FmA \in \TPart$,
        we are done, and if $\FmA \in \FPart$,
        we have $v(\FmA)=\uv$, as desired.
    \item if $v(\FmA\to\FmB)=\uv$:
    then
        $\FmA\to\FmB,(\FmA\to\FmB)\to\FmB_\bv \in \FPart$.
        Then, by (4), either (b): $\FmA \in \FPart$ or
        (c): $\FmB\to\FmB_\bv \in \FPart$.
        Case (b), by (8), we have $\FmB\to\FmB_\bv \in \TPart$. 
        By (7), we have $\FmA\to\FmB_\bv\in\FPart$,
        but, by (6), we have $\FmA\to\FmB_\bv \in \TPart$,
        an absurd.
        Case (c), by (8) we have $\FmA \in \TPart$, i.e. $v(\FmA)=\tv$.
        Also, by (1) and the fact that $\FmA\to\FmB \in \FPart$, we
        have $\FmB \in \FPart$, and then $v(\FmB)=\uv$, as desired;
    \item if $v(\FmA)=\uv$ and $v(\FmB)=\bv$:
    then
        $\FmA,\FmA\to\FmB_\bv \in \FPart$
        and $\FmB \in \FPart$ and $\FmB\to\FmB_\bv \in \TPart$.
        By (5), we have $\FmA\to\FmB \in \FPart$, and, 
        by (6), we have $(\FmA\to\FmB)\to\FmB_\bv \in \TPart$,
        we have $v(\FmA\to\FmB)=\bv$.
\end{itemize}
\end{proof}

==> Translations.tex <==
\section{Translations}
\label{Translations}

Let us consider the fragment $\{\aor\}$ of $\textrm{\L}_3$ obtained by the generating sub-procedure of multiple conclusion Hilbert-style calculi. The rules can be categorized in three classes depending on the output value: $\aor^{ij}_{\bvr}$, $\aor^{ij}_{\uvg}$, and $\aor^{ij}_{\tvb}$ where $i,j \in\{\bv, \uv, \tv\}$. We then apply the streamlining sub-procedure defined by (S1), (S2), (S3), (S4) taking into account the categorization \emph{within each class} and in subsequent \emph{steps}. 

\begin{math}
\hspace{-1.5cm}
\begin{tabular}{@{}ccc@{}}
\mc{3}{c}{Disjunction: $\lukDisj$}\\

%\hline
\rule[-4.5mm]{0mm}{10mm}
\AXC{$\neg\varphi$}
\AXC{$\neg\psi$}
\RL{\fns $\aor^{\bv\bv}_{\bvr\uv}$}
\BIC{$\neg(\varphi \lor \psi), \pmb{\varphi \aor \psi}, \varphi, \psi$}
\DP      
 & 
\AXC{$\neg(\varphi \aor \psi)$}
\AXC{$\neg\varphi$}
\RL{\fns $\aor^{\bv\uv}_{\uvg\bv}$}
\BIC{$\neg\psi, \pmb{\varphi \aor \psi}, \varphi, \psi$}
\DP
 & 
\AXC{$\pmb{\aneg(\varphi \aor \psi)}$}
\AXC{$\aneg \varphi$}
\AXC{$\psi$}
\RL{\fns $\aor^{\bv\tv}_{\tvb\bv}$}
\TIC{$\varphi \aor \psi, \varphi$}
\DP
 \\
%\hline
\rule[-4mm]{0mm}{10mm}
\AXC{$\neg\varphi$}
\AXC{$\neg\psi$}
\AXC{$\pmb{\varphi \lor \psi}$}
\RL{\fns $\aor^{\bv\bv}_{\bvr\tv}$}
\TIC{$\varphi, \psi$}
\DP
 & 
\AXC{$\neg\varphi$}
\AXC{$\pmb{\varphi \lor \psi}$}
\RL{\fns $\aor^{\bv\uv}_{\uvg\tv}$}
\BIC{$\neg\psi, \varphi, \psi$}        
\DP
 &
\AXC{$\neg\varphi$}
\AXC{$\psi$}
\RL{\fns $\aor^{\bv\tv}_{\tvb\uv}$}
\BIC{$\pmb{\aneg(\varphi \aor \psi)}, \varphi \lor \psi, \varphi$}      
\DP
 \\
%\hline

\mc{3}{c}{ \ } \\

%\hline
\rule[-4.5mm]{0mm}{10mm}
\AXC{$\neg(\varphi \lor \psi)$}
\AXC{$\neg\varphi$}
\RL{\fns $\aor^{\uv\bv}_{\uvg\bv}$}
\BIC{$\neg\psi, \pmb{\varphi \aor \psi}, \varphi, \psi$}        
\DP
 & 
\AXC{$\aneg(\varphi \lor \psi)$}
\RL{\fns $\aor^{\uv\uv}_{\uvg\bv}$}
\UIC{$\neg\varphi, \neg\psi, \pmb{\varphi \aor \psi}, \varphi, \psi$}
\DP
 & 
\AXC{$\pmb{\aneg(\varphi \aor \psi)}$}
\AXC{$\psi$}
\RL{\fns $\aor^{\uv\tv}_{\tvb\bv}$}
\BIC{$\neg\varphi, \varphi \lor \psi, \varphi$} 
\DP
 \\
%\hline
\rule[-4.5mm]{0mm}{10mm}
\AXC{$\neg\varphi$}
\AXC{$\pmb{\varphi \lor \psi}$}
\RL{\fns $\aor^{\uv\bv}_{\uvg\tv}$}
\BIC{$\neg\psi, \varphi, \psi$}        
\DP
 & 
\AXC{$\pmb{\varphi \lor \psi}$}
\RL{\fns $\aor^{\uv\uv}_{\uvg\tv}$}
\UIC{$\neg\varphi, \neg\psi, \varphi, \psi$}
\DP
 &
\AXC{$\psi$}
\RL{\fns $\aor^{\uv\tv}_{\tvb\tv}$}
\UIC{$\pmb{\neg(\varphi \aor \psi)}, \neg\varphi, \varphi \lor \psi, \varphi$} 
\DP
 \\
%\hline

\mc{3}{c}{ \ } \\

%\hline
\rule[-4.5mm]{0mm}{10mm}
\AXC{$\pmb{\neg(\varphi \aor \psi)}$}
\AXC{$\neg\psi$}
\AXC{$\varphi$}
\RL{\fns $\aor^{\tv\bv}_{\tvb\bv}$}
\TIC{$\varphi \aor \psi, \varphi$}        
\DP
 &
\AXC{$\pmb{\aneg(\varphi \aor \psi)}$}
\AXC{$\varphi$} 
\RL{\fns $\aor^{\tv\uv}_{\tvb\bv}$}
\BIC{$\aneg \psi, \varphi \lor \psi, \psi$}        
\DP
 &
\AXC{$\pmb{\aneg(\varphi \aor \psi)}$}
\AXC{$\varphi$}
\AXC{$\psi$}
\RL{\fns $\aor^{\tv\tv}_{\tvb\bv}$}
\TIC{$\varphi \aor \psi$} 
\DP
 \\
%\hline
\rule[-4mm]{0mm}{10mm}
\AXC{$\neg\psi$}
\AXC{$\varphi$}
\RL{\fns $\aor^{\tv\bv}_{\tvb\uv}$}
\BIC{$\pmb{\aneg(\varphi \aor \psi)}, \varphi \lor \psi, \psi$}        
\DP
 &
\AXC{$\varphi$}
\RL{\fns $\aor^{\tv\uv}_{\tvb\uv}$}
\UIC{$\pmb{\aneg(\varphi \aor \psi)}, \neg\psi, \varphi \lor \psi, \psi$} 
\DP
 &
\AXC{$\varphi$}
\AXC{$\psi$}
\RL{\fns $\aor^{\tv\tv}_{\tvb\uv}$}
\BIC{$\pmb{\aneg(\varphi \aor \psi)}, \varphi \aor \psi$} 
\DP
 \\
%\hline
\end{tabular}
\end{math}

\vspace{0.5cm}

Notice that each pair of rules $(\aor^{ij}_{kl}, \aor^{i'j'}_{k'l'})$ where $i=i'$, $j=j'$, $k=k'$, and $l \neq l'$ share a formula emphasized in bold, occurring in the premise in one rule and in the conclusion in the other rule. Nonetheless, we cannot apply (S2), because the admissible cuts have to be "additive cuts", namely the pair of rules have to share contexts (in the premise and in the conclusion): this ensures that we do not loose inference power removing rules via (S2). 



==> set-set-calculi/M7.tex <==
\subsection{M7}
Discriminator:
\begin{table}[H]
    \label{tab:seps_configs}
    \centering
    \begin{tabular}{c|cc}
        \toprule
         $x$&$\DesSeps{x}(\PropA)$ & $\NDesSeps{x}(\PropA)$ \\
         \midrule
         $\dv$ & $\EmptySet$ & $\PropA, \PropA\bullet\PropA$\\
         $\uva$ & $\PropA\bullet\PropA$ & $\PropA$\\
         $\uvb$ & $\PropA$ & $\EmptySet$\\
         \bottomrule
    \end{tabular}
\end{table}

\subsubsection{Simplified}

\begin{center}
    r1
\[
\MCRuleInv        
{\text{ $(\varphi \bullet \psi) \bullet (\varphi \bullet \psi)$, $\varphi \bullet \varphi$, $\psi \bullet \psi$ }}        
{\text{  }}        
\]    
r2
\[
\MCRuleInv        
{\text{ $(\varphi \bullet \psi) \bullet (\varphi \bullet \psi)$, $\psi \bullet \psi$ }}        
{\text{ $\varphi$ }}        
\]    
r3
\[
\MCRuleInv        
{\text{ $\varphi \bullet \varphi$, $\psi \bullet \psi$ }}        
{\text{ $\varphi \bullet \psi$ }}        
\]    
r4
\[
\MCRuleInv        
{\text{ $\varphi \bullet \psi$ }}        
{\text{ $\psi \bullet \psi$ }}        
\]    
r5
\[
\MCRuleInv        
{\text{ $\varphi \bullet \psi$ }}        
{\text{ $\psi$ }}        
\]    
r6
\[
\MCRuleInv        
{\text{ $\varphi \bullet \psi$, $\varphi$ }}        
{\text{ $\varphi \bullet \varphi$ }}        
\]    
r7
\[
\MCRuleInv        
{\text{ $\psi \bullet \psi$ }}        
{\text{ $\varphi \bullet \psi$, $\varphi$ }}        
\]
\end{center}

\subsubsection{Full}
\begin{center}
bullet-0,0,1
\[
\MCRuleInv        
{\text{ $(\varphi \bullet \psi) \bullet (\varphi \bullet \psi)$, $\varphi \bullet \varphi$, $\psi \bullet \psi$, $\varphi$, $\psi$ }}        
{\text{  }}        
\]    
bullet-2,0,1
\[
\MCRuleInv        
{\text{ $(\varphi \bullet \psi) \bullet (\varphi \bullet \psi)$, $\psi \bullet \psi$, $\psi$ }}        
{\text{ $\varphi$ }}        
\]    
bullet-0,2,2
\[
\MCRuleInv        
{\text{ $\varphi \bullet \varphi$, $\varphi \bullet \psi$, $\varphi$ }}        
{\text{ $\psi$ }}        
\]    
bullet-0,1,2
\[
\MCRuleInv        
{\text{ $\varphi \bullet \varphi$, $\varphi \bullet \psi$, $\varphi$, $\psi$ }}        
{\text{ $\psi \bullet \psi$ }}        
\]    
bullet-0,0,1
\[
\MCRuleInv        
{\text{ $\varphi \bullet \varphi$, $\psi \bullet \psi$, $\varphi$, $\psi$ }}        
{\text{ $\varphi \bullet \psi$ }}        
\]    
bullet-2,2,2
\[
\MCRuleInv        
{\text{ $\varphi \bullet \psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
bullet-1,0,2
\[
\MCRuleInv        
{\text{ $\varphi \bullet \psi$, $\psi \bullet \psi$, $\varphi$, $\psi$ }}        
{\text{ $\varphi \bullet \varphi$ }}        
\]    
bullet-1,2,2
\[
\MCRuleInv        
{\text{ $\varphi \bullet \psi$, $\varphi$ }}        
{\text{ $\varphi \bullet \varphi$, $\psi$ }}        
\]    
bullet-1,1,2
\[
\MCRuleInv        
{\text{ $\varphi \bullet \psi$, $\varphi$, $\psi$ }}        
{\text{ $\varphi \bullet \varphi$, $\psi \bullet \psi$ }}        
\]    
bullet-2,1,2
\[
\MCRuleInv        
{\text{ $\varphi \bullet \psi$, $\psi$ }}        
{\text{ $\psi \bullet \psi$, $\varphi$ }}        
\]    
bullet-2,0,1
\[
\MCRuleInv        
{\text{ $\psi \bullet \psi$, $\psi$ }}        
{\text{ $\varphi \bullet \psi$, $\varphi$ }}        
\]
\end{center}

==> set-set-calculi/bk.tex <==
\subsection{BK}

\subsubsection{Simplified}
\begin{center}
r2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$ }}        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
\]    
r3
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$ }}        
{\text{ $\neg\varphi$, $\psi$ }}        
\]    
r4
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
r6
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$ }}        
{\text{ $\neg\psi$, $\varphi$ }}        
\]    
r12
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$ }}        
{\text{ $\varphi \to \psi$ }}        
\]    
r13
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$ }}        
{\text{ $\neg(\varphi \to \psi)$ }}        
\]    
r17
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\psi$ }}        
{\text{ $\varphi \to \psi$ }}        
\]    
r18
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$ }}        
\]    
r28
\[
\MCRuleInv        
{\text{ $\psi$ }}        
{\text{ $\varphi \to \psi$, $\varphi$ }}        
\]    
r5
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
r7
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$ }}        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
\]    
r8
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$ }}        
{\text{ $\neg\varphi$, $\psi$ }}        
\]    
r9
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$ }}        
{\text{ $\neg\psi$, $\varphi$ }}        
\]    
r14
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$ }}        
{\text{ $\neg(\varphi \land \psi)$ }}        
\]    
r19
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\psi$ }}        
{\text{ $\neg(\varphi \land \psi)$ }}        
\]    
r25
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\varphi \land \psi$ }}        
\]    
r29
\[
\MCRuleInv        
{\text{ $\psi$ }}        
{\text{ $\varphi \land \psi$ }}        
\]    
r1
\[
\MCRuleInv        
{\text{  }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
r10
\[
\MCRuleInv        
{\text{ $\neg\neg\varphi$ }}        
{\text{ $\varphi$ }}        
\]    
r26
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\neg\neg\varphi$ }}        
\]    
r11
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$ }}        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
\]    
r15
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$ }}        
{\text{ $\neg(\varphi \lor \psi)$ }}        
\]    
r16
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$ }}        
{\text{ $\varphi \lor \psi$ }}        
\]    
r20
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\psi$ }}        
{\text{ $\neg(\varphi \lor \psi)$ }}        
\]    
r21
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\psi$ }}        
{\text{ $\varphi \lor \psi$ }}        
\]    
r22
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$ }}        
{\text{ $\neg\varphi$, $\psi$ }}        
\]    
r23
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$ }}        
{\text{ $\neg\psi$, $\varphi$ }}        
\]    
r24
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
r27
\[
\MCRuleInv        
{\text{ $\varphi$, $\psi$ }}        
{\text{ $\varphi \lor \psi$ }}        
\]    
\end{center}

\subsubsection{Full}

\begin{center}
$\to$-2,2,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
$\to$-0,2,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\varphi$ }}        
{\text{ $\neg\varphi$, $\psi$ }}        
\]    
$\to$-0,0,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\varphi$, $\psi$ }}        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
\]    
$\to$-2,0,0
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$, $\psi$ }}        
{\text{ $\neg\psi$, $\varphi$ }}        
\]    
$\to$-1,1,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
{\text{ $\varphi \to \psi$ }}        
\]    
$\to$-1,1,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$ }}        
\]    
$\to$-1,2,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$ }}        
{\text{ $\varphi \to \psi$, $\psi$ }}        
\]    
$\to$-1,2,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$ }}        
{\text{ $\neg(\varphi \to \psi)$, $\psi$ }}        
\]    
$\to$-1,0,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
{\text{ $\varphi \to \psi$, $\neg\psi$ }}        
\]    
$\to$-1,0,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$, $\neg\psi$ }}        
\]    
$\to$-0,1,1
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
{\text{ $\varphi \to \psi$, $\neg\varphi$ }}        
\]    
$\to$-0,1,1
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$, $\neg\varphi$ }}        
\]    
$\to$-2,1,1
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\psi$ }}        
{\text{ $\varphi \to \psi$, $\varphi$ }}        
\]    
$\to$-2,1,1
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$, $\varphi$ }}        
\]    
$\to$-2,0,0
\[
\MCRuleInv        
{\text{ $\psi$ }}        
{\text{ $\varphi \to \psi$, $\neg\psi$, $\varphi$ }}        
\]    
and-2,2,2
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
and-0,2,0
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$, $\varphi$ }}        
{\text{ $\neg\varphi$, $\psi$ }}        
\]    
and-0,0,0
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$, $\varphi$, $\psi$ }}        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
\]    
and-2,0,0
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$, $\psi$ }}        
{\text{ $\neg\psi$, $\varphi$ }}        
\]    
and-1,1,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
{\text{ $\varphi \land \psi$ }}        
\]    
and-1,1,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
{\text{ $\neg(\varphi \land \psi)$ }}        
\]    
and-1,2,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$ }}        
{\text{ $\varphi \land \psi$, $\psi$ }}        
\]    
and-1,2,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$ }}        
{\text{ $\neg(\varphi \land \psi)$, $\psi$ }}        
\]    
and-1,0,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
{\text{ $\varphi \land \psi$, $\neg\psi$ }}        
\]    
and-1,0,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
{\text{ $\neg(\varphi \land \psi)$, $\neg\psi$ }}        
\]    
and-0,1,1
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
{\text{ $\varphi \land \psi$, $\neg\varphi$ }}        
\]    
and-0,1,1
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
{\text{ $\neg(\varphi \land \psi)$, $\neg\varphi$ }}        
\]    
and-2,1,1
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\psi$ }}        
{\text{ $\varphi \land \psi$, $\varphi$ }}        
\]    
and-2,1,1
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\psi$ }}        
{\text{ $\neg(\varphi \land \psi)$, $\varphi$ }}        
\]    
and-0,2,0
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\varphi \land \psi$, $\neg\varphi$, $\psi$ }}        
\]    
and-0,0,0
\[
\MCRuleInv        
{\text{ $\varphi$, $\psi$ }}        
{\text{ $\varphi \land \psi$, $\neg\varphi$, $\neg\psi$ }}        
\]    
and-2,0,0
\[
\MCRuleInv        
{\text{ $\psi$ }}        
{\text{ $\varphi \land \psi$, $\neg\psi$, $\varphi$ }}        
\]    
neg-2,0
\[
\MCRuleInv        
{\text{  }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
neg-2,0
\[
\MCRuleInv        
{\text{ $\neg\neg\varphi$ }}        
{\text{ $\varphi$ }}        
\]    
neg-1,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$ }}        
{\text{ $\neg\neg\varphi$ }}        
\]    
neg-0,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$ }}        
{\text{ $\neg\varphi$ }}        
\]    
or-0,0,0
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$, $\varphi$, $\psi$ }}        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
\]    
or-1,1,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
{\text{ $\neg(\varphi \lor \psi)$ }}        
\]    
or-1,1,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
{\text{ $\varphi \lor \psi$ }}        
\]    
or-1,2,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\psi$ }}        
\]    
or-1,2,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$ }}        
{\text{ $\varphi \lor \psi$, $\psi$ }}        
\]    
or-1,0,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\neg\psi$ }}        
\]    
or-1,0,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
{\text{ $\neg\psi$, $\varphi \lor \psi$ }}        
\]    
or-0,1,1
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\neg\varphi$ }}        
\]    
or-0,1,1
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
{\text{ $\neg\varphi$, $\varphi \lor \psi$ }}        
\]    
or-2,1,1
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\psi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\varphi$ }}        
\]    
or-2,1,1
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\psi$ }}        
{\text{ $\varphi \lor \psi$, $\varphi$ }}        
\]    
or-2,2,2
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
or-0,2,2
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$, $\varphi$ }}        
{\text{ $\neg\varphi$, $\psi$ }}        
\]    
or-2,0,2
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$, $\psi$ }}        
{\text{ $\neg\psi$, $\varphi$ }}        
\]    
or-0,0,0
\[
\MCRuleInv        
{\text{ $\varphi$, $\psi$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi \lor \psi$ }}        
\]        
\end{center}

==> set-set-calculi/g3.tex <==
\subsection{G3}

\subsubsection{Simplified}
\begin{center}
r2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$ }}        
{\text{ $\neg\varphi$ }}        
\]    
r3
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$ }}        
{\text{ $\psi$ }}        
\]    
r4
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\psi$, $\varphi$ }}        
{\text{  }}        
\]    
r6
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$ }}        
{\text{ $\neg\psi$, $\varphi$ }}        
\]    
r7
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$, $\neg\varphi$ }}        
{\text{ $\neg\psi$ }}        
\]    
r12
\[
\MCRuleInv        
{\text{ $\neg\varphi$ }}        
{\text{ $\varphi \to \psi$, $\neg\psi$ }}        
\]    
r16
\[
\MCRuleInv        
{\text{ $\neg\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$ }}        
\]    
r23
\[
\MCRuleInv        
{\text{ $\psi$ }}        
{\text{ $\varphi \to \psi$, $\varphi$ }}        
\]    
r5
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
r8
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$ }}        
{\text{ $\neg\varphi$ }}        
\]    
r9
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$ }}        
{\text{ $\neg\psi$ }}        
\]    
r13
\[
\MCRuleInv        
{\text{ $\neg\varphi$ }}        
{\text{ $\neg(\varphi \land \psi)$, $\psi$ }}        
\]    
r15
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\neg(\varphi \land \psi)$ }}        
\]    
r17
\[
\MCRuleInv        
{\text{ $\neg\psi$ }}        
{\text{ $\neg(\varphi \land \psi)$, $\varphi$ }}        
\]    
r21
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\varphi \land \psi$ }}        
\]    
r24
\[
\MCRuleInv        
{\text{ $\psi$ }}        
{\text{ $\varphi \land \psi$ }}        
\]    
r1
\[
\MCRuleInv        
{\text{  }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
r10
\[
\MCRuleInv        
{\text{ $\neg\neg\varphi$, $\neg\varphi$ }}        
{\text{  }}        
\]    
r11
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$ }}        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
\]    
r14
\[
\MCRuleInv        
{\text{ $\neg\varphi$ }}        
{\text{ $\neg(\varphi \lor \psi)$ }}        
\]    
r18
\[
\MCRuleInv        
{\text{ $\neg\psi$ }}        
{\text{ $\neg(\varphi \lor \psi)$ }}        
\]    
r19
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$ }}        
{\text{ $\varphi$ }}        
\]    
r20
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$ }}        
{\text{ $\psi$ }}        
\]    
r22
\[
\MCRuleInv        
{\text{ $\varphi$, $\psi$ }}        
{\text{ $\varphi \lor \psi$ }}        
\]       
\end{center}

\subsubsection{Full}
\begin{center}
$\to$-2,2,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
$\to$-1,1,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
{\text{  }}        
\]    
$\to$-1,2,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\varphi$, $\varphi$ }}        
{\text{ $\psi$ }}        
\]    
$\to$-0,1,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\psi$, $\varphi$, $\psi$ }}        
{\text{ $\neg\varphi$ }}        
\]    
$\to$-0,2,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\varphi$ }}        
{\text{ $\neg\varphi$, $\psi$ }}        
\]    
$\to$-0,0,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\varphi$, $\psi$ }}        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
\]    
$\to$-1,0,0
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$, $\neg\varphi$, $\varphi$, $\psi$ }}        
{\text{ $\neg\psi$ }}        
\]    
$\to$-2,0,0
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$, $\psi$ }}        
{\text{ $\neg\psi$, $\varphi$ }}        
\]    
$\to$-1,0,0
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
{\text{ $\varphi \to \psi$, $\neg\psi$ }}        
\]    
$\to$-2,1,1
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\psi$ }}        
{\text{ $\varphi \to \psi$, $\varphi$ }}        
\]    
$\to$-2,1,1
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$, $\varphi$ }}        
\]    
$\to$-2,0,0
\[
\MCRuleInv        
{\text{ $\psi$ }}        
{\text{ $\varphi \to \psi$, $\neg\psi$, $\varphi$ }}        
\]    
and-2,2,2
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
and-1,0,0
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$, $\neg\varphi$, $\varphi$, $\psi$ }}        
{\text{ $\neg\psi$ }}        
\]    
and-0,1,0
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$, $\neg\psi$, $\varphi$, $\psi$ }}        
{\text{ $\neg\varphi$ }}        
\]    
and-0,2,0
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$, $\varphi$ }}        
{\text{ $\neg\varphi$, $\psi$ }}        
\]    
and-0,0,0
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$, $\varphi$, $\psi$ }}        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
\]    
and-2,0,0
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$, $\psi$ }}        
{\text{ $\neg\psi$, $\varphi$ }}        
\]    
and-1,1,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
{\text{ $\varphi \land \psi$ }}        
\]    
and-1,1,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
{\text{ $\neg(\varphi \land \psi)$ }}        
\]    
and-1,2,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$ }}        
{\text{ $\varphi \land \psi$, $\psi$ }}        
\]    
and-1,2,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$ }}        
{\text{ $\neg(\varphi \land \psi)$, $\psi$ }}        
\]    
and-1,0,0
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
{\text{ $\varphi \land \psi$, $\neg\psi$ }}        
\]    
and-0,1,0
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
{\text{ $\varphi \land \psi$, $\neg\varphi$ }}        
\]    
and-2,1,1
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\psi$ }}        
{\text{ $\varphi \land \psi$, $\varphi$ }}        
\]    
and-2,1,1
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\psi$ }}        
{\text{ $\neg(\varphi \land \psi)$, $\varphi$ }}        
\]    
and-0,2,0
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\varphi \land \psi$, $\neg\varphi$, $\psi$ }}        
\]    
and-0,0,0
\[
\MCRuleInv        
{\text{ $\varphi$, $\psi$ }}        
{\text{ $\varphi \land \psi$, $\neg\varphi$, $\neg\psi$ }}        
\]    
and-2,0,0
\[
\MCRuleInv        
{\text{ $\psi$ }}        
{\text{ $\varphi \land \psi$, $\neg\psi$, $\varphi$ }}        
\]    
neg-2,0
\[
\MCRuleInv        
{\text{  }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
neg-2,0
\[
\MCRuleInv        
{\text{ $\neg\neg\varphi$ }}        
{\text{ $\varphi$ }}        
\]    
neg-1,0
\[
\MCRuleInv        
{\text{ $\neg\neg\varphi$, $\neg\varphi$, $\varphi$ }}        
{\text{  }}        
\]    
neg-0,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$ }}        
{\text{ $\neg\varphi$ }}        
\]    
or-0,0,0
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$, $\varphi$, $\psi$ }}        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
\]    
or-1,1,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
{\text{ $\neg(\varphi \lor \psi)$ }}        
\]    
or-1,1,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
{\text{ $\varphi \lor \psi$ }}        
\]    
or-1,2,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi \lor \psi$, $\varphi$ }}        
{\text{ $\psi$ }}        
\]    
or-1,0,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\neg\psi$ }}        
\]    
or-1,0,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
{\text{ $\neg\psi$, $\varphi \lor \psi$ }}        
\]    
or-2,1,2
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi \lor \psi$, $\psi$ }}        
{\text{ $\varphi$ }}        
\]    
or-0,1,1
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\neg\varphi$ }}        
\]    
or-0,1,1
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
{\text{ $\neg\varphi$, $\varphi \lor \psi$ }}        
\]    
or-2,2,2
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
or-0,2,2
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$, $\varphi$ }}        
{\text{ $\neg\varphi$, $\psi$ }}        
\]    
or-2,0,2
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$, $\psi$ }}        
{\text{ $\neg\psi$, $\varphi$ }}        
\]    
or-0,0,0
\[
\MCRuleInv        
{\text{ $\varphi$, $\psi$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi \lor \psi$ }}        
\]    
\end{center}

==> set-set-calculi/j3.tex <==

\subsection{J3}

\subsubsection{Simplified}

\begin{center}
r2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$ }}        
{\text{ $\neg\varphi$ }}        
\]    
r3
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$ }}        
{\text{ $\psi$ }}        
\]    
r4
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\psi$, $\varphi$ }}        
{\text{  }}        
\]    
r6
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$ }}        
{\text{ $\neg\psi$, $\varphi$ }}        
\]    
r11
\[
\MCRuleInv        
{\text{ $\neg\varphi$ }}        
{\text{ $\varphi \to \psi$, $\neg\psi$ }}        
\]    
r15
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$ }}        
{\text{ $\neg(\varphi \to \psi)$, $\neg\psi$ }}        
\]    
r16
\[
\MCRuleInv        
{\text{ $\neg\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$ }}        
\]    
r24
\[
\MCRuleInv        
{\text{ $\psi$ }}        
{\text{ $\varphi \to \psi$, $\varphi$ }}        
\]    
r5
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
r7
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$ }}        
{\text{ $\neg\varphi$ }}        
\]    
r8
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$ }}        
{\text{ $\neg\psi$ }}        
\]    
r12
\[
\MCRuleInv        
{\text{ $\neg\varphi$ }}        
{\text{ $\neg(\varphi \land \psi)$, $\psi$ }}        
\]    
r14
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\neg(\varphi \land \psi)$ }}        
\]    
r17
\[
\MCRuleInv        
{\text{ $\neg\psi$ }}        
{\text{ $\neg(\varphi \land \psi)$, $\varphi$ }}        
\]    
r21
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\varphi \land \psi$ }}        
\]    
r25
\[
\MCRuleInv        
{\text{ $\psi$ }}        
{\text{ $\varphi \land \psi$ }}        
\]    
r1
\[
\MCRuleInv        
{\text{  }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
r9
\[
\MCRuleInv        
{\text{ $\neg\neg\varphi$ }}        
{\text{ $\varphi$ }}        
\]    
r22
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\neg\neg\varphi$ }}        
\]    
r10
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$ }}        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
\]    
r13
\[
\MCRuleInv        
{\text{ $\neg\varphi$ }}        
{\text{ $\neg(\varphi \lor \psi)$ }}        
\]    
r18
\[
\MCRuleInv        
{\text{ $\neg\psi$ }}        
{\text{ $\neg(\varphi \lor \psi)$ }}        
\]    
r19
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$ }}        
{\text{ $\varphi$ }}        
\]    
r20
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$ }}        
{\text{ $\psi$ }}        
\]    
r23
\[
\MCRuleInv        
{\text{ $\varphi$, $\psi$ }}        
{\text{ $\varphi \lor \psi$ }}        
\]       
\end{center}

\subsubsection{Full}
\begin{center}
$\to$-1,1,1
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
$\to$-2,1,1
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\varphi$ }}        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
$\to$-2,2,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
$\to$-1,2,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
$\to$-0,2,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\psi$, $\varphi$ }}        
{\text{ $\psi$ }}        
\]    
$\to$-0,1,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\varphi$ }}        
{\text{ $\neg\psi$, $\psi$ }}        
\]    
$\to$-0,0,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\varphi$, $\psi$ }}        
{\text{  }}        
\]    
$\to$-1,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
$\to$-2,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$, $\neg\varphi$ }}        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
$\to$-2,2,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$, $\varphi$, $\psi$ }}        
\]    
$\to$-2,0,0
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\psi$ }}        
{\text{ $\varphi \to \psi$, $\varphi$ }}        
\]    
$\to$-1,2,2
\[
\MCRuleInv        
{\text{ $\neg\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$, $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
$\to$-0,2,2
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi$ }}        
{\text{ $\neg(\varphi \to \psi)$, $\psi$ }}        
\]    
$\to$-0,1,2
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\neg(\varphi \to \psi)$, $\neg\psi$, $\psi$ }}        
\]    
$\to$-0,0,2
\[
\MCRuleInv        
{\text{ $\varphi$, $\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$ }}        
\]    
$\to$-1,0,0
\[
\MCRuleInv        
{\text{ $\psi$ }}        
{\text{ $\varphi \to \psi$, $\neg\varphi$, $\varphi$ }}        
\]    
and-1,1,1
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
and-2,1,1
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$, $\neg\varphi$ }}        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
and-2,2,2
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$, $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
and-1,2,1
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$, $\neg\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
and-1,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
and-2,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$, $\neg\varphi$ }}        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
and-1,2,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$, $\neg\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
and-2,2,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\neg(\varphi \land \psi)$, $\varphi$, $\psi$ }}        
\]    
and-2,0,0
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\psi$ }}        
{\text{ $\varphi \land \psi$, $\varphi$ }}        
\]    
and-0,2,0
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi$ }}        
{\text{ $\varphi \land \psi$, $\psi$ }}        
\]    
and-0,1,0
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\varphi \land \psi$, $\neg\psi$, $\psi$ }}        
\]    
and-0,0,0
\[
\MCRuleInv        
{\text{ $\varphi$, $\psi$ }}        
{\text{ $\varphi \land \psi$ }}        
\]    
and-1,0,0
\[
\MCRuleInv        
{\text{ $\psi$ }}        
{\text{ $\varphi \land \psi$, $\neg\varphi$, $\varphi$ }}        
\]    
neg-1,1
\[
\MCRuleInv        
{\text{ $\neg\neg\varphi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
neg-1,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
neg-0,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$ }}        
{\text{  }}        
\]    
neg-0,2
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\neg\neg\varphi$ }}        
\]    
or-1,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
or-0,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$, $\varphi$ }}        
{\text{ $\neg\psi$, $\psi$ }}        
\]    
or-1,0,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$, $\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
or-2,1,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
or-2,2,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\varphi$, $\psi$ }}        
\]    
or-2,2,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi \lor \psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
or-2,1,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi \lor \psi$ }}        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
or-2,0,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi \lor \psi$, $\psi$ }}        
{\text{ $\varphi$ }}        
\]    
or-2,0,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\psi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\varphi$ }}        
\]    
or-1,2,2
\[
\MCRuleInv        
{\text{ $\neg\psi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
or-1,2,2
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi \lor \psi$ }}        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
or-0,2,2
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi \lor \psi$, $\varphi$ }}        
{\text{ $\psi$ }}        
\]    
or-0,2,2
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\psi$ }}        
\]    
or-1,1,1
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
or-0,1,1
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$, $\varphi$ }}        
{\text{ $\neg\psi$, $\psi$ }}        
\]    
or-1,0,1
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$, $\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
or-0,0,0
\[
\MCRuleInv        
{\text{ $\varphi$, $\psi$ }}        
{\text{ $\varphi \lor \psi$ }}        
\]    
pos-1,2
\[
\MCRuleInv        
{\text{  }}        
{\text{ $\neg\Diamond\varphi$, $\neg\varphi$, $\varphi$ }}        
\]    
pos-2,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$ }}        
{\text{ $\neg\Diamond\varphi$, $\varphi$ }}        
\]    
pos-2,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\Diamond\varphi$ }}        
{\text{ $\varphi$ }}        
\]    
pos-1,2
\[
\MCRuleInv        
{\text{ $\Diamond\varphi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
pos-0,0
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\Diamond\varphi$ }}        
\]    
\end{center}

==> set-set-calculi/l3.tex <==
\subsection{(Streamlined) multiple conclusion calculus $(s)mc.
\textrm{\L}3$}

Below we list the rules of the multiple conclusion calculus $mc.\textrm{\L}3$ automatically generated by \cite{xxx}. 

\begin{remark}
\label{notation:MultipleConclusionRules}
Notice that the rules and the names of rules are in a one-to-one correspondence with matrix entries. Given the rule name `\,$\conn^{ij}_{km}$\,' the coordinates $i,j,k$ identifies the matrix entries for binary connective $\conn$ (resp.~unary connective if $j$ is empty) cfr.~\ref{notation:3LabelledRules}, where the vector $ij$ refers to the list of input values in the matrix, and $k$ refers to the corresponding output value in the matrix. Following the previous convention, we color the output value in rules' names to emphasize all rules sharing the same output per each connective. Moreover, $m \in V\setminus\{k\}$ identifies a value $m \neq k$.  
\end{remark}

\begin{math}
\hspace{1.5cm}
\begin{tabular}{@{}rrr@{}}

\mc{3}{c}{Negation: $\lukNeg$} \\

%\hline
\rule[-4mm]{0mm}{10mm}
\AXC{$\neg\neg\varphi$}
\AXC{$\neg\varphi$}
\RL{\fns $\aneg^\bv_{\tvb\bv}$}
\BIC{$\neg\varphi, \varphi$}
\DP
 &
\AXC{$\neg\neg\varphi$}
\RL{\fns $\aneg^\uv_{\uvg\bv}$}
\UIC{$\neg\varphi$, $\varphi$}
\DP
 &
\AXC{$\varphi$}
\RL{\fns $\aneg^\tv_{\bvr\uv}$}
\UIC{$\neg\neg\varphi, \aneg \varphi$}
\DP
 \\
%\hline
\rule[-4mm]{0mm}{10mm}
\AXC{$\aneg\varphi$}
\RL{\fns $\aneg^\bv_{\tvb\uv}$}
\UIC{$\aneg\aneg\varphi, \aneg\varphi, \varphi$}
\DP
 & 
\AXC{$\neg\varphi$}
\RL{\fns $\aneg^\uv_{\uvg\tv}$}
\UIC{$\neg\varphi, \varphi$}
\DP
 &
\AXC{$\neg\varphi$, $\varphi$}
\RL{\fns $\aneg^\tv_{\bvr\tv}$}
\UIC{$\ $}        
\DP
 \\
%\hline
\end{tabular}
\end{math}

\vspace{0.5cm}

\begin{math}
\hspace{-2cm}
\begin{tabular}{@{}rrr@{}}

\mc{3}{c}{Conjunction: $\lukConj$}\\

%\hline
\rule[-4.5mm]{0mm}{10mm}
\AXC{$\neg\varphi$}
\AXC{$\neg\psi$}
\RL{\fns $\aand^{\bv\bv}_{\bvr\uv}$}
\BIC{$\varphi \aand \psi, \neg(\varphi \land \psi), \varphi, \psi$}
\DP
 & 
\AXC{$\neg\varphi$}
\RL{\fns $\aand^{\bv\uv}_{\bvr\uv}$}
\UIC{$\varphi \aand \psi, \neg(\varphi \aand \psi), \neg \psi, \varphi, \psi$}
\DP
 &
\AXC{$\neg\varphi$}
\AXC{$\psi$}
\RL{\fns $\aand^{\bv\tv}_{\bvr\uv}$}
\BIC{$\varphi \aand \psi, \neg(\varphi \land \psi), \varphi$}
\DP
 \\
%\hline
\rule[-4mm]{0mm}{10mm}
\AXC{$\varphi \aand \psi$}
\AXC{$\neg\varphi$}
\AXC{$\neg\psi$}
\RL{\fns $\aand^{\bv\bv}_{\bvr\tv}$}
\TIC{$\varphi, \psi$}
\DP
 & 
\AXC{$\varphi \aand \psi$}
\AXC{$\neg \varphi$}
\RL{\fns $\aand^{\bv\uv}_{\bvr\tv}$}
\BIC{$\neg \psi, \varphi, \psi$}
\DP
 & 
\AXC{$\varphi \land \psi$}
\AXC{$\neg\varphi$}
\AXC{$\psi$}
\RL{\fns $\aand^{\bv\tv}_{\bvr\tv}$}
\TIC{$\varphi$}
\DP
 \\
%\hline

\mc{3}{c}{ \ } \\

%\hline
\rule[-4.5mm]{0mm}{10mm}
\AXC{$\neg\psi$}
\RL{\fns $\aand^{\uv\bv}_{\bvr\uv}$}
\UIC{$\varphi \aand \psi, \neg(\varphi \land \psi), \neg\varphi, \varphi, \psi$}
\DP
 &
\AXC{$\neg(\varphi \land \psi)$}
\RL{\fns $\aand^{\uv\uv}_{\uvg\bv}$}
\UIC{$\varphi \aand \psi, \aneg\varphi, \neg\psi, \varphi, \psi$}
\DP
 &
\AXC{$\neg(\varphi \land \psi)$}
\AXC{$\psi$}
\RL{\fns $\aand^{\uv\tv}_{\uvg\bv}$}
\BIC{$\varphi \aand \psi, \neg\varphi, \varphi$}
\DP
 \\
%\hline
\rule[-4mm]{0mm}{10mm}
\AXC{$\varphi \land \psi$}
\AXC{$\neg\psi$}
\RL{\fns $\aand^{\uv\bv}_{\bvr\tv}$}
\BIC{$\neg\varphi, \varphi, \psi$}
\DP
 & 
\AXC{$\varphi \land \psi$}
\RL{\fns $\aand^{\uv\uv}_{\uvg\tv}$}
\UIC{$\neg\varphi, \neg\psi, \varphi, \psi$} 
\DP
 & 
\AXC{$\varphi \land \psi$}
\AXC{$\psi$}
\RL{\fns $\aand^{\uv\tv}_{\uvg\tv}$}
\BIC{$\neg\varphi, \varphi$}        
\DP
 \\
%\hline 

\mc{3}{c}{ \ } \\

%\hline
\rule[-4mm]{0mm}{10mm}
\AXC{$\varphi \aand \psi$}
\AXC{$\neg\psi$}
\AXC{$\varphi$}
\RL{\fns $\aand^{\tv\bv}_{\bvr\tv}$}
\TIC{$\psi$}        
\DP
 & 
\AXC{$\neg(\varphi \aand \psi)$}
\AXC{$\varphi$}
\RL{\fns $\aand^{\tv\uv}_{\uvg\bv}$}
\BIC{$\varphi \aand \psi, \neg\psi, \psi$}
\DP
 & 
\AXC{$\aneg(\varphi \aand \psi)$}
\AXC{$\varphi$}
\AXC{$\psi$}
\RL{\fns $\aand^{\tv\tv}_{\tvb\bv}$}
\TIC{$\varphi \aand \psi$}
\DP
 \\
%\hline
\rule[-4mm]{0mm}{10mm}
\AXC{$\neg\psi$}
\AXC{$\varphi$}
\RL{\fns $\aand^{\tv\bv}_{\bvr\uv}$}
\BIC{$\varphi \aand \psi, \neg(\varphi \land \psi), \psi$}
\DP  
 & 
\AXC{$\varphi \aand \psi$}
\AXC{$\varphi$}
\RL{\fns $\aand^{\tv\uv}_{\uvg\tv}$}
\BIC{$\neg\psi, \psi$}
\DP
 &
\AXC{$\varphi$}
\AXC{$\psi$}
\RL{\fns $\aand^{\tv\tv}_{\tvb\uv}$}
\BIC{$\varphi \aand \psi, \aneg(\varphi \aand \psi)$}
\DP
 \\
%\hline
\end{tabular}
\end{math}

\vspace{0.5cm}

\begin{math}
\hspace{-1.8cm}
\begin{tabular}{@{}rrr@{}}

\mc{3}{c}{Disjunction: $\lukDisj$}\\

%\hline
\rule[-4.5mm]{0mm}{10mm}
\AXC{$\neg\varphi$}
\AXC{$\neg\psi$}
\RL{\fns $\aor^{\bv\bv}_{\bvr\uv}$}
\BIC{$\neg(\varphi \lor \psi), \varphi \aor \psi, \varphi, \psi$}
\DP      
 & 
\AXC{$\neg(\varphi \aor \psi)$}
\AXC{$\neg\varphi$}
\RL{\fns $\aor^{\bv\uv}_{\uvg\bv}$}
\BIC{$\neg\psi, \varphi \aor \psi, \varphi, \psi$}
\DP
 & 
\AXC{$\aneg(\varphi \aor \psi)$}
\AXC{$\aneg \varphi$}
\AXC{$\psi$}
\RL{\fns $\aor^{\bv\tv}_{\tvb\bv}$}
\TIC{$\varphi \aor \psi, \varphi$}
\DP
 \\
%\hline
\rule[-4mm]{0mm}{10mm}
\AXC{$\neg\varphi$}
\AXC{$\neg\psi$}
\AXC{$\varphi \lor \psi$}
\RL{\fns $\aor^{\bv\bv}_{\bvr\tv}$}
\TIC{$\varphi, \psi$}
\DP
 & 
\AXC{$\neg\varphi$}
\AXC{$\varphi \lor \psi$}
\RL{\fns $\aor^{\bv\uv}_{\uvg\tv}$}
\BIC{$\neg\psi, \varphi, \psi$}        
\DP
 &
\AXC{$\neg\varphi$}
\AXC{$\psi$}
\RL{\fns $\aor^{\bv\tv}_{\tvb\uv}$}
\BIC{$\aneg(\varphi \aor \psi), \varphi \lor \psi, \varphi$}      
\DP
 \\
%\hline

\mc{3}{c}{ \ } \\

%\hline
\rule[-4.5mm]{0mm}{10mm}
\AXC{$\neg(\varphi \lor \psi)$}
\AXC{$\neg\varphi$}
\RL{\fns $\aor^{\uv\bv}_{\uvg\bv}$}
\BIC{$\neg\varphi, \varphi \aor \psi, \varphi, \psi$}        
\DP
 & 
\AXC{$\aneg(\varphi \lor \psi)$}
\RL{\fns $\aor^{\uv\uv}_{\uvg\bv}$}
\UIC{$\neg\varphi, \neg\psi, \varphi \aor \psi, \varphi, \psi$}
\DP
 & 
\AXC{$\aneg(\varphi \aor \psi)$}
\AXC{$\psi$}
\RL{\fns $\aor^{\uv\tv}_{\tvb\bv}$}
\BIC{$\neg\varphi, \varphi \lor \psi, \varphi$} 
\DP
 \\
%\hline
\rule[-4.5mm]{0mm}{10mm}
\AXC{$\neg\varphi$}
\AXC{$\varphi \lor \psi$}
\RL{\fns $\aor^{\uv\bv}_{\uvg\tv}$}
\BIC{$\neg\psi, \varphi, \psi$}        
\DP
 & 
\AXC{$\varphi \lor \psi$}
\RL{\fns $\aor^{\uv\uv}_{\uvg\tv}$}
\UIC{$\neg\varphi, \neg\psi, \varphi, \psi$}
\DP
 &
\AXC{$\psi$}
\RL{\fns $\aor^{\uv\tv}_{\tvb\tv}$}
\UIC{$\neg(\varphi \aor \psi), \neg\varphi, \varphi \lor \psi, \varphi$} 
\DP
 \\
%\hline

\mc{3}{c}{ \ } \\

%\hline
\rule[-4.5mm]{0mm}{10mm}
\AXC{$\neg(\varphi \aor \psi)$}
\AXC{$\neg\psi$}
\AXC{$\varphi$}
\RL{\fns $\aor^{\tv\bv}_{\tvb\bv}$}
\TIC{$\varphi \aor \psi, \varphi$}        
\DP
 &
\AXC{$\aneg(\varphi \aor \psi)$}
\AXC{$\varphi$} 
\RL{\fns $\aor^{\tv\uv}_{\tvb\bv}$}
\BIC{$\aneg \psi, \varphi \lor \psi, \psi$}        
\DP
 &
\AXC{$\aneg(\varphi \aor \psi)$}
\AXC{$\varphi$}
\AXC{$\psi$}
\RL{\fns $\aor^{\tv\tv}_{\tvb\bv}$}
\TIC{$\varphi \aor \psi$} 
\DP
 \\
%\hline
\rule[-4mm]{0mm}{10mm}
\AXC{$\neg\psi$}
\AXC{$\varphi$}
\RL{\fns $\aor^{\tv\bv}_{\tvb\uv}$}
\BIC{$\aneg(\varphi \aor \psi), \varphi \lor \psi, \psi$}        
\DP
 &
\AXC{$\varphi$}
\RL{\fns $\aor^{\tv\uv}_{\tvb\uv}$}
\UIC{$\aneg(\varphi \aor \psi), \neg\psi, \varphi \lor \psi, \psi$} 
\DP
 &
\AXC{$\varphi$}
\AXC{$\psi$}
\RL{\fns $\aor^{\tv\tv}_{\tvb\uv}$}
\BIC{$\aneg(\varphi \aor \psi), \varphi \aor \psi$} 
\DP
 \\
%\hline
\end{tabular}
\end{math}

\vspace{0.5cm}

\begin{math}
\hspace{-3cm}
\begin{tabular}{@{}rrr@{}}
\mc{3}{c}{Implication: $\lukImp$} \\
%\hline
\rule[-4.5mm]{0mm}{10mm}
\AXC{$\aneg(\varphi \ararr \psi)$}
\AXC{$\neg\varphi$}
\AXC{$\neg\psi$}
\RL{\fns $\ararr^{\bv\bv}_{\tvb\bv}$}
\TIC{$\varphi \to \psi, \varphi, \psi$}
\DP 
 &
\AXC{$\aneg(\varphi \ararr \psi)$}
\AXC{$\neg\varphi$}
\RL{\fns $\ararr^{\bv\uv}_{\tvb\bv}$}
\BIC{$\varphi \to \psi, \neg\psi, \varphi, \psi$}
\DP     
 &
\AXC{$\neg (\varphi \to \psi)$}
\AXC{$\aneg \varphi$}
\AXC{$\psi$}
\RL{\fns $\ararr^{\bv\tv}_{\tvb\bv}$}
\TIC{$\varphi \to \psi, \aneg \psi, \psi$}
\DP
 \\
%\hline
\rule[-4.5mm]{0mm}{10mm}
\AXC{$\neg\varphi$}
\AXC{$\neg\psi$}
\RL{\fns $\ararr^{\bv\bv}_{\tvb\uv}$}
\BIC{$\varphi \to \psi, \aneg (\varphi \ararr \psi), \varphi, \psi$}
\DP
 &
\AXC{$\neg\varphi$}
\RL{\fns $\ararr^{\bv\uv}_{\tvb\uv}$}
\UIC{$\varphi \to \psi, \aneg(\varphi \ararr \psi), \neg\psi, \varphi, \psi$}
\DP
 &
\AXC{$\neg\varphi$}
\AXC{$\psi$}
\RL{\fns $\ararr^{\bv\tv}_{\tvb\uv}$}
\BIC{$\varphi \to \psi, \aneg (\varphi \to \psi), \varphi$}
\DP
 \\
%\hline

\mc{3}{c}{ \ } \\

%\hline
\rule[-4.5mm]{0mm}{10mm}
\AXC{$\neg(\varphi \to \psi)$}
\AXC{$\neg\psi$}
\RL{\fns $\ararr^{\uv\bv}_{\uvg\bv}$}
\BIC{$\varphi \to \psi, \neg\varphi, \varphi, \psi$}
\DP
 & 
\AXC{$ \ $}
\RL{\fns $\ararr^{\uv\uv}_{\tvb\uv}$}
\UIC{$\varphi \to \psi, \aneg (\varphi \to \psi), \neg\varphi, \neg\psi, \varphi, \psi$}
\DP
 & 
\AXC{$\aneg(\varphi \to \psi)$}
\AXC{$\psi$}  
\RL{\fns $\ararr^{\uv\tv}_{\tvb\bv}$}
\BIC{$\varphi \to \psi, \neg\varphi, \aneg \psi, \varphi$}
\DP
 \\
%\hline
\rule[-4.5mm]{0mm}{10mm}
\AXC{$\varphi \to \psi$}
\AXC{$\neg\psi$} 
\RL{\fns $\ararr^{\uv\bv}_{\uvg\tv}$}
\BIC{$\neg\varphi, \varphi, \psi$}        
\DP
 & 
\AXC{$\aneg (\varphi \ararr \psi)$}
\RL{\fns $\ararr^{\uv\uv}_{\tvb\bv}$}
\UIC{$\varphi \ararr \psi, \neg\varphi, \neg\psi, \varphi, \psi$}
\DP
 &
\AXC{$\psi$}  
\RL{\fns $\ararr^{\uv\tv}_{\tvb\uv}$}
\UIC{$\varphi \to \psi, \aneg(\varphi \to \psi), \neg\varphi, \aneg \psi, \varphi, \psi$}
\DP
 \\
%\hline

\mc{3}{c}{ \ } \\

%\hline
\rule[-4.5mm]{0mm}{10mm}
\AXC{$\neg\psi$}
\AXC{$\varphi$}
\RL{\fns $\ararr^{\tv\bv}_{\bvr\uv}$}
\BIC{$\varphi \to \psi, \neg(\varphi \to \psi), \psi$}
\DP
 &
\AXC{$\neg(\varphi \to \psi)$}
\AXC{$\varphi$}
\RL{\fns $\ararr^{\tv\uv}_{\uvg\bv}$}
\BIC{$\varphi \to \psi, \neg\psi, \psi$}        
\DP
 &
\AXC{$\aneg (\varphi \ararr \psi)$}
\AXC{$\varphi$}
\AXC{$\psi$}
\RL{\fns $\ararr^{\tv\tv}_{\tvb\bv}$}
\TIC{$\varphi \to \psi$}        
\DP
 \\
%\hline
\rule[-4.5mm]{0mm}{10mm}
\AXC{$\varphi \to \psi$}
\AXC{$\neg\psi$}
\AXC{$\varphi$}
\RL{\fns $\ararr^{\tv\bv}_{\bvr\tv}$}
\TIC{$\psi$}
\DP  
 & 
\AXC{$\varphi \to \psi$}
\AXC{$\varphi$}
\RL{\fns $\ararr^{\tv\uv}_\uvg$}
\BIC{$\neg\psi, \psi$}
\DP
 & 
\AXC{$\varphi$}
\AXC{$\psi$}
\RL{\fns $\ararr^{\tv\tv}_{\tvb\uv}$}
\BIC{$\varphi \to \psi, \aneg(\varphi \to \psi)$}        
\DP
 \\
%\hline
\end{tabular}
\end{math}

%\subsubsection{Full}
%\begin{center}
%$\to$-2,2,2
%\[
%\MCRuleInv        
%{\text{ $\varphi \to \psi$ }}        
%{\text{ $\varphi$, $\psi$ }}        
%\]    
%$\to$-1,1,2
%\[
%\MCRuleInv        
%{\text{ $\varphi \to \psi$, $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
%{\text{  }}        
%\]    
%$\to$-1,2,2
%\[
%\MCRuleInv        
%{\text{ $\varphi \to \psi$, $\neg\varphi$, $\varphi$ }}
%{\text{ $\psi$ }}        
%\]    
%$\to$-0,1,2
%\[
%\MCRuleInv        
%{\text{ $\varphi \to \psi$, $\neg\psi$, $\varphi$, $\psi$ }}
%{\text{ $\neg\varphi$ }}        
%\]    
%$\to$-0,2,2
%\[
%\MCRuleInv        
%{\text{ $\varphi \to \psi$, $\varphi$ }}        
%{\text{ $\neg\varphi$, $\psi$ }}        
%\]    
%$\to$-0,0,2
%\[
%\MCRuleInv        
%{\text{ $\varphi \to \psi$, $\varphi$, $\psi$ }}        
%{\text{ $\neg\varphi$, $\neg\psi$ }}        
%\]    
%$\to$-2,0,0
%\[
%\MCRuleInv        
%{\text{ $\neg(\varphi \to \psi)$, $\psi$ }}        
%{\text{ $\neg\psi$, $\varphi$ }}        
%\]    
%$\to$-1,0,1
%\[
%\MCRuleInv        
%{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
%{\text{ $\varphi \to \psi$, $\neg\psi$ }}        
%\]    
%$\to$-1,0,1
%\[
%\MCRuleInv        
%{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
%{\text{ $\neg(\varphi \to \psi)$, $\neg\psi$ }}        
%\] 
%$\to$-2,0,0
%\[
%\MCRuleInv        
%{\text{ $\psi$ }}        
%{\text{ $\varphi \to \psi$, $\neg\psi$, $\varphi$ }}        
%\]  
%$\to$-2,1,1
%\[
%\MCRuleInv        
%{\text{ $\neg\psi$, $\psi$ }}        
%{\text{ $\varphi \to \psi$, $\varphi$ }}        
%\]    
%$\to$-2,1,1
%\[
%\MCRuleInv        
%{\text{ $\neg\psi$, $\psi$ }}        
%{\text{ $\neg(\varphi \to \psi)$, $\varphi$ }}        
%\]    
%$\land$-2,2,2
%\[
%\MCRuleInv        
%{\text{ $\varphi \land \psi$ }}        
%{\text{ $\varphi$, $\psi$ }}        
%\]    
%$\land$-1,0,0
%\[
%\MCRuleInv        
%{\text{ $\neg(\varphi \land \psi)$, $\neg\varphi$, $\varphi$, $\psi$ }}        
%{\text{ $\neg\psi$ }}        
%\]    
%$\land$-0,1,0
%\[
%\MCRuleInv        
%{\text{ $\neg(\varphi \land \psi)$, $\neg\psi$, $\varphi$, $\psi$ }}        
%{\text{ $\neg\varphi$ }}        
%\]    
%$\land$-0,2,0
%\[
%\MCRuleInv        
%{\text{ $\neg(\varphi \land \psi)$, $\varphi$ }}        
%{\text{ $\neg\varphi$, $\psi$ }}        
%\]    
%$\land$-0,0,0
%\[
%\MCRuleInv        
%{\text{ $\neg(\varphi \land \psi)$, $\varphi$, $\psi$ }}        
%{\text{ $\neg\varphi$, $\neg\psi$ }}        
%\]    
%$\land$-2,0,0
%\[
%\MCRuleInv        
%{\text{ $\neg(\varphi \land \psi)$, $\psi$ }}        
%{\text{ $\neg\psi$, $\varphi$ }}        
%\]    
%$\land$-1,1,1
%\[
%\MCRuleInv        
%{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
%{\text{ $\varphi \land \psi$ }}        
%\]    
%$\land$-1,1,1
%\[
%\MCRuleInv        
%{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
%{\text{ $\neg(\varphi \land \psi)$ }}        
%\]    
%$\land$-1,2,1
%\[
%\MCRuleInv        
%{\text{ $\neg\varphi$, $\varphi$ }}        
%{\text{ $\varphi \land \psi$, $\psi$ }}        
%\]    
%$\land$-1,2,1
%\[
%\MCRuleInv        
%{\text{ $\neg\varphi$, $\varphi$ }}        
%{\text{ $\neg(\varphi \land \psi)$, $\psi$ }}        
%\]    
%$\land$-1,0,0
%\[
%\MCRuleInv        
%{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
%{\text{ $\varphi \land \psi$, $\neg\psi$ }}        
%\]    
%$\land$-0,1,0
%\[
%\MCRuleInv        
%{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
%{\text{ $\varphi \land \psi$, $\neg\varphi$ }}        
%\]    
%$\land$-2,1,1
%\[
%\MCRuleInv        
%{\text{ $\neg\psi$, $\psi$ }}        
%{\text{ $\varphi \land \psi$, $\varphi$ }}        
%\]    
%$\land$-2,1,1
%\[
%\MCRuleInv        
%{\text{ $\neg\psi$, $\psi$ }}        
%{\text{ $\neg(\varphi \land \psi)$, $\varphi$ }}        
%\]    
%$\land$-0,2,0
%\[
%\MCRuleInv        
%{\text{ $\varphi$ }}        
%{\text{ $\varphi \land \psi$, $\neg\varphi$, $\psi$ }}
%\]
%$\land$-0,0,0
%\[
%\MCRuleInv        
%{\text{ $\varphi$, $\psi$ }}        
%{\text{ $\varphi \land \psi$, $\neg\varphi$, $\neg\psi$ }}
%\]    
%$\land$-2,0,0
%\[
%\MCRuleInv        
%{\text{ $\psi$ }}        
%{\text{ $\varphi \land \psi$, $\neg\psi$, $\varphi$ }}
%\]    
%$\neg$-2,0
%\[
%\MCRuleInv        
%{\text{  }}        
%{\text{ $\neg\varphi$, $\varphi$ }}        
%\]    
%$\neg$-2,0
%\[
%\MCRuleInv        
%{\text{ $\neg\neg\varphi$ }}        
%{\text{ $\varphi$ }}        
%\]    
%$\neg$-1,1
%\[
%\MCRuleInv        
%{\text{ $\neg\varphi$, $\varphi$ }}        
%{\text{ $\neg\neg\varphi$ }}        
%\]    
%$\neg$-0,2
%\[
%\MCRuleInv        
%{\text{ $\neg\varphi$, $\varphi$ }}        
%{\text{ $\neg\varphi$ }}        
%\]    
%$\lor$-0,0,0
%\[
%\MCRuleInv        
%{\text{ $\neg(\varphi \lor \psi)$, $\varphi$, $\psi$ }}
%{\text{ $\neg\varphi$, $\neg\psi$ }}        
%\]    
%$\lor$-1,1,1
%\[
%\MCRuleInv        
%{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}
%{\text{ $\neg(\varphi \lor \psi)$ }}        
%\]    
%$\lor$-1,1,1
%\[
%\MCRuleInv        
%{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}
%{\text{ $\varphi \lor \psi$ }}        
%\]    
%$\lor$-1,2,2
%\[
%\MCRuleInv        
%{\text{ $\neg\varphi$, $\varphi \lor \psi$, $\varphi$ }}   
%{\text{ $\psi$ }}        
%\]    
%$\lor$-1,0,1
%\[
%\MCRuleInv        
%{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
%{\text{ $\neg(\varphi \lor \psi)$, $\neg\psi$ }}        
%\]    
%$\lor$-1,0,1
%\[
%\MCRuleInv        
%{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
%{\text{ $\neg\psi$, $\varphi \lor \psi$ }}        
%\]    
%$\lor$-0,1,1
%\[
%\MCRuleInv        
%{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
%{\text{ $\neg(\varphi \lor \psi)$, $\neg\varphi$ }}        
%\]    
%$\lor$-0,1,1
%\[
%\MCRuleInv        
%{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
%{\text{ $\neg\varphi$, $\varphi \lor \psi$ }}        
%\] 
%$\lor$-0,2,2
%\[
%\MCRuleInv        
%{\text{ $\varphi \lor \psi$, $\varphi$ }}        
%{\text{ $\neg\varphi$, $\psi$ }}        
%\] 
%$\lor$-2,1,2
%\[
%\MCRuleInv        
%{\text{ $\neg\psi$, $\varphi \lor \psi$, $\psi$ }}        
%{\text{ $\varphi$ }}        
%\]    
%$\lor$-2,2,2
%\[
%\MCRuleInv        
%{\text{ $\varphi \lor \psi$ }}        
%{\text{ $\varphi$, $\psi$ }}        
%\]
%$\lor$-2,0,2
%\[
%\MCRuleInv        
%{\text{ $\varphi \lor \psi$, $\psi$ }}        
%{\text{ $\neg\psi$, $\varphi$ }}        
%\]    
%$\lor$-0,0,0
%\[
%\MCRuleInv        
%{\text{ $\varphi$, $\psi$ }}        
%{\text{ $\neg\varphi$, $\neg\psi$, $\varphi \lor \psi$ }}    
%\]    
%\end{center}

\vspace{0,5cm}

Below we provide the streamlined multiple conclusion calculus $smc.\textrm{\L}3$.

\vspace{0,5cm}

\begin{math}
\hspace{3cm}
\AXC{$\varphi$} 
\RL{\fns $\mathsf{r}_9^\aneg$}
\UIC{$\neg\neg\varphi$}        
\DP
 \ \ \
\AXC{$\neg\varphi, \varphi$}
\RL{\fns $\mathsf{r}_1^\aneg$}
\UIC{$\phantom{\varphi}$}
\DP
 \ \ \ 
\AXC{$\neg\neg\varphi$}
\RL{\fns $\mathsf{r}_{22}^\aneg$}
\UIC{$\varphi$}        
\DP
\end{math}

\vspace{0.5cm}

\begin{math}
\hspace{-3.8cm}
\AXC{$\varphi$}
\AXC{$\psi$} 
\RL{\fns $\mathsf{r}_5^\aand$}
\BIC{$\varphi \land \psi$}
\DP
\ \ \ 
\AXC{$\neg\varphi$} 
\RL{\fns $\mathsf{r}_7^\aand$}
\UIC{$\neg(\varphi \land \psi)$}
\DP
 \ \ \
\AXC{$\neg\psi$}
\RL{\fns $\mathsf{r}_8^\aand$}
\UIC{$\neg(\varphi \land \psi)$}
\DP
 \ \ \ 
\AXC{$\neg(\varphi \land \psi)$}
\AXC{$\psi$}
\RL{\fns $\mathsf{r}_{12}^\aand$}
\BIC{$\neg\varphi$}
\DP
 \ \ \ 
\AXC{$\neg(\varphi \land \psi)$}
\RL{\fns $\mathsf{r}_{14}^\aand$}
\UIC{$\neg\varphi, \neg\psi$}
\DP
 \ \ \ 
\AXC{$\neg(\varphi \land \psi)$}
\AXC{$\varphi$}
\RL{\fns $\mathsf{r}_{16}^\aand$}
\BIC{$\neg\psi$}
\DP
 \ \ \ 
\AXC{$\varphi \land \psi$}  
\RL{\fns $\mathsf{r}_{20}^\aand$}
\UIC{$\varphi$}        
\DP
 \ \ \
\AXC{$\varphi \land \psi$}  
\RL{\fns $\mathsf{r}_{25}^\aand$}
\UIC{$\psi$}        
\DP
\end{math} 

\vspace{0.5cm}

\begin{math}
\hspace{-0.3cm}
\AXC{$\neg\varphi$}
\AXC{$\neg\psi$}
\RL{\fns $\mathsf{r}_{10}^\aor$}
\BIC{$\neg(\varphi \lor \psi)$}        
\DP
 \ \ 
%\AXC{$\neg\psi$}
%\RL{\fns r9}
%\UIC{$\neg(\varphi \lor \psi), \varphi$}        
%\DP
% \ \ 
%\AXC{$\neg\varphi$}
%\RL{\fns r10}
%\UIC{$\neg(\varphi \lor \psi), \psi$}        
%\DP
% \ \  
\AXC{$\neg(\varphi \lor \psi)$}
\RL{\fns $\mathsf{r}_{13}^\aor$}
\UIC{$\neg\varphi$}
\DP
 \ \  
\AXC{$\neg(\varphi \lor \psi)$}
\RL{\fns $\mathsf{r}_{17}^\aor$}
\UIC{$\neg\psi$}
\DP 
 \ \  
\AXC{$\varphi$} 
\RL{\fns $\mathsf{r}_{18}^\aor$}
\UIC{$\varphi \lor \psi$}        
\DP
 \ \  
\AXC{$\psi$} 
\RL{\fns $\mathsf{r}_{19}^\aor$}
\UIC{$\varphi \lor \psi$}        
\DP
 \ \  
\AXC{$\varphi \aor \psi$}
\RL{\fns $\mathsf{r}_{23}^\aor$}
\UIC{$\varphi, \psi$}
\DP
\end{math}

\vspace{0,5cm}

\begin{math}
\hspace{-4.3cm}
\AXC{$\aneg \varphi$}
\RL{\fns $\mathsf{r}_2^\ararr$}
\UIC{$\varphi \to \psi$} 
\DP
 \ \ \
\AXC{$\psi$}
\RL{\fns $\mathsf{r}_3^\ararr$}
\UIC{$\varphi \to \psi$} 
\DP
 \ \ \
\AXC{$\phantom{\varphi}$} 
\RL{\fns $\mathsf{r}_4^\ararr$}
\UIC{$\varphi \to \psi, \aneg \psi, \varphi$}      
\DP
 \ \ \
\AXC{$\neg\psi$}
\AXC{$\varphi$}
\RL{\fns $\mathsf{r}_6^\ararr$}
\BIC{$\neg(\varphi \to \psi)$}
\DP
 \ \ \
\AXC{$\varphi \ararr \psi$}
\AXC{$\aneg \psi$}
\RL{\fns $\mathsf{r}_{11}^\ararr$}
\BIC{$\neg\varphi$}
\DP
 \ \ \
\AXC{$\neg(\varphi \to \psi)$}      
\RL{\fns $\mathsf{r}_{15}^\ararr$}
\UIC{$\neg\psi$}
\DP
 \ \ \
\AXC{$\neg(\varphi \to \psi)$}
\RL{\fns $\mathsf{r}_{21}^\ararr$}
\UIC{$\varphi$}
\DP
 \ \ \
\AXC{$\varphi$}
\AXC{$\varphi \to \psi$} 
\RL{\fns $\mathsf{r}_{24}^\ararr$}
\BIC{$\psi$}
\DP
\end{math}

%\subsubsection{Simplified}
%\begin{center}
%
%r1
%\[
%\MCRuleInv        
%{\text{ $\varphi \to \psi$ }}        
%{\text{ $\psi$ }}        
%\]  
%r2
%\[
%\MCRuleInv        
%{\text{ $\varphi \to \psi$, $\varphi$ }}        
%{\text{  }}        
%\]    
%r4
%\[
%\MCRuleInv        
%{\text{ $\neg(\varphi \to \psi)$ }}        
%{\text{ $\neg\psi$, $\varphi$ }}        
%\]    
%r14
%\[
%\MCRuleInv        
%{\text{ $\neg\psi$ }}        
%{\text{ $\neg(\varphi \to \psi)$ }}        
%\]    
%r19
%\[
%\MCRuleInv        
%{\text{ $\varphi$ }}        
%{\text{ $\neg(\varphi \to \psi)$ }}        
%\]    
%r22
%\[
%\MCRuleInv        
%{\text{ $\psi$ }}        
%{\text{ $\varphi \to \psi$, $\varphi$ }}        
%\]    
%r3
%\[
%\MCRuleInv        
%{\text{ $\varphi \land \psi$ }}        
%{\text{ $\varphi$, $\psi$ }}        
%\]    
%r5
%\[
%\MCRuleInv        
%{\text{ $\neg(\varphi \land \psi)$ }}        
%{\text{ $\neg\varphi$ }}        
%\]    
%r6
%\[
%\MCRuleInv        
%{\text{ $\neg(\varphi \land \psi)$ }}        
%{\text{ $\neg\psi$ }}        
%\]    
%r12
%\[
%\MCRuleInv        
%{\text{ $\neg\varphi$, $\neg\psi$ }}        
%{\text{ $\neg(\varphi \land \psi)$ }}        
%\]    
%r18
%\[
%\MCRuleInv        
%{\text{ $\varphi$ }}        
%{\text{ $\varphi \land \psi$ }}        
%\]    
%r23
%\[
%\MCRuleInv        
%{\text{ $\psi$ }}        
%{\text{ $\varphi \land \psi$ }}        
%\]    
%r7
%\[
%\MCRuleInv        
%{\text{ $\neg\neg\varphi$ }}        
%{\text{ $\varphi$ }}        
%\]    
%r13
%\[
%\MCRuleInv        
%{\text{ $\neg\varphi$, $\varphi$ }}        
%{\text{  }}        
%\]    
%r20
%\[
%\MCRuleInv        
%{\text{ $\varphi$ }}        
%{\text{ $\neg\neg\varphi$ }}        
%\]    
%r8
%\[
%\MCRuleInv        
%{\text{ $\neg(\varphi \lor \psi)$ }}        
%{\text{ $\neg\varphi$, $\neg\psi$ }}        
%\]    
%r9
%\[
%\MCRuleInv        
%{\text{ $\neg(\varphi \lor \psi)$, $\varphi$ }}        
%{\text{ $\neg\psi$ }}        
%\]    
%r10
%\[
%\MCRuleInv        
%{\text{ $\neg(\varphi \lor \psi)$, $\psi$ }}        
%{\text{ $\neg\varphi$ }}        
%\]    
%r11
%\[
%\MCRuleInv        
%{\text{ $\neg\varphi$ }}        
%{\text{ $\neg(\varphi \lor \psi)$ }}        
%\]    
%r15
%\[
%\MCRuleInv        
%{\text{ $\neg\psi$ }}        
%{\text{ $\neg(\varphi \lor \psi)$ }}        
%\]    
%r16
%\[
%\MCRuleInv        
%{\text{ $\varphi \lor \psi$ }}        
%{\text{ $\varphi$ }}        
%\]    
%r17
%\[
%\MCRuleInv        
%{\text{ $\varphi \lor \psi$ }}        
%{\text{ $\psi$ }}        
%\]    
%r21
%\[
%\MCRuleInv        
%{\text{ $\varphi$, $\psi$ }}        
%{\text{ $\varphi \lor \psi$ }}        
%\]    
%\end{center}

\vspace{0.5cm}

\textcolor{red}{G. Below we show that multiple conclusion Hilbert-style calculi can be equivalently presented in disjunctive rule form and in conjunctive rule form.}

Multiple conclusion derivations are acyclic graphs, with a set of premises on the top layer and a set of conclusions on the bottom layer. In order to obtain a tree the downward-branching notation packs all premises in one and the same root node, while the upward-branching notation packs all the conclusions in one and the same root node.

In the downward-branching notation, rules are represented in \emph{disjunctive rule form}, namely metalinguistical conjunctions $\Sand$ (in this case, represented as commas in actual derivations) always occur under the scope of metalinguistical disjunctions $\Sor$ (in this case, represented as withe spaces between branches). Note that the set of formulas labelling each node is upward closed, meaning that each node $n$ is officially labelled with all formulas labelling the nodes above $n$ on the same branch. In actual derivations only active formulas are explicitly depicted. Moreover, proof sections $\pi_i$ where all rules are single conclusion are depicted as a single linear branch: we call them $\Sand$-\emph{components}. Notice that each formula occurs exactly once even tough it is used in multiple rule applications.

Below we provide a $sm.\textrm{L}_3$ derivation $\pi$ in disjunctive rule form of $((A \ararr B) \ararr B) \ararr ((B \ararr A) \ararr A)$, where $\alpha_i = ((A \ararr B) \ararr B) \ararr ((B \ararr A) \ararr A)$ and $1 \leq i \leq 5$. To facilitate the reading, we add superscripts $a, b, c, d$ matching premises with rule application performed at a later stage in the derivation.

\vspace{0.5cm}

\begin{math} 
\hspace{2cm}
    \begin{tikzpicture}[every tree node/.style={},
       level distance=1.2cm,sibling distance=.05cm,
       edge from parent path={(\tikzparentnode) -- (\tikzchildnode)}, baseline]
        \Tree[.\node[style={}] {$\varnothing$};
            \edge[] node[auto=right]{$\RuleA_{4}$};
            [.{$\alpha_5$}
            ]
            [.{$\neg B \to \neg A^{ab}$}
                \edge[] node[auto=right]{$\RuleA_{4}$};
                [.{$A \to B$}
                    \edge[] node[auto=right]{$\RuleA_{3}$};
                    [.{$\alpha_4$}
                    ]
                ]
                [.{$\neg B$}
                    \edge[] node[auto=right]{$\RuleA_{24}^a$};
                    [.{$\neg A$}
                        \edge[] node[auto=right]{$\RuleA_{2}$};
                        [.{$A \to B$}
                            \edge[] node[auto=right]{$\RuleA_{3}$};
                            [.{$\alpha_3$}
                            ]
                        ]
                    ]
                ]
                [.{$A$}
                    \edge[] node[auto=right]{$\RuleA_{9}$};
                    [.{$\neg\neg A$}
                        \edge[] node[auto=right]{$\RuleA_{11}^b$};
                        [.{$\neg\neg B$}
                            \edge[] node[auto=right]{$\RuleA_{22}$};
                            [.{$B$}
                                \edge[] node[auto=right]{$\RuleA_{3}$};
                                [.{$A \to B$}
                                    \edge[] node[auto=right]{$\RuleA_{3}$};
                                    [.{$\alpha_2$}
                                    ]
                                ]
                            ]
                        ]
                    ]
                ]
            ]
            [.{$\neg(A \to B)^c$}
                \edge[] node[auto=right]{$\RuleA_{21}$};
                [.{$A$}
                    \edge[] node[auto=right]{$\RuleA_{9}$};
                    [.{$\neg\neg A^d$}
                        \edge[] node[auto=right]{$\RuleA_{15}^c$};
                        [.{$\neg B$}
                            \edge[] node[auto=right]{$\RuleA_{6}^d$};
                            [.{$\neg(\neg B \to \neg A)$}
                                \edge[] node[auto=right]{$\RuleA_{2}$};
                                [.{$\alpha_1$}
                                ]
                            ]
                        ]
                    ]
                ]
            ]
        ]
    \end{tikzpicture}
\end{math}

\vspace{0.5cm}

Notice that in the previous derivation $\pi$ there are five $\Sand$-components: 
\begin{itemize}
\item $\pi_1$ is the proof section $\lb \mathsf{r}_{21}, \mathsf{r}_9, \mathsf{r}_{15}, \mathsf{r}_6, \mathsf{r}_2 \rb[\aneg(A \ararr B), \aneg(A \ararr B)]$, where $\lb \mathsf{r}_{21}, \mathsf{r}_9, \mathsf{r}_{15}, \mathsf{r}_6, \mathsf{r}_2 \rb$ is the string of rule applications from top to bottom, $\aneg(A \ararr B)$ is the label of the initial node and $\alpha_1$ is the label of the terminal node.
\item $\pi_2$ is the proof section $\lb \mathsf{r}_9, \mathsf{r}_{11}, \mathsf{r}_{22}, \mathsf{r}_3, \mathsf{r}_3 \rb[A, \alpha_2]$;
\item $\pi_3$ is the proof section $\lb \mathsf{r}_{24}, \mathsf{r}_2, \mathsf{r}_3 \rb[\neg B, \alpha_3]$;
\item $\pi_4$ is the proof section $\lb \mathsf{r}_3 \rb[A \ararr B,\alpha_4]$;
\item $\pi_5$ is the proof section $\lb \emptyset \rb[\alpha_1, \emptyset]$, where $\lb \emptyset \rb$ is the empty string of rule applications, and $[\alpha_1, \emptyset]$ denotes the fact that there is only one initial node.
\end{itemize}

In the upward-branching notation, rules are represented in \emph{conjunctive rule form}, namely metalinguistical disjunctions $\Sor$ (in this case, represented as commas in actual derivations) always occur under the scope of metalinguistical conjunctions $\Sand$ (in this case, represented as withe spaces between branches). 

In what follows, we first provide a conjunctive rule form representation of the $\Sand$-components $\pi_1, \pi_2, \pi_3, \pi_4, \pi_5$ occurring in the previous derivation $\pi$.

The conjunctive rule form representation of the $\Sand$-component $\pi_1$ is the following: 

\begin{center}
{\small
\AXC{$\aneg (A \ararr B)$}
\RL{$\mathsf{r}_{21}$}
\UIC{$A $}
\RL{$r_9$}
\UIC{$\aneg \aneg A$}
%
\AXC{$\aneg (A \ararr B)$}
\RL{$\mathsf{r}_{15}$}
\UIC{$\aneg B$}
%
\RL{$\mathsf{r}_6$}
\BIC{$\aneg (\aneg B \ararr \aneg A)$}
\RL{$\mathsf{r}_2$}
\UIC{$\rule[-0.7mm]{0mm}{2.8mm}\alpha_1$}
\DP
 }
\end{center}

Notice that the previous derivation is, indeed, a notational variant of the $\Sand$-component $\pi_1$: the initial nodes are labelled with $\aneg (A \ararr B)$ and the terminal node is labelled with $\alpha_5$ (and the string of rule applications from top-left to right-down is again $\lb \mathsf{r}_{21}, \mathsf{r}_9, \mathsf{r}_{15}, \mathsf{r}_6, \mathsf{r}_2 \rb$). The only difference is just notational: in the previous presentation $\aneg (A \ararr B)$ is used twice (as premise of $\mathsf{r}_{21}$ and as premise of $\mathsf{r}_{15}$) but explicitly represented only once, while in this case $\aneg (A \ararr B)$ is explicitly represented as many times it is used. So, taking into account the arity of rules and the tree-shape of proof sections, we may rewrite the string of rule applications as the following bracketed string: $\mathsf{r}_2(\mathsf{r}_6(\mathsf{r}_9(r_{21} (\aneg(A \ararr B))), \mathsf{r}_{15} (\aneg(A \ararr B))))[\alpha_1]$, where $\aneg(A \ararr B)$ is the label of the leaves (aka the initial node) and $\alpha_1$ is the root (aka the terminal node).

The conjunctive rule form representation of the $\Sand$-component $\pi_2$ is the following: 

\begin{center}
\AXC{$\aneg B \ararr \aneg A$}
\AXC{$A$}
\RL{$\mathsf{r}_9$}
\UIC{$\aneg\aneg A$}
\RL{$\mathsf{r}_{11}$}
\BIC{$\aneg \aneg B$}
\RL{$\mathsf{r}_{22}$}
\UIC{$B$}
\RL{$\mathsf{r}_{3}$}
\UIC{$A \ararr B$}
\RL{$\mathsf{r}_{3}$}
\UIC{$\rule[-0.7mm]{0mm}{2.8mm}\alpha_2$}
\DP
\end{center}

Notice that the previous derivation is, indeed, a notational variant of the $\Sand$-component $\pi_2$. Taking into account the arity of rules and the tree-shape of proof sections, we may rewrite the string of rule applications as the following bracketed string: $\mathsf{r}_3(\mathsf{r}_3(\mathsf{r}_{22}(\aneg B \ararr \aneg A, \mathsf{r}_{11}(\mathsf{r}_9))))[\alpha_2]$.

The conjunctive rule form representation of the $\Sand$-component $\pi_3$ is the following: 

\begin{center}
\AXC{$\aneg B \ararr \aneg A$}
\AXC{$\aneg B$}
\RL{$\mathsf{r}_{24}$}
\BIC{$\aneg A$}
\RL{$\mathsf{r}_2$}
\UIC{$A \ararr B$}
\RL{$\mathsf{r}_3$}
\UIC{$\rule[-0.7mm]{0mm}{2.8mm}\alpha_3$}
\DP
\end{center}

Notice that the previous derivation is, indeed, a notational variant of the $\Sand$-component $\pi_3$. Taking into account the arity of rules and the tree-shape of proof sections, we may rewrite the string of rule applications as the following bracketed string: $\mathsf{r}_2(\aneg B \ararr \aneg A, \mathsf{r}_{24})[\alpha_3]$.

The conjunctive rule form representation of the $\Sand$-component $\pi_4$ is the following: 

\begin{center}
\AXC{$A \ararr B$}
\RL{$\mathsf{r}_3$}
\UIC{$\rule[-0.7mm]{0mm}{2.8mm}\alpha_4$}
\DP
\end{center}

Notice that the previous derivation is, indeed, a notational variant of the $\Sand$-component $\pi_4$. Taking into account the arity of rules and the tree-shape of proof sections, we may rewrite the string of rule applications as the following bracketed string: $\mathsf{r}_3(A \ararr B)[\alpha_4]$.

The conjunctive rule form representation of the $\Sand$-component $\pi_5$ is the following: 

\begin{center}
\AXC{$\alpha_5$}
\DP
\end{center}

Notice that the previous derivation is, indeed, a notational variant of the $\Sand$-component $\pi_5$. Taking into account the arity of rules and the tree-shape of proof sections, we may rewrite the string of rule applications as the following bracketed string: $\emptyset[\alpha_5]$.

Now we put together all the $\Sand$-components $\pi_i$ with $1 \leq i \leq 5$ to represent the full proof $\pi$ in conjunctive rule form. Also in this case we adopt the convention that only active formulas are depicted in the proof: it follows that commas can appear only on the leaves with a disjunctive reading $\Sor$. Vice versa, in the case of disjunctive rule form presentations commas might appear only on the root with a conjunctive reading. Notice that now we have six leaves, given that in the previous proof we have a nesting of two $\mathsf{r}_4$ applications and each of which has three conclusion. To facilitate the reading, we add superscripts $a, b, c, d, e$ matching premises with rule application performed at a later stage in the derivation. 

\vspace{0.5cm}

\begin{math}
\hspace{-1.2cm}
\AXC{$\mathsf{r}_4$}
\UIC{$\aneg (A \ararr B),^a$}
\noLine
\UIC{$\alpha_5,$}
\noLine
\UIC{$\aneg B \ararr \aneg A$}
%%
\AXC{$\mathsf{r}_4$}
\UIC{$\aneg (A \ararr B),^a$}
\noLine
\UIC{$\alpha_5,$}
\noLine
\UIC{$\aneg B \ararr \aneg A$}
%
\AXC{$\mathsf{r}_4$}
\UIC{$A,^b$}
\noLine
\UIC{$A\ararr B,^e$}
\noLine
\UIC{$\aneg B$}
%
\RL{$\mathsf{r}_{24}$}
\BIC{$\aneg A$}
\RL{$\mathsf{r}_2$}
\UIC{$A \ararr B$}
\RL{$\mathsf{r}_3$}
\UIC{$\rule[-0.7mm]{0mm}{2.8mm}\alpha_3$}
\RL{$\mathsf{r}_9^b$}
\UIC{$\aneg \aneg A$}
%%
\RL{$\mathsf{r}_{11}$}
\BIC{$\aneg \aneg B$}
\RL{$\mathsf{r}_{22}$}
\UIC{$B$}
\RL{$\mathsf{r}_{3}$}
\UIC{$A \ararr B$}
\RL{$\mathsf{r}_{3}$}
\UIC{$\rule[-0.7mm]{0mm}{2.8mm}\alpha_2$}
%
\RL{$\mathsf{r}_{21}^a$}
\UIC{$A $}
\RL{$\mathsf{r}_9$}
\UIC{$\aneg \aneg A$}
%
\AXC{$\mathsf{r}_4$}
\UIC{$\aneg (A \ararr B),^c$}
\noLine
\UIC{$\alpha_5,$}
\noLine
\UIC{$\aneg B \ararr \aneg A$}
%%
\AXC{$\mathsf{r}_4$}
\UIC{$\aneg (A \ararr B),^c$}
\noLine
\UIC{$\alpha_5,$}
\noLine
\UIC{$\aneg B \ararr \aneg A$}
%
\AXC{$\mathsf{r}_4$}
\UIC{$A,^d$}
\noLine
\UIC{$A\ararr B,^e$}
\noLine
\UIC{$\aneg B$}
%
\RL{$\mathsf{r}_{24}$}
\BIC{$\aneg A$}
\RL{$\mathsf{r}_2$}
\UIC{$A \ararr B$}
\RL{$\mathsf{r}_3$}
\UIC{$\rule[-0.7mm]{0mm}{2.8mm}\alpha_3$}
\RL{$\mathsf{r}_9^d$}
\UIC{$\aneg \aneg A$}
%%
\RL{$\mathsf{r}_{11}$}
\BIC{$\aneg \aneg B$}
\RL{$\mathsf{r}_{22}$}
\UIC{$B$}
\RL{$\mathsf{r}_{3}$}
\UIC{$A \ararr B$}
\RL{$\mathsf{r}_{3}$}
\UIC{$\rule[-0.7mm]{0mm}{2.8mm}\alpha_2$}
%
\RL{$\mathsf{r}_{15}^c$}
\UIC{$\aneg B$}
%
\RL{$\mathsf{r}_6$}
\BIC{$\aneg (\aneg B \ararr \aneg A)$}
\RL{$\mathsf{r}_2$}
\UIC{$\rule[-0.7mm]{0mm}{2.8mm}\alpha_1$}
\RL{$\mathsf{r}_3^e$}
\UIC{$\rule[-0.7mm]{0mm}{2.8mm}\alpha_4$}
\DP
\end{math}

\vspace{0.5cm}

Notice that the previous derivation is, indeed, a notational variant (in conjunctive rule form) of the derivation $\pi$ (in disjunctive rule form). 

\textcolor{red}{Notice that a way to organize matrices is per output. This more directly/easily/naturally correspond to/can be expressed via rules in conjuctive normal form. This is a reason to go for such a rule form in the case of $n$-labelled sequent calculi. Vice versa, in the case of multiple conclusion Hilbert-style calculi, the organizations of matrices is not like this and it is mediated by separators. This is why having a dicjunctive versus a conjunctive rules form does not make a lot of difference in this case, I guess.}


==> set-set-calculi/lp.tex <==
\subsection{$\LPImpName$}

\subsubsection{Full}

\begin{center}
$\to$-1,1,1
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
$\to$-2,1,1
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\varphi$ }}        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
$\to$-2,2,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
$\to$-1,2,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
$\to$-0,2,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\psi$, $\varphi$ }}        
{\text{ $\psi$ }}        
\]    
$\to$-0,1,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\varphi$ }}        
{\text{ $\neg\psi$, $\psi$ }}        
\]    
$\to$-0,0,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\varphi$, $\psi$ }}        
{\text{  }}        
\]    
$\to$-1,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
$\to$-2,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$, $\neg\varphi$ }}        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
$\to$-2,2,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$, $\varphi$, $\psi$ }}        
\]    
$\to$-2,0,0
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\psi$ }}        
{\text{ $\varphi \to \psi$, $\varphi$ }}        
\]    
$\to$-1,2,2
\[
\MCRuleInv        
{\text{ $\neg\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$, $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
$\to$-0,2,2
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi$ }}        
{\text{ $\neg(\varphi \to \psi)$, $\psi$ }}        
\]    
$\to$-0,1,2
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\neg(\varphi \to \psi)$, $\neg\psi$, $\psi$ }}        
\]    
$\to$-0,0,2
\[
\MCRuleInv        
{\text{ $\varphi$, $\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$ }}        
\]    
$\to$-1,0,0
\[
\MCRuleInv        
{\text{ $\psi$ }}        
{\text{ $\varphi \to \psi$, $\neg\varphi$, $\varphi$ }}        
\]    
and-1,1,1
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
and-2,1,1
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$, $\neg\varphi$ }}        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
and-2,2,2
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$, $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
and-1,2,1
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$, $\neg\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
and-1,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
and-2,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$, $\neg\varphi$ }}        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
and-1,2,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$, $\neg\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
and-2,2,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\neg(\varphi \land \psi)$, $\varphi$, $\psi$ }}        
\]    
and-2,0,0
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\psi$ }}        
{\text{ $\varphi \land \psi$, $\varphi$ }}        
\]    
and-0,2,0
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi$ }}        
{\text{ $\varphi \land \psi$, $\psi$ }}        
\]    
and-0,1,0
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\varphi \land \psi$, $\neg\psi$, $\psi$ }}        
\]    
and-0,0,0
\[
\MCRuleInv        
{\text{ $\varphi$, $\psi$ }}        
{\text{ $\varphi \land \psi$ }}        
\]    
and-1,0,0
\[
\MCRuleInv        
{\text{ $\psi$ }}        
{\text{ $\varphi \land \psi$, $\neg\varphi$, $\varphi$ }}        
\]    
neg-1,1
\[
\MCRuleInv        
{\text{ $\neg\neg\varphi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
neg-1,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
neg-0,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$ }}        
{\text{  }}        
\]    
neg-0,2
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\neg\neg\varphi$ }}        
\]    
or-1,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
or-0,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$, $\varphi$ }}        
{\text{ $\neg\psi$, $\psi$ }}        
\]    
or-1,0,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$, $\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
or-2,1,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
or-2,2,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\varphi$, $\psi$ }}        
\]    
or-2,2,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi \lor \psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
or-2,1,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi \lor \psi$ }}        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
or-2,0,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi \lor \psi$, $\psi$ }}        
{\text{ $\varphi$ }}        
\]    
or-2,0,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\psi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\varphi$ }}        
\]    
or-1,2,2
\[
\MCRuleInv        
{\text{ $\neg\psi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
or-1,2,2
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi \lor \psi$ }}        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
or-0,2,2
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi \lor \psi$, $\varphi$ }}        
{\text{ $\psi$ }}        
\]    
or-0,2,2
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\psi$ }}        
\]    
or-1,1,1
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
or-0,1,1
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$, $\varphi$ }}        
{\text{ $\neg\psi$, $\psi$ }}        
\]    
or-1,0,1
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$, $\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
or-0,0,0
\[
\MCRuleInv        
{\text{ $\varphi$, $\psi$ }}        
{\text{ $\varphi \lor \psi$ }}        
\]    
\end{center}

\subsubsection{Simplified}
\begin{center}
r1
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$ }}        
{\text{ $\psi$ }}        
\]    
r2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\varphi$ }}        
{\text{  }}        
\]    
r4
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$ }}        
{\text{ $\neg\psi$, $\varphi$ }}        
\]    
r14
\[
\MCRuleInv        
{\text{ $\neg\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$ }}        
\]    
r19
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\neg(\varphi \to \psi)$ }}        
\]    
r22
\[
\MCRuleInv        
{\text{ $\psi$ }}        
{\text{ $\varphi \to \psi$, $\varphi$ }}        
\]    
r3
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
r5
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$ }}        
{\text{ $\neg\varphi$ }}        
\]    
r6
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$ }}        
{\text{ $\neg\psi$ }}        
\]    
r12
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\neg(\varphi \land \psi)$ }}        
\]    
r18
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\varphi \land \psi$ }}        
\]    
r23
\[
\MCRuleInv        
{\text{ $\psi$ }}        
{\text{ $\varphi \land \psi$ }}        
\]    
r7
\[
\MCRuleInv        
{\text{ $\neg\neg\varphi$ }}        
{\text{ $\varphi$ }}        
\]    
r13
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$ }}        
{\text{  }}        
\]    
r20
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\neg\neg\varphi$ }}        
\]    
r8
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$ }}        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
\]    
r9
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$, $\varphi$ }}        
{\text{ $\neg\psi$ }}        
\]    
r10
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$, $\psi$ }}        
{\text{ $\neg\varphi$ }}        
\]    
r11
\[
\MCRuleInv        
{\text{ $\neg\varphi$ }}        
{\text{ $\neg(\varphi \lor \psi)$ }}        
\]    
r15
\[
\MCRuleInv        
{\text{ $\neg\psi$ }}        
{\text{ $\neg(\varphi \lor \psi)$ }}        
\]    
r16
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$ }}        
{\text{ $\varphi$ }}        
\]    
r17
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$ }}        
{\text{ $\psi$ }}        
\]    
r21
\[
\MCRuleInv        
{\text{ $\varphi$, $\psi$ }}        
{\text{ $\varphi \lor \psi$ }}        
\]    
    \end{center}

==> set-set-calculi/pwk.tex <==
\subsection{PWK}

\subsubsection{Simplified}
\begin{center}
$\to$-1,1,1
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
$\to$-2,1,1
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\varphi$ }}        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
$\to$-2,2,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
$\to$-1,2,1
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
$\to$-0,2,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\psi$, $\varphi$ }}        
{\text{ $\psi$ }}        
\]    
$\to$-0,1,1
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\varphi$ }}        
{\text{ $\neg\psi$, $\psi$ }}        
\]    
$\to$-0,0,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\varphi$, $\psi$ }}        
{\text{  }}        
\]    
$\to$-1,0,1
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
$\to$-1,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
$\to$-2,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$, $\neg\varphi$ }}        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
$\to$-1,2,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$, $\neg\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
$\to$-0,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$, $\varphi$ }}        
{\text{ $\neg\psi$, $\psi$ }}        
\]    
$\to$-1,0,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$, $\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
$\to$-2,2,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$, $\varphi$, $\psi$ }}        
\]    
$\to$-2,0,0
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\psi$ }}        
{\text{ $\varphi \to \psi$, $\varphi$ }}        
\]    
$\to$-0,2,2
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi$ }}        
{\text{ $\neg(\varphi \to \psi)$, $\psi$ }}        
\]    
$\to$-0,0,2
\[
\MCRuleInv        
{\text{ $\varphi$, $\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$ }}        
\]    
and-1,1,1
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
and-2,1,1
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$, $\neg\varphi$ }}        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
and-2,2,2
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$, $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
and-1,2,1
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$, $\neg\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
and-0,1,1
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$, $\varphi$ }}        
{\text{ $\neg\psi$, $\psi$ }}        
\]    
and-1,0,1
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$, $\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
and-1,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
and-2,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$, $\neg\varphi$ }}        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
and-1,2,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$, $\neg\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
and-0,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$, $\varphi$ }}        
{\text{ $\neg\psi$, $\psi$ }}        
\]    
and-1,0,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$, $\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
and-2,2,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\neg(\varphi \land \psi)$, $\varphi$, $\psi$ }}        
\]    
and-2,0,0
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\psi$ }}        
{\text{ $\varphi \land \psi$, $\varphi$ }}        
\]    
and-0,2,0
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi$ }}        
{\text{ $\varphi \land \psi$, $\psi$ }}        
\]    
and-0,0,0
\[
\MCRuleInv        
{\text{ $\varphi$, $\psi$ }}        
{\text{ $\varphi \land \psi$ }}        
\]    
neg-1,1
\[
\MCRuleInv        
{\text{ $\neg\neg\varphi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
neg-1,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
neg-0,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$ }}        
{\text{  }}        
\]    
neg-0,2
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\neg\neg\varphi$ }}        
\]    
or-1,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
or-2,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$, $\neg\varphi$ }}        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
or-1,2,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$, $\neg\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
or-0,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$, $\varphi$ }}        
{\text{ $\neg\psi$, $\psi$ }}        
\]    
or-1,0,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$, $\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
or-2,2,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\varphi$, $\psi$ }}        
\]    
or-2,2,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi \lor \psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
or-2,1,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi \lor \psi$ }}        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
or-2,0,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi \lor \psi$, $\psi$ }}        
{\text{ $\varphi$ }}        
\]    
or-2,0,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\psi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\varphi$ }}        
\]    
or-1,2,1
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi \lor \psi$ }}        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
or-0,2,2
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi \lor \psi$, $\varphi$ }}        
{\text{ $\psi$ }}        
\]    
or-0,2,2
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\psi$ }}        
\]    
or-1,1,1
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
or-0,1,1
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$, $\varphi$ }}        
{\text{ $\neg\psi$, $\psi$ }}        
\]    
or-1,0,1
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$, $\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
or-0,0,0
\[
\MCRuleInv        
{\text{ $\varphi$, $\psi$ }}        
{\text{ $\varphi \lor \psi$ }}        
\]        
\end{center}

\subsubsection{Full}

\begin{center}
    $\to$-1,1,1
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
$\to$-2,1,1
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\varphi$ }}        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
$\to$-2,2,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
$\to$-1,2,1
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
$\to$-0,2,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\psi$, $\varphi$ }}        
{\text{ $\psi$ }}        
\]    
$\to$-0,1,1
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\varphi$ }}        
{\text{ $\neg\psi$, $\psi$ }}        
\]    
$\to$-0,0,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\varphi$, $\psi$ }}        
{\text{  }}        
\]    
$\to$-1,0,1
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
$\to$-1,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
$\to$-2,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$, $\neg\varphi$ }}        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
$\to$-1,2,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$, $\neg\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
$\to$-0,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$, $\varphi$ }}        
{\text{ $\neg\psi$, $\psi$ }}        
\]    
$\to$-1,0,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$, $\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
$\to$-2,2,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$, $\varphi$, $\psi$ }}        
\]    
$\to$-2,0,0
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\psi$ }}        
{\text{ $\varphi \to \psi$, $\varphi$ }}        
\]    
$\to$-0,2,2
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi$ }}        
{\text{ $\neg(\varphi \to \psi)$, $\psi$ }}        
\]    
$\to$-0,0,2
\[
\MCRuleInv        
{\text{ $\varphi$, $\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$ }}        
\]    
and-1,1,1
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
and-2,1,1
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$, $\neg\varphi$ }}        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
and-2,2,2
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$, $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
and-1,2,1
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$, $\neg\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
and-0,1,1
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$, $\varphi$ }}        
{\text{ $\neg\psi$, $\psi$ }}        
\]    
and-1,0,1
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$, $\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
and-1,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
and-2,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$, $\neg\varphi$ }}        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
and-1,2,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$, $\neg\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
and-0,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$, $\varphi$ }}        
{\text{ $\neg\psi$, $\psi$ }}        
\]    
and-1,0,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$, $\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
and-2,2,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\neg(\varphi \land \psi)$, $\varphi$, $\psi$ }}        
\]    
and-2,0,0
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\psi$ }}        
{\text{ $\varphi \land \psi$, $\varphi$ }}        
\]    
and-0,2,0
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi$ }}        
{\text{ $\varphi \land \psi$, $\psi$ }}        
\]    
and-0,0,0
\[
\MCRuleInv        
{\text{ $\varphi$, $\psi$ }}        
{\text{ $\varphi \land \psi$ }}        
\]    
neg-1,1
\[
\MCRuleInv        
{\text{ $\neg\neg\varphi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
neg-1,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
neg-0,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$ }}        
{\text{  }}        
\]    
neg-0,2
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\neg\neg\varphi$ }}        
\]    
or-1,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
or-2,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$, $\neg\varphi$ }}        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
or-1,2,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$, $\neg\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
or-0,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$, $\varphi$ }}        
{\text{ $\neg\psi$, $\psi$ }}        
\]    
or-1,0,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$, $\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
or-2,2,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\varphi$, $\psi$ }}        
\]    
or-2,2,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi \lor \psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
or-2,1,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi \lor \psi$ }}        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
or-2,0,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi \lor \psi$, $\psi$ }}        
{\text{ $\varphi$ }}        
\]    
or-2,0,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\psi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\varphi$ }}        
\]    
or-1,2,1
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi \lor \psi$ }}        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
or-0,2,2
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi \lor \psi$, $\varphi$ }}        
{\text{ $\psi$ }}        
\]    
or-0,2,2
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\psi$ }}        
\]    
or-1,1,1
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
or-0,1,1
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$, $\varphi$ }}        
{\text{ $\neg\psi$, $\psi$ }}        
\]    
or-1,0,1
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$, $\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
or-0,0,0
\[
\MCRuleInv        
{\text{ $\varphi$, $\psi$ }}        
{\text{ $\varphi \lor \psi$ }}        
\] 
\end{center}


==> set-set-calculi/s3.tex <==

\subsection{S3}

\subsubsection{Simplified}

\begin{center}
r1
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$ }}        
{\text{ $\neg\varphi$, $\psi$ }}        
\]    
r2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\psi$ }}        
{\text{  }}        
\]    
r3
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\varphi$ }}        
{\text{  }}        
\]    
r5
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$ }}        
\]    
r9
\[
\MCRuleInv        
{\text{ $\neg\varphi$ }}        
{\text{ $\varphi \to \psi$, $\neg\psi$ }}        
\]    
r14
\[
\MCRuleInv        
{\text{ $\neg\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$ }}        
\]    
r20
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\neg(\varphi \to \psi)$ }}        
\]    
r24
\[
\MCRuleInv        
{\text{ $\psi$ }}        
{\text{ $\varphi \to \psi$, $\varphi$ }}        
\]    
r4
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
r6
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$ }}        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
\]    
r10
\[
\MCRuleInv        
{\text{ $\neg\varphi$ }}        
{\text{ $\neg(\varphi \land \psi)$, $\psi$ }}        
\]    
r15
\[
\MCRuleInv        
{\text{ $\neg\psi$ }}        
{\text{ $\neg(\varphi \land \psi)$, $\varphi$ }}        
\]    
r19
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\varphi \land \psi$ }}        
\]    
r25
\[
\MCRuleInv        
{\text{ $\psi$ }}        
{\text{ $\varphi \land \psi$ }}        
\]    
r7
\[
\MCRuleInv        
{\text{ $\neg\neg\varphi$ }}        
{\text{ $\varphi$ }}        
\]    
r13
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$ }}        
{\text{  }}        
\]    
r21
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\neg\neg\varphi$ }}        
\]    
r8
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$ }}        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
\]    
r11
\[
\MCRuleInv        
{\text{ $\neg\varphi$ }}        
{\text{ $\neg(\varphi \lor \psi)$ }}        
\]    
r12
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi \lor \psi$ }}        
{\text{  }}        
\]    
r16
\[
\MCRuleInv        
{\text{ $\neg\psi$ }}        
{\text{ $\neg(\varphi \lor \psi)$ }}        
\]    
r17
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi \lor \psi$ }}        
{\text{  }}        
\]    
r18
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
r22
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\neg\psi$, $\varphi \lor \psi$ }}        
\]    
r23
\[
\MCRuleInv        
{\text{ $\varphi$, $\psi$ }}        
{\text{ $\varphi \lor \psi$ }}        
\]    
r26
\[
\MCRuleInv        
{\text{ $\psi$ }}        
{\text{ $\neg\varphi$, $\varphi \lor \psi$ }}        
\] 
\end{center}

\subsubsection{Full}
\begin{center}
$\to$-1,1,1
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
$\to$-2,2,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
$\to$-1,2,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
$\to$-0,2,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\psi$, $\varphi$ }}        
{\text{ $\psi$ }}        
\]    
$\to$-0,1,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\varphi$ }}        
{\text{ $\neg\psi$, $\psi$ }}        
\]    
$\to$-0,0,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\varphi$, $\psi$ }}        
{\text{  }}        
\]    
$\to$-1,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
$\to$-2,1,0
\[
\MCRuleInv        
{\text{ $\neg\varphi$ }}        
{\text{ $\varphi \to \psi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
$\to$-2,2,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$, $\varphi$, $\psi$ }}        
\]    
$\to$-2,0,0
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\psi$ }}        
{\text{ $\varphi \to \psi$, $\varphi$ }}        
\]    
$\to$-1,2,2
\[
\MCRuleInv        
{\text{ $\neg\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$, $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
$\to$-0,2,2
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi$ }}        
{\text{ $\neg(\varphi \to \psi)$, $\psi$ }}        
\]    
$\to$-0,1,2
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\neg(\varphi \to \psi)$, $\neg\psi$, $\psi$ }}        
\]    
$\to$-0,0,2
\[
\MCRuleInv        
{\text{ $\varphi$, $\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$ }}        
\]    
$\to$-1,0,0
\[
\MCRuleInv        
{\text{ $\psi$ }}        
{\text{ $\varphi \to \psi$, $\neg\varphi$, $\varphi$ }}        
\]    
and-1,1,1
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
and-2,1,2
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$, $\neg\varphi$ }}        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
and-2,2,2
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$, $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
and-1,2,2
\[
\MCRuleInv        
{\text{ $\varphi \land \psi$, $\neg\psi$ }}        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
and-1,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \land \psi)$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
and-2,1,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$ }}        
{\text{ $\neg(\varphi \land \psi)$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
and-2,2,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\neg(\varphi \land \psi)$, $\varphi$, $\psi$ }}        
\]    
and-2,0,0
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\psi$ }}        
{\text{ $\varphi \land \psi$, $\varphi$ }}        
\]    
and-1,2,2
\[
\MCRuleInv        
{\text{ $\neg\psi$ }}        
{\text{ $\neg(\varphi \land \psi)$, $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
and-0,2,0
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi$ }}        
{\text{ $\varphi \land \psi$, $\psi$ }}        
\]    
and-0,1,0
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\varphi \land \psi$, $\neg\psi$, $\psi$ }}        
\]    
and-0,0,0
\[
\MCRuleInv        
{\text{ $\varphi$, $\psi$ }}        
{\text{ $\varphi \land \psi$ }}        
\]    
and-1,0,0
\[
\MCRuleInv        
{\text{ $\psi$ }}        
{\text{ $\varphi \land \psi$, $\neg\varphi$, $\varphi$ }}        
\]    
neg-1,1
\[
\MCRuleInv        
{\text{ $\neg\neg\varphi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
neg-1,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$ }}        
{\text{ $\neg\varphi$, $\varphi$ }}        
\]    
neg-0,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$ }}        
{\text{  }}        
\]    
neg-0,2
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\neg\neg\varphi$ }}        
\]    
or-1,1,1
\[
\MCRuleInv        
{\text{ $\neg(\varphi \lor \psi)$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
or-2,1,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
or-2,2,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\varphi$, $\psi$ }}        
\]    
or-2,2,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi \lor \psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
or-2,1,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi \lor \psi$ }}        
{\text{ $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
or-2,0,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi \lor \psi$, $\psi$ }}        
{\text{ $\varphi$ }}        
\]    
or-2,0,2
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\psi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\varphi$ }}        
\]    
or-1,2,2
\[
\MCRuleInv        
{\text{ $\neg\psi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
or-1,2,2
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi \lor \psi$ }}        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
\]    
or-0,2,2
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi \lor \psi$, $\varphi$ }}        
{\text{ $\psi$ }}        
\]    
or-0,2,2
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\varphi$ }}        
{\text{ $\neg(\varphi \lor \psi)$, $\psi$ }}        
\]    
or-1,1,1
\[
\MCRuleInv        
{\text{ $\varphi \lor \psi$ }}        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
\]    
or-0,1,0
\[
\MCRuleInv        
{\text{ $\varphi$ }}        
{\text{ $\neg\psi$, $\varphi \lor \psi$, $\psi$ }}        
\]    
or-0,0,0
\[
\MCRuleInv        
{\text{ $\varphi$, $\psi$ }}        
{\text{ $\varphi \lor \psi$ }}        
\]    
or-1,0,0
\[
\MCRuleInv        
{\text{ $\psi$ }}        
{\text{ $\neg\varphi$, $\varphi \lor \psi$, $\varphi$ }}        
\]    
\end{center}

==> set-set-calculi/sk.tex <==
\subsection{$\SKName$}

Notice that we will only change the implication
with respect to $\L_3$.

\subsubsection{Simplified}
\begin{center}
r2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$ }}        
{\text{ $\neg\varphi$ }}        
\]    
r3
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$ }}        
{\text{ $\psi$ }}        
\]    
r5
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$ }}        
{\text{ $\neg\psi$, $\varphi$ }}        
\]    
r13
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$ }}        
{\text{ $\neg(\varphi \to \psi)$ }}        
\]    
r14
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\psi$ }}        
{\text{ $\varphi \to \psi$ }}        
\]    
r15
\[
\MCRuleInv        
{\text{ $\neg\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$, $\varphi$ }}        
\]    
r23
\[
\MCRuleInv        
{\text{ $\psi$ }}        
{\text{ $\varphi \to \psi$, $\varphi$ }}        
\]
\end{center}

\subsubsection{Full}

\begin{center}
$\to$-2,2,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$ }}        
{\text{ $\varphi$, $\psi$ }}        
\]    
$\to$-1,2,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\varphi$, $\varphi$ }}        
{\text{ $\psi$ }}        
\]    
$\to$-0,1,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\neg\psi$, $\varphi$, $\psi$ }}        
{\text{ $\neg\varphi$ }}        
\]    
$\to$-0,2,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\varphi$ }}        
{\text{ $\neg\varphi$, $\psi$ }}        
\]    
$\to$-0,0,2
\[
\MCRuleInv        
{\text{ $\varphi \to \psi$, $\varphi$, $\psi$ }}        
{\text{ $\neg\varphi$, $\neg\psi$ }}        
\]    
$\to$-2,0,0
\[
\MCRuleInv        
{\text{ $\neg(\varphi \to \psi)$, $\psi$ }}        
{\text{ $\neg\psi$, $\varphi$ }}        
\]    
$\to$-1,1,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
{\text{ $\varphi \to \psi$ }}        
\]    
$\to$-1,1,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\neg\psi$, $\varphi$, $\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$ }}        
\]    
$\to$-1,0,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
{\text{ $\varphi \to \psi$, $\neg\psi$ }}        
\]    
$\to$-1,0,1
\[
\MCRuleInv        
{\text{ $\neg\varphi$, $\varphi$, $\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$, $\neg\psi$ }}        
\]    
$\to$-2,1,1
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\psi$ }}        
{\text{ $\varphi \to \psi$, $\varphi$ }}        
\]    
$\to$-2,1,1
\[
\MCRuleInv        
{\text{ $\neg\psi$, $\psi$ }}        
{\text{ $\neg(\varphi \to \psi)$, $\varphi$ }}        
\]    
$\to$-2,0,0
\[
\MCRuleInv        
{\text{ $\psi$ }}        
{\text{ $\varphi \to \psi$, $\neg\psi$, $\varphi$ }}        
\]
\end{center}

==> umberto.tex <==
\section{U}

A provisional abstract:

The topic of our chapter would be ‘Alternative proof-theoretic approaches (to 3-valued logics)’. Namely, we deal with two main approaches and the connection between them: (1) Display style-calculi and (2) Multiple-conclusion (Hilbert-style) calculi. 

Regarding (1) … 

Regarding (2), we show that a very inclusive class of 3-valued logics may be axiomatized in a systematic and indeed algorithmic fashion using multiple-conclusion calculi enjoying desirable proof-theoretic properties (e.g. analyticity and a straightforward proof-search and counter-model search procedure). This class corresponds to logics characterised by logical matrices that are monadic, i.e. capable of distinguishing each truth value by using only formulas in a single variable. Such a requirement is met in the presence of a suitable negation. Indeed, our method applies uniformly to virtually all the 3-valued logics considered in the literature, and in particular to the systems considered by Avron-Zamansky and by Paoli-Pra Baldi in their respective chapters in this book, giving analytic multiple-conclusion calculi for each of them. We also show that, under more restrictive assumptions (e.g. if the logic possesses a disjunction connective), our multiple-conclusion calculi can be translated into single-conclusion Hilbert calculi. With regards to the sequent calculi considered by Avron-Zamansky, we show that they are essentially equivalent to our approach (ours being simpler in that it does not employ meta-theoretic notions such as ’sequent’) and can be directly translated into our calculi. We include a few examples of non-monadic matrices in order to exemplify how one can go beyond the above-mentioned technical provisos in our general approach [and we discuss the relation of the multiple-conclusion approach with the display calculus one].


Reasonable assumptions:
\begin{itemize}
    \item That all logics considered here possess a negation, either the Kleene or the Godel negation.
    Or even more generally, that every matrix considered is monadic, observing that having a negation of the above kind (or which other connectives?) is as sufficient condition.
    
    \item That all logics are sub-classical in the sense that their tables coincide with the classical ones on
    the classical values $\{ 0,1 \}$.
\end{itemize}

Connection with Giuseppe's work: we try to translate the same calculi from Avron's papers using our approach and the display calculi, and we discuss the features of the resulting axiomatizations.

\textbf{Remark}: let us use '(subset of) designated elements' instead of 'filter', to avoid confusion with lattice filters.

\section{Analytic calculi for three-valued logics (Giuseppe)}

We review the proof-theoretic literature on propositional finite-valued logics and, in particular, so-called \emph{sub-classical 3-valued logics}, namely logics characterized by truth-tables that coincide with the classical ones on the values $\{0,1\}$.

We will consider and compare various generalizations and refinements of traditional Hilbert, tableaux, natural deduction, relational and sequent calculi. Specific, desirable features--such as automatic generation of rules, analyticity, proof search and counter-model generation procedures--will be considered. 

A preliminary analysis of the state-of-the-art literature on non-classical logics, and 3-valued logics in particular, reveals that two main strategies are pursued: (i) expanding the \emph{meta-language} of the formalisms (via labels or types) or (ii) generalizing the usual notion of \emph{sub-formula property} (while remaining as close as possible to the original language of the logic), where, in both cases, the minimal desirable feature is to guarantee \emph{decidability} of the associated symbolic procedure.

We will explore up to which extent the two strategies are compatible with one another, aiming to provide formal translations between proofs of various formalism whenever possible.  

The key ingredient of the present approach rests on the order-theoretic analysis of the relevant connectives and their mutual interactions. An expected by-product of the analysis will provide a (tentative) classification (and relative comparison) of the current approaches, where various semantic features are "imported" in various formalisms. 

==> upward-branching-notation.tex <==
\subsection{Upward-branching derivation trees}

Recall that \SetSet{} proofs were defined as trees built starting from
the premises and expanding
the nodes until obtaining a conclusion formula in
each of the leaf nodes.
%\SetSet{} proofs are trees with a set of premises on the top layer and conclusion formulas on the bottom layer. 
In this downward-branching perspective, trees pack all premises in one and the same root node. An alternative would be the upward-branching perspective, which packs all the conclusions in one and the same root node, getting closer to the
most usual notation for derivation trees in sequent-style
systems (see Section~\ref{sec:3LabelledCalculi}).
We will now compare and illustrate these different
views (which we shall refer simply as different notations)
on \SetSet{} proofs.

In the downward-branching notation (the one we have been working with), rules are represented in \emph{disjunctive rule form}, meaning that metalinguistical conjunctions $\Sand$ (in this case, represented as commas in derivations trees) always occur under the scope of metalinguistical disjunctions $\Sor$ (in this case, represented as white spaces between branches). Note that the set of formulas labelling each node is upward closed, meaning that each node $\NodeA$ is actually labelled with all formulas labelling the nodes above $\NodeA$ on the same branch. When writing derivations, only active formulas are explicitly depicted. We call $\Sand$-\emph{components} or \emph{proof sections} the branches in a derivation tree, that is, the sequences of nodes from the root to a leaf. Notice that each formula occurs exactly once in a proof section even though it is used in multiple rule applications.

In order to guide our discussion, we present again the
\SetSet{} rules for the negation and implication connectives of 
$\LThreeName$ below, obtained
from our recipe (we call it $\smcName{\LThreeName}$).
\Fixed{21}{Note that we have simplified the notation for the name
of the rules in order to avoid cluttering of symbols in the subsequent
discussion}.

\begin{gather*}
    \MCRule{\PropA}{\neg\neg\PropA}{\LukRule{1}{\lukNeg}}
    \quad
    \MCRule{\neg\neg\PropA}{\PropA}{\LukRule{2}{\lukNeg}}
    \quad
    \MCRule{\PropA,\neg\PropA}{}{\LukRule{3}{\lukNeg}}
    \\
    %%%%
    %\MCRule{\PropA,\PropB}{\PropA\land\PropB}{\LukRule{4}{\aand}}%5
    %\quad
    %\MCRule{\neg\PropA}{\neg(\PropA\land\PropB)}{\mathsf{r}_7^\aand}
    %\quad
    %\MCRule{\neg\PropB}{\neg(\PropA\land\PropB)}{\mathsf{r}_8^\aand}
    %\quad
    %\MCRule{\neg(\PropA\land\PropB), \PropB}{\neg\PropA}{\mathsf{r}_{12}^\aand}
    %\\
    %\MCRule{\neg(\PropA\land\PropB)}{\neg\PropA,\neg\PropB}{\mathsf{r}_{14}^\aand}
    %\quad
    %\MCRule{\neg(\PropA\land\PropB), \PropA}{\neg\PropB}{\mathsf{r}_{16}^\aand}
    %\quad
    %\MCRule{\PropA\land\PropB}{\PropA}{\mathsf{r}_{20}^\aand}\quad
    %\MCRule{\PropA\land\PropB}{\PropB}{\mathsf{r}_{25}^\aand}\\
    %%%%
    %\MCRule{\neg\PropA,\neg\PropB}{\neg(\PropA\lor\PropB)}{\mathsf{r}_{10}^\aor}
    %\quad
    %\MCRule{\neg(\PropA\lor\PropB)}{\neg\PropA}{\mathsf{r}_{13}^\aor}
    %\quad
    %\MCRule{\neg(\PropA\lor\PropB)}{\neg\PropB}{\mathsf{r}_{17}^\aor}
    %\quad
    %\MCRule{\PropA}{\PropA\lor\PropB}{\mathsf{r}_{18}^\aor}
    %\quad
    %\MCRule{\PropB}{\PropA\lor\PropB}{\mathsf{r}_{19}^\aor}
    %\quad
    %\MCRule{\PropA\lor\PropB}{\PropA,\PropB}{\mathsf{r}_{23}^\aor}\\
    %%%%
    \MCRule{\neg\PropA}{\PropA\to\PropB}{\LukRule{4}{\lukImp}}\quad
    \MCRule{\PropB}{\PropA\to\PropB}{\LukRule{5}{\lukImp}}\quad
    \MCRule{}{\PropA,\neg\PropB,\PropA\to\PropB}{\LukRule{6}{\lukImp}}\quad
    \MCRule{\PropA,\neg\PropB}{\neg(\PropA\to\PropB)}{\LukRule{7}{\lukImp}}\\
    \MCRule{\PropA\to\PropB,\neg\PropB}{\neg\PropA}{\LukRule{8}{\lukImp}}\quad%11
    \MCRule{\neg(\PropA\to\PropB)}{\neg\PropB}{\LukRule{9}{\lukImp}}\quad%15
    \MCRule{\neg(\PropA\to\PropB)}{\PropA}{\LukRule{10}{\lukImp}}\quad%21
    \MCRule{\PropA,\PropA\to\PropB}{\PropB}{\LukRule{11}{\lukImp}}\quad%24
\end{gather*}

Below we provide a $\smcName{\LThreeName}$-proof $\TreeA$ in disjunctive rule form of 
%$((\FmA \ararr \FmB) \ararr \FmB) \ararr ((\FmB \ararr \FmA) \ararr \FmA)$
\Fixed{22}{$(\neg\FmB \to \neg\FmA) \to (\FmA\to\FmB)$}
. In order to simplify the presentation of the tree, we will write $\alpha_i$ for the formula 
%$((\FmA \ararr \FmB) \ararr \FmB) \ararr ((\FmB \ararr \FmA) \ararr \FmA)$
\Fixed{22}{$(\neg\FmB \to \neg\FmA) \to (\FmA\to\FmB)$}
, with $1 \leq i \leq 5$. Besides, to facilitate the reading, we add superscripts $a, b, c, d$ matching premises with rule applications performed at a later stage in the derivation.

\vspace{0.5cm}

\begin{math} 
\hspace{2cm}
    \begin{tikzpicture}[every tree node/.style={},
       level distance=1.2cm,sibling distance=.05cm,
       edge from parent path={(\tikzparentnode) -- (\tikzchildnode)}, baseline]
        \Tree[.\node[style={}] {$\varnothing$};
            \edge[] node[auto=right]{$\LukRule{6}{\lukImp}$};
            [.{$\alpha_5$}
            ]
            [.{$\neg \FmB \to \neg \FmA^{ab}$}
                \edge[] node[auto=right]{$\LukRule{6}{\lukImp}$};
                [.{$\FmA \to \FmB$}
                    \edge[] node[auto=right]{$\LukRule{5}{\lukImp}$};
                    [.{$\alpha_4$}
                    ]
                ]
                [.{$\neg \FmB$}
                    \edge[] node[auto=right]{$\LukRule{11}{\lukImp}^a$};
                    [.{$\neg \FmA$}
                        \edge[] node[auto=right]{$\LukRule{4}{\lukImp}$};
                        [.{$\FmA \to \FmB$}
                            \edge[] node[auto=right]{$\LukRule{5}{\lukImp}$};
                            [.{$\alpha_3$}
                            ]
                        ]
                    ]
                ]
                [.{$\FmA$}
                    \edge[] node[auto=right]{$\LukRule{1}{\lukNeg}$};
                    [.{$\neg\neg \FmA$}
                        \edge[] node[auto=right]{$\LukRule{8}{\lukImp}^b$};
                        [.{$\neg\neg \FmB$}
                            \edge[] node[auto=right]{$\LukRule{2}{\lukNeg}$};
                            [.{$\FmB$}
                                \edge[] node[auto=right]{$\LukRule{5}{\lukImp}$};
                                [.{$\FmA \to \FmB$}
                                    \edge[] node[auto=right]{$\LukRule{5}{\lukImp}$};
                                    [.{$\alpha_2$}
                                    ]
                                ]
                            ]
                        ]
                    ]
                ]
            ]
            [.{$\neg(\FmA \to \FmB)^c$}
                \edge[] node[auto=right]{$\LukRule{10}{\lukImp}$};
                [.{$\FmA$}
                    \edge[] node[auto=right]{$\LukRule{1}{\lukNeg}$};
                    [.{$\neg\neg \FmA^d$}
                        \edge[] node[auto=right]{$\LukRule{9}{\lukImp}^c$};
                        [.{$\neg \FmB$}
                            \edge[] node[auto=right]{$\LukRule{7}{\lukImp}^d$};
                            [.{$\neg(\neg \FmB \to \neg \FmA)$}
                                \edge[] node[auto=right]{$\LukRule{4}{\lukImp}$};
                                [.{$\alpha_1$}
                                ]
                            ]
                        ]
                    ]
                ]
            ]
        ]
    \end{tikzpicture}
\end{math}

\vspace{0.5cm}

\noindent Notice that in the derivation $\TreeA$ above there are five $\Sand$-components: 
\begin{itemize}
\item $\pi_1$ is the proof section $\lb \LukRule{10}{\lukImp}, \LukRule{1}{\lukNeg}, \LukRule{9}{\lukImp}, \LukRule{7}{\lukImp}, \LukRule{4}{\lukImp} \rb[\aneg(\FmA \ararr \FmB), \alpha_1]$, where $\lb \LukRule{10}{\lukImp}, \LukRule{1}{\lukNeg}, \LukRule{9}{\lukImp}, \LukRule{7}{\lukImp}, \LukRule{4}{\lukImp} \rb$ is the string of rule applications from top to bottom, $\aneg(\FmA \ararr \FmB)$ is the label of the initial node and $\alpha_1$ is the label of the terminal node;
\item $\pi_2$ is the proof section $\lb \LukRule{1}{\lukNeg}, \LukRule{8}{\lukImp}, \LukRule{2}{\lukNeg}, \LukRule{5}{\lukImp}, \LukRule{5}{\lukImp} \rb[\FmA, \alpha_2]$;
\item $\pi_3$ is the proof section $\lb \LukRule{11}{\lukImp}, \LukRule{4}{\lukImp}, \LukRule{5}{\lukImp} \rb[\neg \FmB, \alpha_3]$;
\item $\pi_4$ is the proof section $\lb \LukRule{5}{\lukImp} \rb[\FmA \ararr \FmB,\alpha_4]$; and
\item $\pi_5$ is the proof section $\lb \varnothing \rb[\alpha_5, \varnothing]$, where $\lb \varnothing \rb$ is the empty string of rule applications, and $[\alpha_5, \varnothing]$ denotes the fact that there is only one initial node.
\end{itemize}

In the upward-branching notation, rules are represented in \emph{conjunctive rule form}, meaning that metalinguistic disjunctions $\Sor$ (in this case, represented as commas in actual derivations) always occur under the scope of metalinguistic conjunctions $\Sand$ (in this case, represented as white spaces between branches). 
%
In what follows, we first provide a conjunctive rule form representation of the $\Sand$-components $\pi_1, \pi_2, \pi_3, \pi_4, \pi_5$ occurring in the previous derivation $\pi$.

The conjunctive rule form representation of the $\Sand$-component $\pi_1$ is the following: 

\begin{center}
{\small
\AXC{$\aneg (\FmA \ararr \FmB)$}
\RL{$\LukRule{10}{\lukImp}$}
\UIC{$\FmA $}
\RL{$\LukRule{1}{\lukNeg}$}
\UIC{$\aneg \aneg \FmA$}
%
\AXC{$\aneg (\FmA \ararr \FmB)$}
\RL{$\LukRule{9}{\lukImp}$}
\UIC{$\aneg \FmB$}
%
\RL{$\LukRule{7}{\lukImp}$}
\BIC{$\aneg (\aneg \FmB \ararr \aneg \FmA)$}
\RL{$\LukRule{4}{\lukImp}$}
\UIC{$\rule[-0.7mm]{0mm}{2.8mm}\alpha_1$}
\DP
 }
\end{center}

\noindent \sloppy Notice that the previous derivation is, indeed, a notational variant of the $\Sand$-component $\pi_1$: the initial nodes are labelled with $\aneg (\FmA \ararr \FmB)$ and the terminal node is labelled with $\alpha_1$ (and the string of rule applications from top-left to right-down is again $\lb \LukRule{10}{\lukImp}, \LukRule{1}{\lukNeg}, \LukRule{9}{\lukImp}, \LukRule{7}{\lukImp}, \LukRule{4}{\lukImp} \rb$). The only difference is just notational: in the previous presentation, $\aneg (\FmA \ararr \FmB)$ is used twice (as premise of $\LukRule{10}{\lukImp}$ and as premise of $\LukRule{9}{\lukImp}$) but explicitly represented only once, while in this case $\aneg (\FmA \ararr \FmB)$ is explicitly represented as many times it is used. So, taking into account the arity of rules and the tree-shape of proof sections, we may rewrite the string of rule applications as the following bracketed string: $\LukRule{4}{\lukImp}(\LukRule{7}{\lukImp}(\LukRule{1}{\lukNeg}(\LukRule{10}{\lukImp} (\aneg(\FmA \ararr \FmB))), \LukRule{9}{\lukImp} (\aneg(\FmA \ararr \FmB))))[\alpha_1]$, where $\aneg(\FmA \ararr \FmB)$ is the label of the leaves (aka the initial node) and $\alpha_1$ is the root (aka the terminal node).

The conjunctive rule form representation of the $\Sand$-component $\pi_2$ is the following: 

\begin{center}
\AXC{$\aneg \FmB \ararr \aneg \FmA$}
\AXC{$\FmA$}
\RL{$\LukRule{1}{\lukNeg}$}
\UIC{$\aneg\aneg \FmA$}
\RL{$\LukRule{8}{\lukImp}$}
\BIC{$\aneg \aneg \FmB$}
\RL{$\LukRule{2}{\lukNeg}$}
\UIC{$\FmB$}
\RL{$\LukRule{5}{\lukImp}$}
\UIC{$\FmA \ararr \FmB$}
\RL{$\LukRule{5}{\lukImp}$}
\UIC{$\rule[-0.7mm]{0mm}{2.8mm}\alpha_2$}
\DP
\end{center}

\noindent Again, notice that the previous derivation is, indeed, a notational variant of the $\Sand$-component $\pi_2$. Taking into account the arity of rules and the tree-shape of proof sections, we may rewrite the string of rule applications as the following bracketed string: 
\Fixed{23}{$\LukRule{5}{\lukImp}(
    \LukRule{5}{\lukImp}(
        \LukRule{2}{\lukImp}(
            \LukRule{8}{\lukImp}(
            \neg\FmB \to \neg\FmA,
                \LukRule{1}{\lukImp}(
                    \FmA
                )
            )
        )
    )
)[\alpha_2]$}.
%$\LukRule{5}{\lukImp}(\LukRule{5}{\lukImp}(\LukRule{2}{\lukNeg}(\aneg \FmB \ararr \aneg \FmA, \LukRule{8}{\lukImp}(\LukRule{1}{\lukNeg}))))[\alpha_2]$.

%The conjunctive rule form representation of the $\Sand$-component $\pi_3$ is the following: 
%
%\begin{center}
%\AXC{$\aneg B \ararr \aneg A$}
%\AXC{$\aneg B$}
%\RL{$\mathsf{r}_{24}$}
%\BIC{$\aneg A$}
%\RL{$\mathsf{r}_2$}
%\UIC{$A \ararr B$}
%\RL{$\mathsf{r}_3$}
%\UIC{$\rule[-0.7mm]{0mm}{2.8mm}\alpha_3$}
%\DP
%\end{center}
%
%Notice that the previous derivation is, indeed, a notational variant of the $\Sand$-component $\pi_3$. Taking into account the arity of rules and the tree-shape of proof sections, we may rewrite the string of rule applications as the following bracketed string: $\mathsf{r}_2(\aneg B \ararr \aneg A, \mathsf{r}_{24})[\alpha_3]$.
%
%The conjunctive rule form representation of the $\Sand$-component $\pi_4$ is the following: 
%
%\begin{center}
%\AXC{$A \ararr B$}
%\RL{$\mathsf{r}_3$}
%\UIC{$\rule[-0.7mm]{0mm}{2.8mm}\alpha_4$}
%\DP
%\end{center}
%
%Notice that the previous derivation is, indeed, a notational variant of the $\Sand$-component $\pi_4$. Taking into account the arity of rules and the tree-shape of proof sections, we may rewrite the string of rule applications as the following bracketed string: $\mathsf{r}_3(A \ararr B)[\alpha_4]$.
%
%The conjunctive rule form representation of the $\Sand$-component $\pi_5$ is the following: 
%
%\begin{center}
%\AXC{$\alpha_5$}
%\DP
%\end{center}
%
%Notice that the previous derivation is, indeed, a notational variant of the $\Sand$-component $\pi_5$. Taking into account the arity of rules and the tree-shape of proof sections, we may rewrite the string of rule applications as the following bracketed string: $\emptyset[\alpha_5]$.

Assume we have done this process for the other
proof sections.
Now we put together all the $\Sand$-components $\pi_i$ with $1 \leq i \leq 5$, to represent the full proof $\TreeA$ in conjunctive rule form. Also in this case we adopt the convention that only active formulas are depicted in the proof: it follows that commas can appear only on the leaves with a disjunctive reading $\Sor$. Vice-versa, in the case of disjunctive rule form presentations, commas might appear only on the root with a conjunctive reading. Notice that now we have six leaves, given that in the previous proof we have a nesting of two $\LukRule{6}{\lukImp}$ applications and each of which has three conclusion formulas. To facilitate the reading, we add superscripts $a, b, c, d, e$ matching premises with rule applications performed at a later stage in the derivation.
\vspace{0.5cm}
{
\small
\begin{equation*}
\def\ScoreOverhang{.2pt} 
\AXC{$\LukRule{6}{\lukImp}$}
\UIC{$\aneg (\FmA \ararr \FmB),^a$}
\noLine
\UIC{$\alpha_5,$}
\noLine
\UIC{$\aneg \FmB \ararr \aneg \FmA$}
%%
\AXC{$\LukRule{6}{\lukImp}$}
\UIC{$\aneg (\FmA \ararr \FmB),^a$}
\noLine
\UIC{$\alpha_5,$}
\noLine
\UIC{$\aneg \FmB \ararr \aneg \FmA$}
%
\AXC{$\LukRule{6}{\lukImp}$}
\UIC{$\Fixed{24}{\FmA},^b$}
\noLine
\UIC{$\FmA\ararr \FmB,^e$}
\noLine
\UIC{$\aneg \FmB$}
%
\RL{$\LukRule{11}{\lukImp}$}
\BIC{$\aneg \FmA$}
\RL{$\LukRule{4}{\lukImp}$}
\UIC{$\FmA \ararr \FmB$}
\RL{$\LukRule{5}{\lukImp}$}
\UIC{$\rule[-0.7mm]{0mm}{2.8mm}\alpha_3$}
\RL{${\LukRule{1}{\lukNeg}}^b$}
\UIC{$\aneg \aneg \FmA$}
%%
\RL{$\LukRule{8}{\lukImp}$}
\BIC{$\aneg \aneg \FmB$}
\RL{$\LukRule{2}{\lukNeg}$}
\UIC{$\FmB$}
\RL{$\LukRule{5}{\lukImp}$}
\UIC{$\FmA \ararr \FmB$}
\RL{$\LukRule{5}{\lukImp}$}
\UIC{$\rule[-0.7mm]{0mm}{2.8mm}\alpha_2$}
%
\RL{$\LukRule{10}{\lukImp}^a$}
\UIC{$\FmA $}
\RL{$\LukRule{1}{\lukNeg}$}
\UIC{$\aneg \aneg \FmA$}
%
\AXC{$\LukRule{6}{\lukImp}$}
\UIC{$\aneg (\FmA \ararr \FmB),^c$}
\noLine
\UIC{$\alpha_5,$}
\noLine
\UIC{$\aneg \FmB \ararr \aneg \FmA$}
%%
\AXC{$\LukRule{6}{\lukImp}$}
\UIC{$\aneg (\FmA \ararr \FmB),^c$}
\noLine
\UIC{$\alpha_5,$}
\noLine
\UIC{$\aneg \FmB \ararr \aneg \FmA$}
%
\AXC{$\LukRule{6}{\lukImp}$}
\UIC{$\FmA,^d$}
\noLine
\UIC{$\FmA\ararr \FmB,^e$}
\noLine
\UIC{$\aneg \FmB$}
%
\RL{$\LukRule{11}{\lukImp}$}
\BIC{$\aneg \FmA$}
\RL{$\LukRule{4}{\lukImp}$}
\UIC{$\FmA \ararr \FmB$}
\RL{$\LukRule{5}{\lukImp}$}
\UIC{$\rule[-0.7mm]{0mm}{2.8mm}\alpha_3$}
\RL{$\mathsf{r}_9^d$}
\UIC{$\aneg \aneg \FmA$}
%%
\RL{$\LukRule{8}{\lukImp}$}
\BIC{$\aneg \aneg \FmB$}
\RL{$\LukRule{2}{\lukNeg}$}
\UIC{$\FmB$}
\RL{$\LukRule{5}{\lukImp}$}
\UIC{$\FmA \ararr \FmB$}
\RL{$\LukRule{5}{\lukImp}$}
\UIC{$\rule[-0.7mm]{0mm}{2.8mm}\alpha_2$}
%
\RL{$\LukRule{9}{\lukImp}^c$}
\UIC{$\aneg \FmB$}
%
\RL{$\LukRule{7}{\lukImp}$}
\BIC{$\aneg (\aneg \FmB \ararr \aneg \FmA)$}
\RL{$\LukRule{4}{\lukImp}$}
\UIC{$\rule[-0.7mm]{0mm}{2.8mm}\alpha_1$}
\RL{$\LukRule{5}{\lukImp}^e$}
\UIC{$\rule[-0.7mm]{0mm}{2.8mm}\alpha_4$}
\DP
\end{equation*}
}

\vspace{0.5cm}

Notice that the previous derivation is, indeed, a notational variant (in conjunctive rule form) of the derivation $\TreeA$ (in disjunctive rule form).
